Strong, weak and flavor scalar triplets for the CDF Wjj anomaly

A model describing the 4.1\sigma\ Wjj anomaly observed by the CDF experiment at the Tevatron collider is introduced. It features new scalar particles which are charged both under the SU(3)_C and the SU(2)_L gauge groups and which couple to pairs of quarks. We introduce several identical replicas of the scalar multiplets in order to leave an unbroken U(3)_Q x U(3)_U x U(3)_D flavor symmetry to satisfy the constraints coming from flavor physics. We discuss the LHC reach on the new scalar resonances both in the resonant production channel (with the Wjj final state) and in the QCD pair production channel (with the 4j final state).

==> pbound1 <==
pbound1 = Graphics[{GraphicsComplex[{{0.5589473890581718, 
       0.035789496759002774}, {0.637368433434903, 0.035789496759002774}, 
       {0.7157894778116343, 0.035789496759002774}, {0.7942105221883655, 
       0.035789496759002774}, {0.8726315665650968, 0.035789496759002774}, 
       {0.951052610941828, 0.035789496759002774}, {1.0294736553185593, 
       0.035789496759002774}, {1.1078946996952905, 0.035789496759002774}, 
       {1.1863157440720218, 0.035789496759002774}, {1.264736788448753, 
       0.035789496759002774}, {1.3431578328254843, 0.035789496759002774}, 
       {1.4215788772022155, 0.035789496759002774}, {1.4999999215789475, 
       0.035789496759002774}, {0.4021053003047092, 0.06157896772853186}, 
       {0.4805263446814405, 0.06157896772853186}, {0.5589473890581718, 
       0.06157896772853186}, {0.637368433434903, 0.06157896772853186}, 
       {0.3236842559279779, 0.08736843869806095}, {0.4021053003047092, 
       0.08736843869806095}, {0.4805263446814405, 0.08736843869806095}, 
       {0.5589473890581718, 0.08736843869806095}, {0.3236842559279779, 
       0.11315790966759004}, {0.4021053003047092, 0.11315790966759004}, 
       {0.4805263446814405, 0.11315790966759004}, {0.3236842559279779, 
       0.13894738063711912}, {0.4021053003047092, 0.13894738063711912}, 
       {0.3236842559279779, 0.1647368516066482}, {0.4021053003047092, 
       0.1647368516066482}, {0.3236842559279779, 0.19052632257617727}, 
       {0.4021053003047092, 0.19052632257617727}, {0.3236842559279779, 
       0.21631579354570635}, {0.4021053003047092, 0.21631579354570635}, 
       {0.3236842559279779, 0.24210526451523542}, {0.4021053003047092, 
       0.24210526451523542}, {0.3236842559279779, 0.2678947354847645}, 
       {0.4021053003047092, 0.2678947354847645}, {0.3236842559279779, 
       0.2936842064542936}, {0.4021053003047092, 0.2936842064542936}, 
       {0.3236842559279779, 0.3194736774238227}, {0.4021053003047092, 
       0.3194736774238227}, {0.3236842559279779, 0.3452631483933518}, 
       {0.4021053003047092, 0.3452631483933518}, {0.3236842559279779, 
       0.3710526193628809}, {0.4021053003047092, 0.3710526193628809}, 
       {0.3236842559279779, 0.39684209033241}, {0.4021053003047092, 
       0.39684209033241}, {0.3236842559279779, 0.42263156130193913}, 
       {0.4021053003047092, 0.42263156130193913}, {0.3236842559279779, 
       0.44842103227146823}, {0.4021053003047092, 0.44842103227146823}, 
       {0.3236842559279779, 0.47421050324099734}, {0.4021053003047092, 
       0.47421050324099734}, {0.3236842559279779, 0.49999997421052633}, 
       {0.4021053003047092, 0.49999997421052633}, {0.5197368668698061, 
       0.04868423224376732}, {0.9118420887534624, 0.02289476127423823}, 
       {0.9902631331301937, 0.02289476127423823}, {1.068684177506925, 
       0.02289476127423823}, {1.1471052218836562, 0.02289476127423823}, 
       {1.2255262662603874, 0.02289476127423823}, {1.3039473106371187, 
       0.02289476127423823}, {1.38236835501385, 0.02289476127423823}, 
       {1.4607893993905816, 0.02289476127423823}, {1.4999999215789475, 
       0.02289476127423823}, {0.4413158224930749, 0.04868423224376732}, 
       {0.3628947781163435, 0.07447370321329641}, {0.4805263446814405, 
       0.04868423224376732}, {0.6765789556232686, 0.04868423224376732}, 
       {0.7549999999999999, 0.04868423224376732}, {0.8334210443767311, 
       0.04868423224376732}, {0.9118420887534624, 0.04868423224376732}, 
       {0.3236842559279779, 0.07447370321329641}, {0.5981579112465374, 
       0.07447370321329641}, {0.2844737337396122, 0.1260526451523546}, 
       {0.5197368668698061, 0.10026317418282549}, {0.2844737337396122, 
       0.15184211612188364}, {0.4413158224930749, 0.1260526451523546}, 
       {0.4805263446814405, 0.1260526451523546}, {0.4413158224930749, 
       0.15184211612188364}, {0.2844737337396122, 0.17763158709141275}, 
       {0.4413158224930749, 0.17763158709141275}, {0.2844737337396122, 
       0.2034210580609418}, {0.4413158224930749, 0.2034210580609418}, 
       {0.2844737337396122, 0.2292105290304709}, {0.4413158224930749, 
       0.2292105290304709}, {0.2844737337396122, 0.25499999999999995}, 
       {0.4413158224930749, 0.25499999999999995}, {0.2844737337396122, 
       0.28078947096952905}, {0.4413158224930749, 0.28078947096952905}, 
       {0.2844737337396122, 0.30657894193905816}, {0.4413158224930749, 
       0.30657894193905816}, {0.2844737337396122, 0.33236841290858726}, 
       {0.4413158224930749, 0.33236841290858726}, {0.2844737337396122, 
       0.35815788387811637}, {0.4413158224930749, 0.35815788387811637}, 
       {0.2844737337396122, 0.3839473548476455}, {0.4413158224930749, 
       0.3839473548476455}, {0.2844737337396122, 0.4097368258171746}, 
       {0.4413158224930749, 0.4097368258171746}, {0.2844737337396122, 
       0.4355262967867037}, {0.4413158224930749, 0.4355262967867037}, 
       {0.2844737337396122, 0.4613157677562328}, {0.4413158224930749, 
       0.4613157677562328}, {0.2844737337396122, 0.48710523872576184}, 
       {0.4413158224930749, 0.48710523872576184}, {0.2844737337396122, 
       0.49999997421052633}, {0.4413158224930749, 0.49999997421052633}, 
       {0.5197368668698061, 0.035789496759002774}, {0.951052610941828, 
       0.02289476127423823}, {1.0294736553185593, 0.02289476127423823}, 
       {1.1078946996952905, 0.02289476127423823}, {1.1863157440720218, 
       0.02289476127423823}, {1.264736788448753, 0.02289476127423823}, 
       {1.3431578328254843, 0.02289476127423823}, {1.4215788772022155, 
       0.02289476127423823}, {0.4021053003047092, 0.04868423224376732}, 
       {0.3628947781163435, 0.06157896772853186}, {0.7157894778116343, 
       0.04868423224376732}, {0.6765789556232686, 0.06157896772853186}, 
       {0.7942105221883655, 0.04868423224376732}, {0.8726315665650968, 
       0.04868423224376732}, {0.2844737337396122, 0.11315790966759004}, 
       {0.2844737337396122, 0.13894738063711912}, {0.4413158224930749, 
       0.13894738063711912}, {0.2844737337396122, 0.1647368516066482}, 
       {0.4413158224930749, 0.1647368516066482}, {0.2844737337396122, 
       0.19052632257617727}, {0.4413158224930749, 0.19052632257617727}, 
       {0.2844737337396122, 0.21631579354570635}, {0.4413158224930749, 
       0.21631579354570635}, {0.2844737337396122, 0.24210526451523542}, 
       {0.4413158224930749, 0.24210526451523542}, {0.2844737337396122, 
       0.2678947354847645}, {0.4413158224930749, 0.2678947354847645}, 
       {0.2844737337396122, 0.2936842064542936}, {0.4413158224930749, 
       0.2936842064542936}, {0.2844737337396122, 0.3194736774238227}, 
       {0.4413158224930749, 0.3194736774238227}, {0.2844737337396122, 
       0.3452631483933518}, {0.4413158224930749, 0.3452631483933518}, 
       {0.2844737337396122, 0.3710526193628809}, {0.4413158224930749, 
       0.3710526193628809}, {0.2844737337396122, 0.39684209033241}, 
       {0.4413158224930749, 0.39684209033241}, {0.2844737337396122, 
       0.42263156130193913}, {0.4413158224930749, 0.42263156130193913}, 
       {0.2844737337396122, 0.44842103227146823}, {0.4413158224930749, 
       0.44842103227146823}, {0.2844737337396122, 0.47421050324099734}, 
       {0.4413158224930749, 0.47421050324099734}, {0.38250003921052633, 
       0.05513159998614959}, {0.6961842167174515, 0.05513159998614959}, 
       {0.4609210835872577, 0.13250001289473684}, {0.5001316057756233, 
       0.042236864501385044}, {0.3432895170221607, 0.06802633547091413}, 
       {0.6765789556232686, 0.035789496759002774}, {0.7549999999999999, 
       0.035789496759002774}, {0.8334210443767311, 0.035789496759002774}, 
       {0.6569736945290858, 0.0293421290166205}, {0.7353947389058171, 
       0.0293421290166205}, {0.8138157832825483, 0.0293421290166205}, 
       {0.9902631331301937, 0.035789496759002774}, {0.9706578720360108, 
       0.042236864501385044}, {1.0098683942243765, 0.042236864501385044}, 
       {1.068684177506925, 0.035789496759002774}, {1.049078916412742, 
       0.042236864501385044}, {1.0882894386011077, 0.042236864501385044}, 
       {1.1471052218836562, 0.035789496759002774}, {1.1274999607894733, 
       0.042236864501385044}, {1.166710482977839, 0.042236864501385044}, 
       {1.2255262662603874, 0.035789496759002774}, {1.2059210051662046, 
       0.042236864501385044}, {1.2451315273545702, 0.042236864501385044}, 
       {1.3039473106371187, 0.035789496759002774}, {1.2843420495429358, 
       0.042236864501385044}, {1.38236835501385, 0.035789496759002774}, 
       {1.4607893993905816, 0.035789496759002774}, {0.6961842167174515, 
       0.0293421290166205}, {0.7157894778116343, 0.0293421290166205}, 
       {0.7746052610941827, 0.0293421290166205}, {0.7942105221883655, 
       0.0293421290166205}, {0.853026305470914, 0.0293421290166205}, 
       {0.9118420887534624, 0.035789496759002774}, {0.9314473498476452, 
       0.042236864501385044}, {0.951052610941828, 0.042236864501385044}, 
       {1.0294736553185593, 0.042236864501385044}, {1.1078946996952905, 
       0.042236864501385044}, {1.1863157440720218, 0.042236864501385044}, 
       {1.264736788448753, 0.042236864501385044}, {0.5981579112465374, 
       0.04868423224376732}, {0.5981579112465374, 0.035789496759002774}, 
       {0.3628947781163435, 0.10026317418282549}, {0.3236842559279779, 
       0.10026317418282549}, {0.3040789948337951, 0.10671054192520776}, 
       {0.4609210835872577, 0.15828948386426592}, {0.4609210835872577, 
       0.184078954833795}, {0.4609210835872577, 0.20986842580332407}, 
       {0.4609210835872577, 0.042236864501385044}, {0.7353947389058171, 
       0.05513159998614959}, {0.3040789948337951, 0.09381580644044321}, 
       {0.4609210835872577, 0.1453947483795014}, {0.4609210835872577, 
       0.17118421934903047}, {0.4609210835872577, 0.19697369031855955}, 
       {0.4609210835872577, 0.22276316128808862}, {0.5001316057756233, 
       0.035789496759002774}, {0.6177631723407202, 0.0293421290166205}, 
       {0.637368433434903, 0.0293421290166205}, {0.8922368276592796, 
       0.0293421290166205}, {0.8726315665650968, 0.0293421290166205}, 
       {0.8922368276592796, 0.02289476127423823}, {0.7157894778116343, 
       0.05513159998614959}, {0.7746052610941827, 0.05513159998614959}, 
       {0.5981579112465374, 0.06157896772853186}, {0.6177631723407202, 
       0.06802633547091413}, {0.5197368668698061, 0.07447370321329641}, 
       {0.5197368668698061, 0.08736843869806095}, {0.539342127963989, 
       0.09381580644044321}, {0.6961842167174515, 0.042236864501385044}, 
       {0.7746052610941827, 0.042236864501385044}, {0.853026305470914, 
       0.042236864501385044}, {0.5589473890581718, 0.07447370321329641}, 
       {0.5785526501523546, 0.08092107095567869}, {0.4413158224930749, 
       0.10026317418282549}, {0.4805263446814405, 0.10026317418282549}, 
       {0.5001316057756233, 0.10671054192520776}, {0.8922368276592796, 
       0.042236864501385044}, {0.9118420887534624, 0.042236864501385044}, 
       {0.637368433434903, 0.04868423224376732}, {0.6177631723407202, 
       0.042236864501385044}, {0.6961842167174515, 0.035789496759002774}, 
       {0.7746052610941827, 0.035789496759002774}, {0.853026305470914, 
       0.035789496759002774}, {0.3628947781163435, 0.08736843869806095}, 
       {0.3432895170221607, 0.09381580644044321}, {0.4021053003047092, 
       0.046165729219399244}, {0.4805263446814405, 0.03594060694046486}, 
       {0.7058719726878191, 0.06157896772853186}, {1.3431578328254843, 
       0.041934644138460875}, {1.4215788772022155, 0.04153168365456198}, 
       {1.4999999215789475, 0.04112872317066309}, {0.3236842559279779, 
       0.0705448384952822}, {0.29931169989976036, 0.08736843869806095}, 
       {0.637368433434903, 0.07014187801138333}, {0.5589473890581718, 
       0.08758251145513224}, {0.4782479989097532, 0.13894738063711912}, 
       {0.46712431073033894, 0.1647368516066482}, {0.4637546564797764, 
       0.19052632257617727}, {0.46295053444271017, 0.21631579354570635}, 
       {0.4596191717177221, 0.24210526451523542}, {0.4576280123878442, 
       0.2678947354847645}, {0.45655584967175605, 0.2936842064542936}, 
       {0.45619208017879753, 0.3194736774238227}, {0.45609635136486115, 
       0.3452631483933518}, {0.45609635136486115, 0.3710526193628809}, 
       {0.4559048937369883, 0.39684209033241}, {0.45517735475107135, 
       0.42263156130193913}, {0.45364569372808833, 0.44842103227146823}, 
       {0.4508887038867188, 0.47421050324099734}, {0.44671492759909004, 
       0.49999997421052633}, {0.545152866969931, 0.031253043186359776}, 
       {0.7135302778027344, 0.06083600933634327}, {0.7767591594077525, 
       0.05583992896175311}, {0.30618502874039677, 0.0816136592873799}, 
       {0.4786117684027117, 0.1383177548810271}, {0.46819647344642706, 
       0.16068206173741556}, {0.46406098868437295, 0.1851115410737859}, 
       {0.46390782258207464, 0.2108506419828276}, {0.6657807454112383, 
       0.026445850538597215}, {0.7498689355730066, 0.024582158300564844}, 
       {0.8319659664048973, 0.02337327684886816}, {0.9108465090885234, 
       0.02256735588107038}, {0.9129525429951251, 0.022529578335704854}, 
       {0.9874965704074306, 0.021984952056685263}, {0.9930967060227123, 
       0.021962915155222043}, {1.0646827130843817, 0.02157884344400591}, 
       {1.07274307921783, 0.02155995467132315}, {1.1422804896612595, 
       0.02130810436888634}, {1.1520448286827765, 0.02127032682352082}, 
       {1.2200888696287975, 0.021106624126936896}, {1.2310593917059136, 
       0.02107514283913229}, {1.2980887072242084, 0.02096810646059665}, 
       {1.3098442055756037, 0.02095551394547481}, {1.3763182939730667, 
       0.020905143884987445}, {1.3885045719871758, 0.020876810725963306}, 
       {1.4545861722475002, 0.020854773824500086}, {1.466992626533663, 
       0.020854773824500086}, {0.42301247326842767, 0.042665010015527624}, 
       {0.8194063460164365, 0.05329309277836089}, {0.9098126378980098, 
       0.049351635545224856}, {0.9852852348054988, 0.047047205277928064}, 
       {0.9960451534919548, 0.04678276246036943}, {1.0587379537389288, 
       0.04541332644086928}, {1.079846157211914, 0.04501351408575084}, 
       {1.1333298455582024, 0.04415407492868524}, {1.1620963541461027, 
       0.04375426257356681}, {1.2088407339912661, 0.04319704377942537}, 
       {1.2433701171781397, 0.0428161201969897}, {1.285031297003278, 
       0.042463529773578174}, {0.31660032369668145, 0.07447370321329641}, 
       {0.2888772591806884, 0.09881503494381383}, {0.6124215045230668, 
       0.07447370321329641}, {0.27585814048533264, 0.1232193292499405}, 
       {0.273886126918242, 0.12953447558354347}, {0.5260932601151858, 
       0.10026317418282549}, {0.27061220148161574, 0.14728362564777742}, 
       {0.26984637097012426, 0.15665245689842666}, {0.4805263446814405, 
       0.13557258658446592}, {0.48852927352652686, 0.1260526451523546}, 
       {0.2697506421561878, 0.1727897650270651}, {0.27030586927701916, 
       0.1822908176864937}, {0.2720289879278751, 0.1993284906463437}, 
       {0.2729767031858458, 0.20720196072627436}, {0.27290969301609036, 
       0.22540758946367512}, {0.2726416523370684, 0.23310161620311956}, 
       {0.27229702860689714, 0.25099558019125473}, {0.2721438625045988, 
       0.2590547898692325}, {0.45894907002016705, 0.24920114678639244}, 
       {0.2719906964023005, 0.2766843110398091}, {0.2718758218255768, 
       0.28493240844461454}, {0.4571685140809492, 0.2755761697090871}, 
       {0.2718375303000022, 0.30242341194885086}, {0.27174180148606575, 
       0.31076595321707007}, {0.45640268356945773, 0.301617490981053}, 
       {0.2717226557232785, 0.3281751053730144}, {0.2716843641977039, 
       0.3365743129592819}, {0.45609635136486115, 0.3275077020715569}, 
       {0.2716843641977039, 0.3539519838274217}, {0.27158863538376743, 
       0.36239526521661564}, {0.45609635136486115, 0.353297173041086}, 
       {0.2715311980954056, 0.37969108473646346}, {0.27141632351868195, 
       0.38824140250419303}, {0.45609635136486115, 0.3790866440106151}, 
       {0.271224865890809, 0.40537981558501784}, {0.2710716997885107, 
       0.41414420610981867}, {0.45575172763468996, 0.4049894476162408}, 
       {0.27067921165137127, 0.43098984321406075}, {0.2704590353793175, 
       0.4401351573212972}, {0.45480401237671925, 0.43109058333503547}, 
       {0.26988466249569887, 0.45651801949481163}, {0.2695400387655276, 
       0.4662268486537506}, {0.45282242592823496, 0.45753171696211975}, 
       {0.26877420825403614, 0.4819423075258073}, {0.26816154384484286, 
       0.4924696501676658}, {0.44945277167767217, 0.48442932926237076}, 
       {0.267702045537948, 0.49999997421052633}, {0.5197368668698061, 
       0.032868033250735805}, {0.637368433434903, 0.027302141566882362}, 
       {0.7157894778116343, 0.02526215411714422}, {0.7942105221883655, 
       0.02387697745374178}, {0.8726315665650968, 0.022995501395212954}, 
       {0.8735122716533121, 0.02289476127423823}, {0.3891627646605025, 
       0.04868423224376732}, {0.3435575577011828, 0.06157896772853186}, 
       {0.3628947781163435, 0.055232340107124314}, {0.6765789556232686, 
       0.06470191147874826}, {0.7942105221883655, 0.054731787631031155}, 
       {0.8726315665650968, 0.05074940472374914}, {0.5595983449929396, 
       0.08736843869806095}, {0.5981579112465374, 0.07734479666107602}, 
       {0.2800127710101742, 0.11315790966759004}, {0.2844737337396122, 
       0.1051994401105869}, {0.5037310091796334, 0.11315790966759004}, 
       {0.5197368668698061, 0.1033861179330419}, {0.2717513743674594, 
       0.13894738063711912}, {0.2695974760538895, 0.1647368516066482}, 
       {0.2710716997885107, 0.19052632257617727}, {0.27312986928814414, 
       0.21631579354570635}, {0.27245019470919546, 0.24210526451523542}, 
       {0.2720289879278751, 0.2678947354847645}, {0.2718375303000022, 
       0.2936842064542936}, {0.2717226557232785, 0.3194736774238227}, 
       {0.2716843641977039, 0.3452631483933518}, {0.27156948962098015, 
       0.3710526193628809}, {0.27129187606056454, 0.39684209033241}, 
       {0.2709185336862124, 0.42263156130193913}, {0.2701909947002955, 
       0.44842103227146823}, {0.26913797774699455, 0.47421050324099734}, 
       {0.5309371381003696, 0.03210618608586446}, {0.3737312798539485, 
       0.052247914023248146}, {0.30951639146538484, 0.07913293380837735}, 
       {0.6035282977083718, 0.07623980345913453}, {0.5234894363761147, 
       0.10149724066476584}, {0.4809092599371863, 0.03591542191022118}, 
       {0.3346739237678812, 0.06519301956850004}, {0.6553654504549538, 
       0.06749744983579684}, {0.6607932742051499, 0.06677023208751057}, 
       {0.5592728670255557, 0.0874754750765966}, {0.4967715244064543, 
       0.11850028420803083}, {0.49266475828858103, 0.12206081785873119}, 
       {0.6765789556232686, 0.026219185266404092}, {0.7549999999999999, 
       0.02448141817959012}, {0.8334210443767311, 0.023398461879111845}, 
       {0.6495834300931926, 0.02691177359810531}, {0.7224904947871851, 
       0.025098451420560296}, {0.7970440950808841, 0.023826607393254415}, 
       {0.9118420887534624, 0.02259254091131406}, {0.9491380346630993, 
       0.022265135518146212}, {0.9902631331301937, 0.021988100185465723}, 
       {0.9531203533228552, 0.022214765457658846}, {1.0260657095424222, 
       0.021774027428394432}, {1.068684177506925, 0.02158513970156683}, 
       {1.0330156214342074, 0.021729953625467993}, {1.1034145912030653, 
       0.021421437004982904}, {1.1471052218836562, 0.02127662308108174}, 
       {1.1124130997130903, 0.021408844489861065}, {1.1810985237124858, 
       0.021179031088887475}, {1.2255262662603874, 0.02107514283913229}, 
       {1.1915999746013135, 0.021156994187424255}, {1.2590504969009286, 
       0.02102477277864493}, {1.3039473106371187, 0.02098069897571849}, 
       {1.2704805172849394, 0.02100588400596217}, {1.337165209073063, 
       0.020924032657670205}, {1.38236835501385, 0.02098069897571849}, 
       {1.349169602340693, 0.020917736400109285}, {1.4154139415847087, 
       0.020867366339621926}, {1.4607893993905816, 0.020854773824500086}, 
       {1.427782104345297, 0.020854773824500086}, {1.4937966944358663, 
       0.020854773824500086}, {0.9902631331301937, 0.046921280126709666}, 
       {0.9533118109507279, 0.04794127385157873}, {1.0218536417292186, 
       0.04617832173452109}, {1.068684177506925, 0.04515832800965201}, 
       {1.038165831623988, 0.04582573131110955}, {1.0958711606648737, 
       0.04473018249550943}, {1.1471052218836562, 0.04394944655795534}, 
       {1.121143567544094, 0.044327222011610545}, {1.1709225507910421, 
       0.04362204116478749}, {1.2255262662603874, 0.042942045348208106}, 
       {1.202819391594664, 0.04325685822625412}, {1.2468546460054262, 
       0.04280352768186786}, {1.3039473106371187, 0.0422872345618724}, 
       {1.2836528020825937, 0.042463529773578174}, {1.323782320884749, 
       0.042161309410654005}, {1.323322822577854, 0.042161309410654005}, 
       {1.38236835501385, 0.041733163896511424}, {1.3617292227291535, 
       0.041896866593095355}, {1.363816110872968, 0.041890570335534436}, 
       {1.4037733178100378, 0.041645016290658546}, {1.4002122059316022, 
       0.041657608805780386}, {1.4607893993905816, 0.04133020341261254}, 
       {1.438810063710775, 0.041456128563830935}, {1.443596504407597, 
       0.041443536048709095}, {1.4833813994795815, 0.0412546483218815}, 
       {1.477503650303884, 0.0412861296096861}, {0.6857593488797733, 
       0.025913816774699457}, {0.7082077557478681, 0.025388079268362625}, 
       {0.7595758373061617, 0.024399566831298153}, {0.791156773023793, 
       0.023899014355205}, {0.8347229562462668, 0.023322906788380803}, 
       {0.8725549835139477, 0.02291994630448191}, {0.951052610941828, 
       0.02223995048790253}, {1.0294736553185593, 0.021786619943516276}, 
       {1.1078946996952905, 0.021434029520104744}, {1.1863157440720218, 
       0.021182179217667935}, {1.264736788448753, 0.02103106903620585}, 
       {1.3431578328254843, 0.02098069897571849}, {1.4215788772022155, 
       0.020867366339621926}, {1.4999999215789475, 0.020854773824500086}, 
       {0.9491380346630993, 0.0480546064876753}, {0.951052610941828, 
       0.04797905139694426}, {1.0294736553185593, 0.0459642489774498}, 
       {1.1078946996952905, 0.044503517223316316}, {1.1863157440720218, 
       0.04345204221064264}, {1.264736788448753, 0.0426429731140644}, 
       {0.5981579112465374, 0.02871250326052848}, {0.7549999999999999, 
       0.057360475162715335}, {0.8334210443767311, 0.052562726901294154}, 
       {0.9118420887534624, 0.04918793284864094}, {0.2878050964646003, 
       0.10026317418282549}, {0.2871541405298325, 0.10114465024135433}, 
       {0.47137467006911693, 0.15184211612188364}, {0.46999617514843217, 
       0.15530505778038975}, {0.4647693819075026, 0.17763158709141275}, 
       {0.4642141547866712, 0.18299599853331672}, {0.4637546564797764, 
       0.2034210580609418}, {0.4640035513960111, 0.20885472833601593}, 
       {0.4610933954523433, 0.2292105290304709}, {0.4603467107036391, 
       0.23546900904602555}, {0.4602318361269153, 0.23588456204504626}, 
       {0.4584895717132721, 0.25499999999999995}, {0.458087510694739, 
       0.26051552162336605}, {0.45793434459244076, 0.2624295839218858}, 
       {0.4569770564530764, 0.28078947096952905}, {0.4568238903507781, 
       0.2858894395938745}, {0.45670901577405437, 0.2886220153753138}, 
       {0.45634524628109585, 0.30657894193905816}, {0.4562495174671594, 
       0.31149002283657595}, {0.4562112259415848, 0.3145751890414268}, 
       {0.45609635136486115, 0.33236841290858726}, {0.45609635136486115, 
       0.33722912374561764}, {0.45609635136486115, 0.34040243755632144}, 
       {0.45609635136486115, 0.35815788387811637}, {0.45609635136486115, 
       0.36301859471514675}, {0.45609635136486115, 0.36619190852585054}, 
       {0.4560580598392866, 0.3839473548476455}, {0.45602934119510563, 
       0.38878602878321267}, {0.45594318526256283, 0.392031749555867}, 
       {0.45563685305796625, 0.4097368258171746}, {0.45548368695566793, 
       0.41439605641225546}, {0.4553305208533696, 0.41802270076734555}, 
       {0.4545263988163035, 0.4355262967867037}, {0.45425835813728155, 
       0.4397825668978857}, {0.45395202593268497, 0.4442655022812609}, 
       {0.4524203649097019, 0.4613157677562328}, {0.45207574117953064, 
       0.46485426450546996}, {0.45134820219361377, 0.4709112642790751}, 
       {0.4490124191335646, 0.48710523872576184}, {0.44859121235224425, 
       0.4894978165989115}, {0.44705955132926123, 0.49811109694225025}, 
       {0.5778059654036503, 0.029587683061496388}, {0.5791270230359733, 
       0.02953101674344811}, {0.4413158224930749, 0.04017169202140322}, 
       {0.4181973139274247, 0.0433922277638139}, {0.4799519717978219, 
       0.03597838448583038}, {0.45104186998901713, 0.038987995599950226}, 
       {0.7198483795225392, 0.06024416112561677}, {0.7446038508065026, 
       0.0581600998729522}, {0.8098430375041861, 0.05382512654225865}, 
       {0.8783082852315278, 0.05055107261058015}, {0.2955782761562393, 
       0.09102026808339467}, {0.27493914387154283, 0.1260526451523546}, 
       {0.2792277947358953, 0.11488308423928217}, {0.2726033608114938, 
       0.1350437009493486}, {0.2701527031747209, 0.15184211612188364}, 
       {0.2710716997885107, 0.14335476092976324}, {0.26969320486782594, 
       0.1598761407696178}, {0.48666256165476623, 0.1280705957006295}, 
       {0.4776257616191663, 0.1399012636575985}, {0.4724851243107796, 
       0.14919768794629718}, {0.2699995370724226, 0.17763158709141275}, 
       {0.26969320486782594, 0.16959756244367857}, {0.27061220148161574, 
       0.18596783210207107}, {0.4660521480142508, 0.16949682232270386}, 
       {0.46543948360505766, 0.17267013613340765}, {0.27250763199755734, 
       0.2034210580609418}, {0.2715311980954056, 0.1947825926873593}, 
       {0.2732734625090488, 0.21263248287256803}, {0.46371636495420177, 
       0.1960544367146652}, {0.46371636495420177, 0.1978929439224539}, 
       {0.27275652691379204, 0.2292105290304709}, {0.2730628591183886, 
       0.22006836305201477}, {0.272517204878951, 0.23817325166844075}, 
       {0.46203153782892037, 0.22239797834955524}, {0.46191666325219666, 
       0.22309056668125649}, {0.2722012997929607, 0.25499999999999995}, 
       {0.272354465895259, 0.24609079555129793}, {0.2721438625045988, 
       0.26383994561553187}, {0.4590065073085289, 0.24792300650152566}, 
       {0.27189496758836407, 0.28078947096952905}, {0.2719906964023005, 
       0.2719998954144845}, {0.2718375303000022, 0.28952867646408625}, 
       {0.45732168018324754, 0.27315840680569375}, {0.27174180148606575, 
       0.30657894193905816}, {0.2718375303000022, 0.29783973644450096}, 
       {0.2717226557232785, 0.3152803698882498}, {0.45640268356945773, 
       0.2986456574122987}, {0.2716843641977039, 0.33236841290858726}, 
       {0.2717226557232785, 0.3236669849593956}, {0.2716843641977039, 
       0.3410572483426571}, {0.45609635136486115, 0.3243343882608531}, 
       {0.27158863538376743, 0.35815788387811637}, {0.2716843641977039, 
       0.3494690484440465}, {0.27156948962098015, 0.36680894176682066}, 
       {0.45609635136486115, 0.3501238592303822}, {0.2714354692814692, 
       0.3839473548476455}, {0.2715311980954056, 0.375308889474063}, 
       {0.27137803199310734, 0.3925354501607406}, {0.45609635136486115, 
       0.3759133301999113}, {0.2711291370768726, 0.4097368258171746}, 
       {0.2712631574163836, 0.401186508049445}, {0.27097597097457427, 
       0.41819269972149037}, {0.45579001916026457, 0.4016020610484657}, 
       {0.27061220148161574, 0.4355262967867037}, {0.27076536758391406, 
       0.427139681715558}, {0.2703441608025937, 0.4437743941915091}, 
       {0.4549858971231985, 0.4271270892004362}, {0.26969320486782594, 
       0.4613157677562328}, {0.2699995370724226, 0.4531810029875239}, 
       {0.2693868726632293, 0.46924905228299224}, {0.4533010699979171, 
       0.45236248950460434}, {0.2684678760494395, 0.48710523872576184}, 
       {0.26892737435633446, 0.4793230643804645}, {0.26804666926811915, 
       0.4945977852232568}, {0.4505249343937604, 0.47723900312779993}, 
       {0.5589473890581718, 0.030525825438073494}, {0.512346602433913, 
       0.03335914134048758}, {0.48201971417884903, 0.035789496759002774}, 
       {0.5001316057756233, 0.03427839494438193}, {0.6140106028344117, 
       0.028108062534680144}, {0.6225208943933613, 0.027777509012731835}, 
       {0.8727081496162459, 0.02291994630448191}, {0.8922368276592796, 
       0.022794021153263504}, {0.7157894778116343, 0.06062193657927199}, 
       {0.7713504814203436, 0.05620196377150602}, {0.7877009628406877, 
       0.05513159998614959}, {0.8437214647562921, 0.052071618811542375}, 
       {0.8653561767059272, 0.05107681011691699}, {0.9134503328275945, 
       0.04921311787888462}, {0.39716569350558895, 0.047059797793049904}, 
       {0.6837011793801397, 0.06392117554119417}, {0.9294753362805546, 
       0.04868423224376732}, {0.9314473498476452, 0.048583492122792594}, 
       {0.31916585591017793, 0.07298778642891923}, {0.6285613825527505, 
       0.07157742473527312}, {0.5402994161033534, 0.09413061931848923}, 
       {0.35286239841580463, 0.05827972876660968}, {0.5804002162613278, 
       0.08152865981030749}, {0.2807211642333038, 0.11192384318564969}, 
       {0.5090248125903185, 0.1096351535622552}}, 
       {{{EdgeForm[], RGBColor[0, 1, 0], Opacity[0.2], GraphicsGroup[
           {Polygon[{{198, 67, 65}, {51, 54, 53}, {49, 52, 51}, {15, 55, 16}, 
             {154, 108, 55}, {105, 54, 52}, {155, 117, 66}, {101, 50, 48}, 
             {183, 56, 6}, {63, 64, 13}, {103, 52, 50}, {14, 65, 15}, {162, 
             57, 7}, {165, 58, 8}, {177, 63, 13}, {65, 67, 15}, {195, 126, 
             79}, {24, 77, 23}, {153, 124, 77}, {125, 76, 27}, {152, 119, 
             68}, {158, 70, 4}, {197, 130, 83}, {128, 83, 30}, {196, 128, 
             81}, {124, 79, 26}, {129, 82, 31}, {156, 68, 2}, {126, 81, 28}, 
             {127, 80, 29}, {157, 69, 3}, {176, 62, 12}, {233, 66, 19}, {70, 
             120, 4}, {55, 108, 1}, {226, 121, 5}, {76, 123, 25}, {74, 122, 
             22}, {77, 124, 26}, {69, 118, 3}, {130, 85, 32}, {136, 91, 38}, 
             {68, 119, 17}, {139, 92, 41}, {105, 107, 54}, {106, 104, 53}, 
             {174, 61, 11}, {211, 152, 118}, {151, 116, 14}, {131, 84, 33}, 
             {133, 86, 35}, {47, 50, 49}, {168, 59, 9}, {171, 60, 10}, {66, 
             117, 14}, {61, 114, 11}, {62, 115, 12}, {58, 111, 8}, {60, 113, 
             10}, {56, 109, 6}, {59, 112, 9}, {57, 110, 7}, {227, 226, 183}, 
             {216, 75, 20}, {213, 73, 16}, {396, 272, 56}, {441, 239, 12}, 
             {219, 231, 4}, {435, 437, 176}, {436, 238, 11}, {427, 295, 170}, 
             {440, 442, 177}, {401, 276, 58}, {308, 527, 78}, {398, 274, 57}, 
             {474, 266, 196}, {472, 265, 195}, {533, 534, 202}, {306, 524, 
             76}, {424, 293, 167}, {193, 234, 192}, {238, 433, 11}, {451, 
             399, 109}, {206, 207, 2}, {262, 594, 212}, {240, 443, 13}, {586, 
             346, 108}, {192, 233, 19}, {528, 529, 201}, {430, 297, 173}, 
             {220, 232, 5}, {511, 465, 191}, {66, 233, 18}, {233, 234, 18}, 
             {404, 278, 59}, {407, 280, 60}, {410, 282, 61}, {118, 218, 3}, 
             {156, 218, 68}, {287, 512, 65}, {515, 514, 198}, {235, 513, 
             116}, {216, 217, 75}, {213, 214, 73}, {190, 213, 16}, {123, 74, 
             25}, {214, 213, 17}, {413, 284, 62}, {360, 608, 122}, {62, 176, 
             11}, {217, 216, 21}, {421, 291, 164}, {476, 267, 197}, {182, 
             232, 158}, {180, 231, 157}, {312, 535, 82}, {303, 521, 74}, 
             {310, 530, 80}, {517, 516, 199}, {191, 206, 2}, {216, 215, 21}, 
             {538, 539, 203}, {215, 216, 20}, {543, 544, 204}, {157, 219, 
             69}, {16, 215, 15}, {138, 93, 40}, {137, 90, 39}, {135, 88, 37}, 
             {132, 87, 34}, {110, 58, 7}, {111, 59, 8}, {67, 55, 15}, {113, 
             61, 10}, {112, 60, 9}, {114, 62, 11}, {80, 125, 27}, {199, 118, 
             69}, {222, 221, 73}, {190, 16, 1}, {193, 192, 22}, {225, 224, 
             75}, {223, 23, 19}, {215, 20, 15}, {115, 63, 12}, {22, 26, 25}, 
             {95, 44, 42}, {41, 44, 43}, {43, 46, 45}, {35, 38, 37}, {89, 38, 
             36}, {116, 65, 14}, {93, 42, 40}, {79, 28, 26}, {77, 26, 23}, 
             {39, 42, 41}, {25, 28, 27}, {37, 40, 39}, {91, 40, 38}, {228, 
             68, 17}, {72, 66, 18}, {14, 20, 19}, {184, 227, 183}, {218, 230, 
             3}, {226, 227, 71}, {190, 228, 17}, {158, 220, 70}, {68, 228, 
             2}, {121, 220, 5}, {199, 211, 118}, {209, 208, 5}, {120, 219, 
             4}, {182, 209, 5}, {208, 210, 56}, {120, 212, 69}, {228, 229, 
             2}, {191, 229, 190}, {178, 230, 156}, {223, 224, 24}, {23, 223, 
             24}, {81, 128, 30}, {416, 286, 63}, {79, 126, 28}, {75, 224, 
             20}, {20, 223, 19}, {73, 221, 16}, {121, 226, 71}, {183, 226, 
             5}, {224, 225, 24}, {221, 222, 21}, {215, 221, 21}, {87, 36, 
             34}, {454, 408, 112}, {29, 32, 31}, {81, 30, 28}, {36, 33, 34}, 
             {86, 33, 35}, {38, 35, 36}, {90, 37, 39}, {92, 39, 41}, {40, 37, 
             38}, {88, 35, 37}, {94, 41, 43}, {100, 47, 49}, {42, 39, 40}, 
             {50, 47, 48}, {44, 41, 42}, {102, 49, 51}, {48, 45, 46}, {97, 
             46, 44}, {99, 48, 46}, {143, 96, 45}, {148, 103, 50}, {140, 95, 
             42}, {134, 89, 36}, {141, 94, 43}, {45, 48, 47}, {149, 102, 51}, 
             {147, 100, 49}, {145, 98, 47}, {146, 101, 48}, {142, 97, 44}, 
             {144, 99, 46}, {150, 105, 52}, {98, 45, 47}, {34, 31, 32}, {96, 
             43, 45}, {74, 22, 25}, {26, 22, 23}, {32, 29, 30}, {76, 25, 27}, 
             {78, 77, 24}, {28, 25, 26}, {104, 51, 53}, {109, 57, 6}, {83, 
             32, 30}, {54, 51, 52}, {33, 36, 35}, {85, 34, 32}, {31, 34, 33}, 
             {80, 27, 29}, {30, 27, 28}, {224, 223, 20}, {82, 29, 31}, {66, 
             14, 19}, {84, 31, 33}, {46, 43, 44}, {52, 49, 50}, {220, 121, 
             70}, {20, 14, 15}, {219, 120, 69}, {192, 19, 23}, {221, 215, 
             16}, {218, 118, 68}, {55, 1, 16}, {229, 228, 190}, {27, 30, 29}, 
             {452, 402, 110}, {239, 438, 12}, {455, 411, 113}, {227, 184, 
             71}, {163, 185, 6}, {449, 450, 182}, {166, 186, 7}, {351, 592, 
             210}, {169, 187, 8}, {418, 458, 64}, {294, 426, 169}, {447, 448, 
             180}, {172, 188, 9}, {191, 190, 1}, {290, 420, 163}, {292, 423, 
             166}, {213, 190, 17}, {175, 189, 10}, {229, 191, 2}, {126, 202, 
             81}, {355, 386, 119}, {22, 192, 23}, {194, 193, 22}, {260, 585, 
             1}, {184, 183, 6}, {185, 184, 6}, {234, 193, 18}, {382, 363, 
             75}, {124, 201, 79}, {193, 200, 18}, {381, 359, 73}, {122, 194, 
             22}, {387, 244, 21}, {234, 233, 192}, {167, 165, 8}, {296, 429, 
             172}, {445, 446, 178}, {603, 241, 72}, {495, 496, 97}, {380, 
             299, 72}, {89, 136, 38}, {298, 432, 175}, {565, 330, 96}, {569, 
             333, 98}, {492, 493, 95}, {573, 336, 100}, {498, 499, 99}, {561, 
             327, 94}, {557, 324, 92}, {489, 490, 93}, {92, 137, 39}, {589, 
             590, 206}, {91, 138, 40}, {100, 145, 47}, {434, 431, 174}, {600, 
             355, 119}, {439, 435, 176}, {444, 440, 177}, {58, 165, 7}, {186, 
             164, 7}, {500, 256, 146}, {93, 140, 42}, {300, 520, 200}, {97, 
             144, 46}, {98, 143, 45}, {95, 142, 44}, {96, 141, 43}, {102, 
             147, 49}, {94, 139, 41}, {497, 255, 144}, {574, 375, 145}, {578, 
             376, 147}, {415, 457, 115}, {412, 456, 114}, {242, 263, 18}, 
             {491, 253, 140}, {522, 360, 122}, {599, 235, 116}, {409, 455, 
             113}, {403, 453, 111}, {180, 181, 4}, {231, 180, 4}, {178, 179, 
             3}, {406, 454, 112}, {400, 452, 110}, {482, 250, 134}, {550, 
             369, 133}, {362, 388, 24}, {554, 370, 135}, {63, 177, 12}, {189, 
             173, 10}, {541, 367, 129}, {536, 366, 127}, {174, 175, 10}, 
             {525, 364, 123}, {61, 174, 10}, {531, 365, 125}, {546, 368, 
             131}, {485, 251, 136}, {558, 371, 137}, {488, 252, 138}, {562, 
             372, 139}, {479, 249, 132}, {230, 178, 3}, {501, 502, 101}, 
             {171, 172, 9}, {187, 167, 8}, {281, 410, 61}, {393, 268, 159}, 
             {60, 171, 9}, {188, 170, 9}, {283, 413, 62}, {279, 407, 60}, 
             {232, 182, 5}, {494, 254, 142}, {506, 258, 150}, {503, 257, 
             148}, {582, 377, 149}, {385, 243, 17}, {208, 183, 5}, {285, 416, 
             63}, {168, 169, 8}, {277, 404, 59}, {170, 168, 9}, {397, 451, 
             109}, {519, 357, 121}, {518, 356, 120}, {358, 387, 21}, {165, 
             166, 7}, {566, 373, 141}, {82, 127, 29}, {570, 374, 143}, {273, 
             398, 57}, {271, 396, 56}, {394, 269, 160}, {395, 270, 161}, {59, 
             168, 8}, {275, 401, 58}, {173, 171, 10}, {453, 405, 111}, {86, 
             131, 33}, {509, 259, 107}, {371, 555, 137}, {373, 563, 141}, 
             {376, 575, 147}, {370, 551, 135}, {374, 567, 143}, {372, 559, 
             139}, {352, 599, 116}, {353, 606, 117}, {103, 150, 52}, {237, 
             600, 119}, {377, 579, 149}, {375, 571, 145}, {587, 588, 205}, 
             {345, 583, 106}, {328, 561, 94}, {323, 486, 91}, {322, 553, 90}, 
             {160, 157, 3}, {252, 560, 138}, {326, 489, 93}, {325, 557, 92}, 
             {118, 152, 68}, {117, 151, 14}, {230, 218, 156}, {253, 564, 
             140}, {84, 129, 31}, {78, 153, 77}, {299, 603, 72}, {369, 547, 
             133}, {357, 597, 121}, {598, 468, 71}, {364, 523, 123}, {596, 
             467, 70}, {367, 537, 129}, {467, 288, 70}, {468, 289, 71}, {608, 
             361, 122}, {365, 526, 125}, {456, 414, 114}, {314, 540, 84}, 
             {457, 417, 115}, {231, 219, 157}, {595, 262, 212}, {346, 378, 
             108}, {585, 510, 1}, {601, 598, 71}, {459, 602, 184}, {368, 542, 
             131}, {366, 532, 127}, {159, 156, 2}, {67, 154, 55}, {154, 205, 
             108}, {606, 354, 117}, {130, 204, 85}, {72, 155, 66}, {128, 203, 
             83}, {249, 548, 132}, {251, 556, 136}, {317, 480, 87}, {545, 
             315, 86}, {477, 478, 85}, {480, 481, 87}, {527, 307, 78}, {530, 
             309, 80}, {88, 133, 35}, {540, 313, 84}, {99, 146, 48}, {232, 
             220, 158}, {87, 134, 36}, {162, 163, 6}, {101, 148, 50}, {316, 
             545, 86}, {301, 381, 73}, {90, 135, 37}, {524, 305, 76}, {577, 
             339, 102}, {504, 505, 103}, {486, 487, 91}, {507, 508, 105}, 
             {581, 342, 104}, {553, 321, 90}, {483, 484, 89}, {549, 318, 88}, 
             {85, 132, 34}, {521, 302, 74}, {304, 382, 75}, {83, 130, 32}, 
             {389, 308, 78}, {161, 158, 4}, {255, 572, 144}, {535, 311, 82}, 
             {183, 208, 56}, {256, 576, 146}, {338, 501, 101}, {337, 573, 
             100}, {344, 507, 105}, {57, 162, 6}, {343, 581, 104}, {258, 584, 
             150}, {331, 565, 96}, {329, 492, 95}, {341, 504, 103}, {179, 
             160, 3}, {257, 580, 148}, {181, 161, 4}, {207, 159, 2}, {340, 
             577, 102}, {335, 498, 99}, {332, 495, 97}, {104, 149, 51}, {164, 
             162, 7}, {250, 552, 134}, {320, 483, 89}, {319, 549, 88}, {254, 
             568, 142}, {334, 569, 98}}], Polygon[{{363, 609, 225, 75}, {526, 
             306, 76, 125}, {269, 391, 157, 160}, {268, 390, 156, 159}, {270, 
             392, 158, 161}, {359, 607, 222, 73}, {466, 517, 199, 69}, {571, 
             334, 98, 145}, {542, 314, 84, 131}, {551, 319, 88, 135}, {579, 
             340, 102, 149}, {547, 316, 86, 133}, {555, 322, 90, 137}, {567, 
             331, 96, 143}, {559, 325, 92, 139}, {532, 310, 80, 127}, {523, 
             303, 74, 123}, {583, 343, 104, 106}, {563, 328, 94, 141}, {537, 
             312, 82, 129}, {575, 337, 100, 147}, {512, 515, 198, 65}, {502, 
             503, 148, 101}, {548, 317, 87, 132}, {297, 428, 171, 173}, {552, 
             320, 89, 134}, {576, 338, 101, 146}, {580, 341, 103, 148}, {293, 
             422, 165, 167}, {295, 425, 168, 170}, {584, 344, 105, 150}, 
             {417, 285, 63, 115}, {597, 596, 70, 121}, {514, 236, 67, 198}, 
             {379, 352, 116, 151}, {513, 287, 65, 116}, {572, 335, 99, 144}, 
             {414, 283, 62, 114}, {568, 332, 97, 142}, {556, 323, 91, 136}, 
             {473, 474, 196, 81}, {471, 472, 195, 79}, {291, 419, 162, 164}, 
             {422, 292, 166, 165}, {419, 290, 163, 162}, {475, 476, 197, 83}, 
             {286, 418, 64, 63}, {470, 469, 193, 194}, {560, 326, 93, 138}, 
             {347, 393, 159, 207}, {378, 260, 1, 108}, {244, 605, 217, 21}, 
             {243, 604, 214, 17}, {564, 329, 95, 140}, {399, 273, 57, 109}, 
             {402, 275, 58, 110}, {411, 281, 61, 113}, {462, 424, 167, 187}, 
             {463, 427, 170, 188}, {461, 421, 164, 186}, {274, 400, 110, 57}, 
             {460, 459, 184, 185}, {464, 430, 173, 189}, {386, 385, 17, 119}, 
             {261, 237, 119, 152}, {266, 247, 128, 196}, {265, 246, 126, 
             195}, {264, 245, 124, 153}, {267, 248, 130, 197}, {384, 353, 
             117, 155}, {272, 397, 109, 56}, {276, 403, 111, 58}, {278, 406, 
             112, 59}, {284, 415, 115, 62}, {350, 591, 208, 209}, {349, 395, 
             161, 181}, {348, 394, 160, 179}, {408, 279, 60, 112}, {405, 277, 
             59, 111}, {263, 380, 72, 18}, {336, 574, 145, 100}, {307, 264, 
             153, 78}, {241, 384, 155, 72}, {282, 412, 114, 61}, {280, 409, 
             113, 60}, {388, 389, 78, 24}, {354, 379, 151, 117}, {593, 261, 
             152, 211}, {236, 383, 154, 67}, {333, 570, 143, 98}, {342, 582, 
             149, 104}, {339, 578, 147, 102}, {520, 242, 18, 200}, {302, 522, 
             122, 74}, {245, 528, 201, 124}, {313, 541, 129, 84}, {309, 531, 
             125, 80}, {305, 525, 123, 76}, {529, 471, 79, 201}, {442, 441, 
             12, 177}, {446, 348, 179, 178}, {390, 445, 178, 156}, {443, 444, 
             177, 13}, {448, 349, 181, 180}, {438, 439, 176, 12}, {247, 538, 
             203, 128}, {539, 475, 83, 203}, {311, 536, 127, 82}, {469, 300, 
             200, 193}, {493, 494, 142, 95}, {499, 500, 146, 99}, {510, 511, 
             191, 1}, {508, 509, 107, 105}, {496, 497, 144, 97}, {490, 491, 
             140, 93}, {437, 436, 11, 176}, {478, 479, 132, 85}, {484, 485, 
             136, 89}, {534, 473, 81, 202}, {246, 533, 202, 126}, {289, 519, 
             121, 71}, {288, 518, 120, 70}, {487, 488, 138, 91}, {481, 482, 
             134, 87}, {505, 506, 150, 103}, {425, 294, 169, 168}, {433, 434, 
             174, 11}, {450, 350, 209, 182}, {604, 301, 73, 214}, {590, 347, 
             207, 206}, {465, 589, 206, 191}, {591, 351, 210, 208}, {605, 
             304, 75, 217}, {607, 358, 21, 222}, {315, 546, 131, 86}, {330, 
             566, 141, 96}, {318, 550, 133, 88}, {321, 554, 135, 90}, {327, 
             562, 139, 94}, {324, 558, 137, 92}, {383, 587, 205, 154}, {588, 
             586, 108, 205}, {592, 271, 56, 210}, {516, 593, 211, 199}, {429, 
             463, 188, 172}, {432, 464, 189, 175}, {392, 449, 182, 158}, 
             {391, 447, 180, 157}, {431, 298, 175, 174}, {361, 470, 194, 
             122}, {428, 296, 172, 171}, {426, 462, 187, 169}, {420, 460, 
             185, 163}, {594, 466, 69, 212}, {356, 595, 212, 120}, {248, 543, 
             204, 130}, {544, 477, 85, 204}, {602, 601, 71, 184}, {423, 461, 
             186, 166}, {609, 362, 24, 225}}]}]}, {}, {}, {}, {}}, 
        {{RGBColor[0, 2/3, 0], Dashing[{Small, Small}], Line[{240, 13, 64, 
           458, 418, 286, 416, 285, 417, 457, 415, 284, 413, 283, 414, 456, 
           412, 282, 410, 281, 411, 455, 409, 280, 407, 279, 408, 454, 406, 
           278, 404, 277, 405, 453, 403, 276, 401, 275, 402, 452, 400, 274, 
           398, 273, 399, 451, 397, 272, 396, 271, 592, 351, 591, 350, 450, 
           449, 392, 270, 395, 349, 448, 447, 391, 269, 394, 348, 446, 445, 
           390, 268, 393, 347, 590, 589, 465, 511, 510, 585, 260, 378, 346, 
           586, 588, 587, 383, 236, 514, 515, 512, 287, 513, 235, 599, 352, 
           379, 354, 606, 353, 384, 241, 603, 299, 380, 263, 242, 520, 300, 
           469, 470, 361, 608, 360, 522, 302, 521, 303, 523, 364, 525, 305, 
           524, 306, 526, 365, 531, 309, 530, 310, 532, 366, 536, 311, 535, 
           312, 537, 367, 541, 313, 540, 314, 542, 368, 546, 315, 545, 316, 
           547, 369, 550, 318, 549, 319, 551, 370, 554, 321, 553, 322, 555, 
           371, 558, 324, 557, 325, 559, 372, 562, 327, 561, 328, 563, 373, 
           566, 330, 565, 331, 567, 374, 570, 333, 569, 334, 571, 375, 574, 
           336, 573, 337, 575, 376, 578, 339, 577, 340, 579, 377, 582, 342, 
           581, 343, 583, 345, 106, 53, 54, 107, 259, 509, 508, 507, 344, 
           584, 258, 506, 505, 504, 341, 580, 257, 503, 502, 501, 338, 576, 
           256, 500, 499, 498, 335, 572, 255, 497, 496, 495, 332, 568, 254, 
           494, 493, 492, 329, 564, 253, 491, 490, 489, 326, 560, 252, 488, 
           487, 486, 323, 556, 251, 485, 484, 483, 320, 552, 250, 482, 481, 
           480, 317, 548, 249, 479, 478, 477, 544, 543, 248, 267, 476, 475, 
           539, 538, 247, 266, 474, 473, 534, 533, 246, 265, 472, 471, 529, 
           528, 245, 264, 307, 527, 308, 389, 388, 362, 609, 363, 382, 304, 
           605, 244, 387, 358, 607, 359, 381, 301, 604, 243, 385, 386, 355, 
           600, 237, 261, 593, 516, 517, 466, 594, 262, 595, 356, 518, 288, 
           467, 596, 597, 357, 519, 289, 468, 598, 601, 602, 459, 460, 420, 
           290, 419, 291, 421, 461, 423, 292, 422, 293, 424, 462, 426, 294, 
           425, 295, 427, 463, 429, 296, 428, 297, 430, 464, 432, 298, 431, 
           434, 433, 238, 436, 437, 435, 439, 438, 239, 441, 442, 440, 444, 
           443, 240}]}}}], GraphicsComplex[{{0.7157894778116343, 
       0.035789496759002774}, {0.7942105221883655, 0.035789496759002774}, 
       {0.8726315665650968, 0.035789496759002774}, {0.951052610941828, 
       0.035789496759002774}, {1.0294736553185593, 0.035789496759002774}, 
       {1.1078946996952905, 0.035789496759002774}, {1.1863157440720218, 
       0.035789496759002774}, {1.264736788448753, 0.035789496759002774}, 
       {1.3431578328254843, 0.035789496759002774}, {1.4215788772022155, 
       0.035789496759002774}, {1.4999999215789475, 0.035789496759002774}, 
       {0.4805263446814405, 0.06157896772853186}, {0.5589473890581718, 
       0.06157896772853186}, {0.4021053003047092, 0.08736843869806095}, 
       {0.4805263446814405, 0.08736843869806095}, {0.4021053003047092, 
       0.11315790966759004}, {0.4021053003047092, 0.13894738063711912}, 
       {0.4021053003047092, 0.1647368516066482}, {0.4021053003047092, 
       0.19052632257617727}, {0.4021053003047092, 0.21631579354570635}, 
       {0.4021053003047092, 0.24210526451523542}, {0.4021053003047092, 
       0.2678947354847645}, {0.4021053003047092, 0.2936842064542936}, 
       {0.4021053003047092, 0.3194736774238227}, {0.4021053003047092, 
       0.3452631483933518}, {0.4021053003047092, 0.3710526193628809}, 
       {0.4021053003047092, 0.39684209033241}, {0.4021053003047092, 
       0.42263156130193913}, {0.3236842559279779, 0.44842103227146823}, 
       {0.4021053003047092, 0.44842103227146823}, {0.3236842559279779, 
       0.47421050324099734}, {0.4021053003047092, 0.47421050324099734}, 
       {0.3236842559279779, 0.49999997421052633}, {0.4021053003047092, 
       0.49999997421052633}, {0.6765789556232686, 0.04868423224376732}, 
       {0.5197368668698061, 0.04868423224376732}, {0.4413158224930749, 
       0.07447370321329641}, {0.5981579112465374, 0.04868423224376732}, 
       {0.4021053003047092, 0.07447370321329641}, {0.3628947781163435, 
       0.10026317418282549}, {0.5197368668698061, 0.07447370321329641}, 
       {0.3628947781163435, 0.1260526451523546}, {0.4413158224930749, 
       0.10026317418282549}, {0.3628947781163435, 0.15184211612188364}, 
       {0.3628947781163435, 0.17763158709141275}, {0.3628947781163435, 
       0.2034210580609418}, {0.3628947781163435, 0.2292105290304709}, 
       {0.3628947781163435, 0.25499999999999995}, {0.3628947781163435, 
       0.28078947096952905}, {0.3628947781163435, 0.30657894193905816}, 
       {0.3628947781163435, 0.33236841290858726}, {0.3628947781163435, 
       0.35815788387811637}, {0.3628947781163435, 0.3839473548476455}, 
       {0.3628947781163435, 0.4097368258171746}, {0.3628947781163435, 
       0.4355262967867037}, {0.6765789556232686, 0.035789496759002774}, 
       {0.4413158224930749, 0.06157896772853186}, {0.5589473890581718, 
       0.04868423224376732}, {0.5981579112465374, 0.06157896772853186}, 
       {0.7157894778116343, 0.04868423224376732}, {0.3628947781163435, 
       0.11315790966759004}, {0.4413158224930749, 0.11315790966759004}, 
       {0.3628947781163435, 0.13894738063711912}, {0.3628947781163435, 
       0.1647368516066482}, {0.3628947781163435, 0.19052632257617727}, 
       {0.3628947781163435, 0.21631579354570635}, {0.3628947781163435, 
       0.24210526451523542}, {0.3628947781163435, 0.2678947354847645}, 
       {0.3628947781163435, 0.2936842064542936}, {0.3628947781163435, 
       0.3194736774238227}, {0.3628947781163435, 0.3452631483933518}, 
       {0.3628947781163435, 0.3710526193628809}, {0.3628947781163435, 
       0.39684209033241}, {0.3628947781163435, 0.42263156130193913}, 
       {0.4609210835872577, 0.05513159998614959}, {0.38250003921052633, 
       0.08092107095567869}, {0.42171056139889207, 0.06802633547091413}, 
       {0.3432895170221607, 0.42907892904432143}, {0.7549999999999999, 
       0.035789496759002774}, {0.8334210443767311, 0.035789496759002774}, 
       {0.9118420887534624, 0.035789496759002774}, {0.9902631331301937, 
       0.035789496759002774}, {1.068684177506925, 0.035789496759002774}, 
       {1.1471052218836562, 0.035789496759002774}, {1.2255262662603874, 
       0.035789496759002774}, {1.3039473106371187, 0.035789496759002774}, 
       {1.38236835501385, 0.035789496759002774}, {1.4607893993905816, 
       0.035789496759002774}, {0.637368433434903, 0.04868423224376732}, 
       {0.6177631723407202, 0.05513159998614959}, {0.6569736945290858, 
       0.042236864501385044}, {0.8922368276592796, 0.0293421290166205}, 
       {0.9706578720360108, 0.0293421290166205}, {1.049078916412742, 
       0.0293421290166205}, {1.1274999607894733, 0.0293421290166205}, 
       {1.2059210051662046, 0.0293421290166205}, {1.2843420495429358, 
       0.0293421290166205}, {1.362763093919667, 0.0293421290166205}, 
       {1.4411841382963986, 0.0293421290166205}, {1.4803946604847646, 
       0.0293421290166205}, {0.7353947389058171, 0.042236864501385044}, 
       {0.7746052610941827, 0.042236864501385044}, {0.8138157832825483, 
       0.042236864501385044}, {0.853026305470914, 0.042236864501385044}, 
       {0.8922368276592796, 0.042236864501385044}, {0.4021053003047092, 
       0.1260526451523546}, {0.42171056139889207, 0.13250001289473684}, 
       {0.4021053003047092, 0.15184211612188364}, {0.42171056139889207, 
       0.15828948386426592}, {0.4021053003047092, 0.17763158709141275}, 
       {0.4021053003047092, 0.2034210580609418}, {0.42171056139889207, 
       0.20986842580332407}, {0.4021053003047092, 0.2292105290304709}, 
       {0.4021053003047092, 0.25499999999999995}, {0.4021053003047092, 
       0.28078947096952905}, {0.4021053003047092, 0.30657894193905816}, 
       {0.4021053003047092, 0.33236841290858726}, {0.4021053003047092, 
       0.35815788387811637}, {0.4021053003047092, 0.3839473548476455}, 
       {0.4021053003047092, 0.4097368258171746}, {0.4021053003047092, 
       0.4355262967867037}, {0.9314473498476452, 0.0293421290166205}, 
       {0.951052610941828, 0.0293421290166205}, {1.0098683942243765, 
       0.0293421290166205}, {1.0294736553185593, 0.0293421290166205}, 
       {1.0882894386011077, 0.0293421290166205}, {1.1078946996952905, 
       0.0293421290166205}, {1.166710482977839, 0.0293421290166205}, 
       {1.1863157440720218, 0.0293421290166205}, {1.2451315273545702, 
       0.0293421290166205}, {1.264736788448753, 0.0293421290166205}, 
       {1.3235525717313015, 0.0293421290166205}, {1.3431578328254843, 
       0.0293421290166205}, {1.4019736161080327, 0.0293421290166205}, 
       {1.4215788772022155, 0.0293421290166205}, {0.42171056139889207, 
       0.11960527740997232}, {0.42171056139889207, 0.1453947483795014}, 
       {0.42171056139889207, 0.17118421934903047}, {0.7942105221883655, 
       0.042236864501385044}, {0.8726315665650968, 0.042236864501385044}, 
       {0.4021053003047092, 0.10026317418282549}, {0.38250003921052633, 
       0.09381580644044321}, {0.38250003921052633, 0.08736843869806095}, 
       {0.5197368668698061, 0.06157896772853186}, {0.539342127963989, 
       0.06802633547091413}, {0.5589473890581718, 0.06802633547091413}, 
       {0.4413158224930749, 0.08736843869806095}, {0.4609210835872577, 
       0.09381580644044321}, {0.4805263446814405, 0.09381580644044321}, 
       {0.7746052610941827, 0.035789496759002774}, {0.853026305470914, 
       0.035789496759002774}, {0.9314473498476452, 0.035789496759002774}, 
       {1.0098683942243765, 0.035789496759002774}, {1.0882894386011077, 
       0.035789496759002774}, {1.166710482977839, 0.035789496759002774}, 
       {1.2451315273545702, 0.035789496759002774}, {1.3235525717313015, 
       0.035789496759002774}, {1.4019736161080327, 0.035789496759002774}, 
       {1.4999999215789475, 0.0293421290166205}, {1.4803946604847646, 
       0.035789496759002774}, {0.3628947781163435, 0.4613157677562328}, 
       {0.3236842559279779, 0.4613157677562328}, {0.3628947781163435, 
       0.48710523872576184}, {0.3236842559279779, 0.48710523872576184}, 
       {0.6569736945290858, 0.05513159998614959}, {0.5785526501523546, 
       0.042236864501385044}, {0.6177631723407202, 0.042236864501385044}, 
       {0.3432895170221607, 0.11960527740997232}, {0.3432895170221607, 
       0.13250001289473684}, {0.4609210835872577, 0.10026317418282549}, 
       {0.42171056139889207, 0.1260526451523546}, {0.3432895170221607, 
       0.1453947483795014}, {0.3432895170221607, 0.15828948386426592}, 
       {0.42171056139889207, 0.15184211612188364}, {0.3432895170221607, 
       0.17118421934903047}, {0.3432895170221607, 0.184078954833795}, 
       {0.3432895170221607, 0.19697369031855955}, {0.3432895170221607, 
       0.20986842580332407}, {0.42171056139889207, 0.2034210580609418}, 
       {0.3432895170221607, 0.22276316128808862}, {0.3432895170221607, 
       0.23565789677285315}, {0.3432895170221607, 0.2485526322576177}, 
       {0.3432895170221607, 0.2614473677423822}, {0.3432895170221607, 
       0.2743421032271468}, {0.3432895170221607, 0.2872368387119113}, 
       {0.3432895170221607, 0.3001315741966759}, {0.3432895170221607, 
       0.3130263096814404}, {0.3432895170221607, 0.325921045166205}, 
       {0.3432895170221607, 0.3388157806509695}, {0.3432895170221607, 
       0.3517105161357341}, {0.3432895170221607, 0.3646052516204986}, 
       {0.3432895170221607, 0.3774999871052632}, {0.3432895170221607, 
       0.3903947225900277}, {0.3432895170221607, 0.40328945807479233}, 
       {0.3432895170221607, 0.4161841935595568}, {0.3628947781163435, 
       0.44842103227146823}, {0.3432895170221607, 0.44197366452908593}, 
       {0.3432895170221607, 0.4355262967867037}, {0.4021053003047092, 
       0.4613157677562328}, {0.4021053003047092, 0.48710523872576184}, 
       {0.6569736945290858, 0.035789496759002774}, {0.5001316057756233, 
       0.05513159998614959}, {0.4805263446814405, 0.05513159998614959}, 
       {0.5001316057756233, 0.04868423224376732}, {0.3628947781163435, 
       0.09381580644044321}, {0.4805263446814405, 0.07447370321329641}, 
       {0.5001316057756233, 0.08092107095567869}, {0.3432895170221607, 
       0.11315790966759004}, {0.3432895170221607, 0.13894738063711912}, 
       {0.42171056139889207, 0.13894738063711912}, {0.3432895170221607, 
       0.1647368516066482}, {0.42171056139889207, 0.1647368516066482}, 
       {0.3432895170221607, 0.19052632257617727}, {0.3432895170221607, 
       0.21631579354570635}, {0.3432895170221607, 0.24210526451523542}, 
       {0.3432895170221607, 0.2678947354847645}, {0.3432895170221607, 
       0.2936842064542936}, {0.3432895170221607, 0.3194736774238227}, 
       {0.3432895170221607, 0.3452631483933518}, {0.3432895170221607, 
       0.3710526193628809}, {0.3432895170221607, 0.39684209033241}, 
       {0.3432895170221607, 0.42263156130193913}, {0.3432895170221607, 
       0.45486840001385054}, {0.5001316057756233, 0.06802633547091413}, 
       {0.5197368668698061, 0.06802633547091413}, {0.42171056139889207, 
       0.09381580644044321}, {0.4413158224930749, 0.09381580644044321}, 
       {0.3628947781163435, 0.47421050324099734}, {0.3432895170221607, 
       0.4806578709833796}, {0.38250003921052633, 0.44197366452908593}, 
       {0.3628947781163435, 0.44197366452908593}, {0.5589473890581718, 
       0.0418213115023643}, {0.637368433434903, 0.03649467760582584}, 
       {0.6057396333103036, 0.06157896772853186}, {0.951052610941828, 
       0.04112872317066309}, {1.0294736553185593, 0.03964280638628592}, 
       {1.1078946996952905, 0.03850948002532029}, {1.1863157440720218, 
       0.03770355905752251}, {1.264736788448753, 0.037099118331674175}, 
       {1.3431578328254843, 0.036645787787287915}, {1.4215788772022155, 
       0.03629319736387639}, {1.4999999215789475, 0.0360161620311959}, 
       {0.4021053003047092, 0.0705448384952822}, {0.4514439310075502, 
       0.11315790966759004}, {0.32320561185829566, 0.44842103227146823}, 
       {0.3215016389702271, 0.47421050324099734}, {0.31920414743575254, 
       0.49999997421052633}, {0.7085140879524647, 0.0333969188858531}, 
       {0.7805021560326675, 0.031281376345383916}, {0.8541750512381512, 
       0.029719904470275713}, {0.6284082164504523, 0.05863231919002121}, 
       {0.32320561185829566, 0.4482636258324452}, {0.321530357614408, 
       0.47350217426539387}, {0.31935731353805086, 0.4985770200017584}, 
       {0.892926075119622, 0.029115463744427375}, {0.974525316119043, 
       0.028070284989314624}, {1.055128977453525, 0.02735251162736972}, 
       {1.1350816828532393, 0.02684881102249611}, {1.2146706187599947, 
       0.026464739311279975}, {1.293857493648218, 0.026212889008843172}, 
       {1.3727954736202057, 0.02604289005469832}, {1.4516185790154705, 
       0.025910668645918997}, {1.4999999215789475, 0.025866594842992557}, 
       {0.5132273075221283, 0.04654350467305446}, {0.5331389008209075, 
       0.044276851951123186}, {0.753946983046699, 0.04833793807791671}, 
       {0.7564933694974083, 0.04819312415401554}, {0.8224696680624024, 
       0.045082772918920974}, {0.8471677020580037, 0.04416351931502663}, 
       {0.8935387395288152, 0.042665010015527624}, {0.3922643782320432, 
       0.07447370321329641}, {0.35500672384798093, 0.09766911606772638}, 
       {0.34750158483536403, 0.10532536526180533}, {0.4692686361625152, 
       0.10026317418282549}, {0.43966928689336804, 0.12551116700211543}, 
       {0.4385971241772799, 0.12694671372600527}, {0.4274542902350784, 
       0.14728362564777742}, {0.4243526766635378, 0.15742060032085894}, 
       {0.42194031055233955, 0.17125977443976154}, {0.4223327986894789, 
       0.20966379743259414}, {0.3236842559279779, 0.4392536812627684}, 
       {0.32391400508142537, 0.4355262967867037}, {0.6765789556232686, 
       0.034681355428280825}, {0.951052610941828, 0.028328431549312354}, 
       {1.0294736553185593, 0.02762954696005021}, {1.1078946996952905, 
       0.027025106234201873}, {1.1863157440720218, 0.026622145750302983}, 
       {1.264736788448753, 0.02629474035713513}, {1.3431578328254843, 
       0.026093260115185687}, {1.4215788772022155, 0.026017705024454642}, 
       {0.4805263446814405, 0.051202735268135395}, {0.4968385345762098, 
       0.04868423224376732}, {0.4302112800764479, 0.06157896772853186}, 
       {0.4413158224930749, 0.05885898446221434}, {0.5981579112465374, 
       0.06263673899876646}, {0.7157894778116343, 0.0507053309208227}, 
       {0.7478777762431288, 0.04868423224376732}, {0.3628947781163435, 
       0.09114619323461307}, {0.4413158224930749, 0.12348377206749916}, 
       {0.4311302766902377, 0.13894738063711912}, {0.42285930716612935, 
       0.1647368516066482}, {0.6806378573341736, 0.034454690156087694}, 
       {0.45992550392231873, 0.054804194592981734}, {0.4646736530935662, 
       0.05389753350420923}, {0.38031742225277554, 0.08020329759373379}, 
       {0.37406633070272605, 0.08369457241126402}, {0.5272611516452104, 
       0.07694813243473804}, {0.45992550392231873, 0.1063831365320399}, 
       {0.45835555137376105, 0.10755424043837108}, {0.4153541681535125, 
       0.06593597796068862}, {0.574129978948491, 0.06657189997434156}, 
       {0.5920121213918179, 0.06360006640558724}, {0.4890270633589963, 
       0.0901639770551095}, {0.3244117949138948, 0.42287081908925406}, 
       {0.32391400508142537, 0.4354507416959726}, {0.7549999999999999, 
       0.03193618713171961}, {0.7549999999999999, 0.04828756801742935}, 
       {0.8334210443767311, 0.030122864954174607}, {0.8334210443767311, 
       0.04466721991990023}, {0.9118420887534624, 0.028838428411746886}, 
       {0.9118420887534624, 0.04213612438041032}, {0.9902631331301937, 
       0.0279065822927307}, {0.9902631331301937, 0.040322802202865306}, 
       {1.068684177506925, 0.027276956536638683}, {1.068684177506925, 
       0.039038365660437585}, {1.1471052218836562, 0.02682362599225243}, 
       {1.1471052218836562, 0.03805614948093404}, {1.2255262662603874, 
       0.0264710355688409}, {1.2255262662603874, 0.03730059857362362}, 
       {1.3039473106371187, 0.026219185266404092}, {1.3039473106371187, 
       0.036847268029237365}, {1.38236835501385, 0.026017705024454642}, 
       {1.38236835501385, 0.03644430754533848}, {1.4607893993905816, 
       0.025904372388358077}, {1.4607893993905816, 0.03609171712192694}, 
       {0.637368433434903, 0.057599732950030305}, {0.724749694796085, 
       0.03284284822049212}, {0.7442017897879696, 0.03223840749464378}, 
       {0.6391681351369081, 0.036381344969729265}, {0.8100249222506652, 
       0.0305887880136827}, {0.8171471460075366, 0.030437677832220615}, 
       {0.8915475801989372, 0.029115463744427375}, {0.9670584686320007, 
       0.02815843259516751}, {1.043335187576556, 0.027453251748344447}, 
       {1.1201096963535804, 0.02691177359810531}, {1.197420286488649, 
       0.02654659065957194}, {1.2749797715399525, 0.02626325906933053}, 
       {1.3528838803214267, 0.026093260115185687}, {1.4308454263912629, 
       0.025942149933723603}, {1.4699027824773307, 0.025891779873236237}, 
       {1.4909822673061348, 0.025860298585431638}, {0.7878541289429859, 
       0.04659387473354182}, {0.8025963662891975, 0.04592647143208428}, 
       {0.8576978715910122, 0.04377315134624957}, {0.8906668751107221, 
       0.0427531576213805}, {0.9333619261263739, 0.041607238745293026}, 
       {0.9298008142479386, 0.041695386351145905}, {0.9664458042228075, 
       0.0408516878379826}, {0.9754826042584075, 0.04065020759603316}, 
       {1.0170480552696093, 0.03987576791603997}, {1.0033588348766984, 
       0.04009613693067218}, {1.04069307231191, 0.039479103689702005}, 
       {1.0583454656017892, 0.039189475841899676}, {1.0992408149154365, 
       0.0386354051765387}, {1.0782187673749943, 0.03892503302434103}, 
       {1.1159359200659513, 0.03843392493458925}, {1.1398681235500614, 
       0.0381694821170306}, {1.1803039745568131, 0.03776652163313171}, 
       {1.1538828219103563, 0.03801837193556852}, {1.1920020356198462, 
       0.03765948525459607}, {1.220586659461267, 0.03741393120972018}, 
       {1.2606778867378479, 0.037124303361917854}, {1.2301978323804859, 
       0.037325783603867305}, {1.2686425240573596, 0.037073933301430495}, 
       {1.3006542394377054, 0.036872453059481045}, {1.3405157175608384, 
       0.036658380302409754}, {1.3070872157342337, 0.036822082998993685}, 
       {1.3456850735134065, 0.036620602757044235}, {1.3803006126328228, 
       0.03646949257558216}, {1.4200089246536578, 0.036305789878998226}, 
       {1.3843786601065151, 0.0364506038028994}, {1.4231201111065923, 
       0.03629634549265685}, {1.4596789451489187, 0.03615467969753615}, 
       {1.4993106741186053, 0.0360161620311959}, {1.4618807078694571, 
       0.03614838343997523}, {0.43262364618764615, 0.13608887970446135}, 
       {0.42393146988221747, 0.15901984974133265}, {0.42144252071987, 
       0.17763158709141275}, {0.421174480040848, 0.18425525004550075}, 
       {0.421174480040848, 0.18390265962208924}, {0.4223423715708726, 
       0.21007620230283447}, {0.42010231732475983, 0.2292105290304709}, 
       {0.41948965291556667, 0.2363882626499199}, {0.4196045274922904, 
       0.23496530844115196}, {0.4181111579948819, 0.25499999999999995}, 
       {0.4177665342647108, 0.2627443967999318}, {0.4179005546042217, 
       0.26019441248775915}, {0.4170389952787938, 0.28078947096952905}, 
       {0.416847537650921, 0.28883608813238504}, {0.4168858291764955, 
       0.28565018180655943}, {0.4165124868021434, 0.30657894193905816}, 
       {0.416388039344026, 0.3147766692833762}, {0.4164263308696006, 
       0.3112885425946264}, {0.4162157274789404, 0.33236841290858726}, 
       {0.416119998665004, 0.34065428785875823}, {0.416119998665004, 
       0.3369772734431808}, {0.4159668325627057, 0.35815788387811637}, 
       {0.4158136664604074, 0.36654449894926205}, {0.4159093952743439, 
       0.3626974855795398}, {0.4154690427302362, 0.3839473548476455}, 
       {0.4152010020512142, 0.3925354501607406}, {0.4153541681535125, 
       0.3883043650798022}, {0.4145213274722655, 0.4097368258171746}, 
       {0.41397567323282775, 0.4187278816141686}, {0.4142820054374244, 
       0.4137412456259198}, {0.4127503444144413, 0.4355262967867037}, 
       {0.4118313478006515, 0.44522253343052076}, {0.4124440122098447, 
       0.4389262758696006}, {0.7157894778116343, 0.03314506858341629}, 
       {0.7677893695419082, 0.031583596708308084}, {0.7942105221883655, 
       0.030941378437094227}, {0.8517243936013783, 0.02977027453076307}, 
       {0.8726315665650968, 0.029442869137595223}, {0.8766904682760017, 
       0.0293421290166205}, {0.9292264413643199, 0.028611763139553763}, 
       {0.9339075803658117, 0.028533059920042257}, {1.0050819535275546, 
       0.027768064626390455}, {1.0149420213630074, 0.02767362076297665}, 
       {1.081665004676706, 0.027163623900542118}, {1.0952202047301058, 
       0.027062883779567393}, {1.158707554132753, 0.026710293356155865}, 
       {1.1749048694507978, 0.026647330780546666}, {1.2361713103701195, 
       0.026395480478109856}, {1.2542449104413191, 0.026345110417622497}, 
       {1.3138839615237212, 0.026162518948355806}, {1.3333647751597864, 
       0.026115297016648907}, {1.3918263618307702, 0.026005112509332802}, 
       {1.4122453178434127, 0.025964186835186823}, {0.4292348461742962, 
       0.14292031915805975}, {0.42194031055233955, 0.1711086642582994}, 
       {0.42144252071987, 0.19688554271270667}, {0.42144252071987, 
       0.19706183792441243}, {0.4208298563106768, 0.22247353344028628}, 
       {0.4207149817339531, 0.22309056668125649}, {0.4186568122343196, 
       0.24754837917665093}, {0.41850364613202135, 0.24960725539907183}, 
       {0.4173070359578158, 0.27289396398813515}, {0.4171921613810921, 
       0.2758280200115239}, {0.41657949697189894, 0.29844417717034927}, 
       {0.41657949697189894, 0.30181897122300255}, {0.4162731647673023, 
       0.32413290801890365}, {0.4162348732417277, 0.3277217748286282}, 
       {0.4160625613766421, 0.34985312015526265}, {0.4159668325627057, 
       0.3535993934040102}, {0.41566050035810914, 0.3755103697160124}, 
       {0.41560306306974726, 0.37950849326719677}, {0.4148946698466176, 
       0.40104799038310474}, {0.41470321221874473, 0.4055938883420891}, 
       {0.4134778834003583, 0.4263715382931258}, {0.41305667661903794, 
       0.43192483746185734}, {0.7942105221883655, 0.04629165437061765}, 
       {0.8726315665650968, 0.04329463577161964}, {0.3664941815203537, 
       0.08855213511951393}, {0.36821730017120957, 0.08736843869806095}, 
       {0.5496808398691244, 0.07142631455381104}, {0.5589473890581718, 
       0.06946188219480395}, {0.566308934849884, 0.06802633547091413}, 
       {0.4733466836362076, 0.09790207759748042}, {0.4805263446814405, 
       0.0941180268033674}, {0.48117730061620834, 0.09381580644044321}, 
       {0.7746052610941827, 0.031457671557089686}, {0.853026305470914, 
       0.029741941371738932}, {0.9314473498476452, 0.041657608805780386}, 
       {1.0098683942243765, 0.03991984171896641}, {1.0882894386011077, 
       0.03871096026726974}, {1.166710482977839, 0.03785466923898459}, 
       {1.2451315273545702, 0.03722504348289257}, {1.3235525717313015, 
       0.03669615784777528}, {1.4019736161080327, 0.03629319736387639}, 
       {1.4803946604847646, 0.03604134706143958}, {0.6765789556232686, 
       0.05374642332274715}, {0.3224206355840169, 0.4613157677562328}, 
       {0.3223823440584423, 0.4617439132703754}, {0.320429476254139, 
       0.48710523872576184}, {0.3203050287960216, 0.4882165281852642}, 
       {0.6550974097759317, 0.05574863322711977}, {0.6579692741940248, 
       0.055459005379317444}, {0.5197368668698061, 0.04576276873550035}, 
       {0.5426351991634026, 0.04331982080186332}, {0.5981579112465374, 
       0.038805404130683535}, {0.5735747518276597, 0.04059983753554579}, 
       {0.5864407044207172, 0.03964280638628592}, {0.634841192746981, 
       0.036620602757044235}, {0.6058066434800591, 0.03830485165459039}, 
       {0.35224973400661147, 0.10026317418282549}, {0.3456635916077844, 
       0.10749127786276186}, {0.5367478771063114, 0.07447370321329641}, 
       {0.539342127963989, 0.07376852236647335}, {0.3342335712237735, 
       0.1260526451523546}, {0.33837862886722136, 0.11799028734559627}, 
       {0.33620558479086426, 0.12193489270751279}, {0.3302321068012304, 
       0.13679406055128443}, {0.33295080511702524, 0.12910003381183993}, 
       {0.4609210835872577, 0.1056024005944858}, {0.4392480801120478, 
       0.1260526451523546}, {0.3269773271273914, 0.15184211612188364}, 
       {0.32915994408514226, 0.1407481102995423}, {0.32716878475526434, 
       0.15069619724579617}, {0.3259051644113033, 0.16400648572958143}, 
       {0.3268624525506677, 0.1528872948769964}, {0.4258843376865208, 
       0.15184211612188364}, {0.32580943559736686, 0.17763158709141275}, 
       {0.32580943559736686, 0.16543573619591034}, {0.3257902898345796, 
       0.1769389987597115}, {0.3265561203460712, 0.18958188394203926}, 
       {0.3259051644113033, 0.17836195296847945}, {0.42171056139889207, 
       0.17405531279681008}, {0.32804948984347954, 0.2034210580609418}, 
       {0.32672843221115666, 0.19152742752836355}, {0.3278963237411812, 
       0.20203588139753936}, {0.328547279675949, 0.2147165441252326}, 
       {0.32820265594577785, 0.20490697484531895}, {0.42178714445004123, 
       0.2034210580609418}, {0.42171056139889207, 0.2013936631263255}, 
       {0.3277814491644575, 0.2292105290304709}, {0.3283558220480762, 
       0.21785208039057086}, {0.3278963237411812, 0.22782535236706847}, 
       {0.32732195085756266, 0.2409089755786606}, {0.32774315763888295, 
       0.23054533563338597}, {0.3268624525506677, 0.25499999999999995}, 
       {0.32719750339944526, 0.24326062777766425}, {0.326881598313455, 
       0.2539485249873263}, {0.3265561203460712, 0.26695029685062643}, 
       {0.32682416102509315, 0.25603258623999087}, {0.32636466271819825, 
       0.28078947096952905}, {0.32651782882049657, 0.26882658160378076}, 
       {0.32636466271819825, 0.2799079949110002}, {0.32621149661589993, 
       0.2928531004562521}, {0.32636466271819825, 0.2816709470280579}, 
       {0.3260583305136016, 0.30657894193905816}, {0.32621149661589993, 
       0.2945153124523351}, {0.3260583305136016, 0.30579820600150404}, 
       {0.3259721745810588, 0.31872127464529276}, {0.3260583305136016, 
       0.3073596778766123}, {0.3259051644113033, 0.33236841290858726}, 
       {0.3259626016996652, 0.32022293207357216}, {0.3259051644113033, 
       0.3316380470315205}, {0.3258190084787605, 0.3445611156753092}, 
       {0.3259051644113033, 0.333098778785654}, {0.325751998309005, 
       0.35815788387811637}, {0.3258190084787605, 0.3459651811113944}, 
       {0.325751998309005, 0.35747788806153696}, {0.32563712373228126, 
       0.3704104010916671}, {0.325751998309005, 0.35883787969469577}, 
       {0.3254456661044084, 0.3839473548476455}, {0.3255988322067067, 
       0.3716822451189729}, {0.3254456661044084, 0.3833680991520408}, 
       {0.3251967711881737, 0.39634468598509737}, {0.3254456661044084, 
       0.38452661054325016}, {0.3248712932207898, 0.4097368258171746}, 
       {0.3251776254253864, 0.39733319842216175}, {0.3248712932207898, 
       0.4093464578483975}, {0.3244309406766821, 0.42238600725706327}, 
       {0.3248330016952152, 0.4101146012708298}, {0.32391400508142537, 
       0.4356018518774348}, {0.32320561185829566, 0.44857843871049125}, 
       {0.3224397813468042, 0.4609065110147729}, {0.4099550630474973, 
       0.4613157677562328}, {0.41118039186588373, 0.4514054583553444}, 
       {0.4102996867776684, 0.4586209695201589}, {0.4084616935500888, 
       0.4721201457307718}, {0.40964873084290065, 0.4637964932352354}, 
       {0.3214633474446525, 0.47494086911806405}, {0.32054435083086263, 
       0.486072652485771}, {0.40616420201561426, 0.48710523872576184}, 
       {0.407944757954832, 0.47613086179707803}, {0.406413096931849, 
       0.48568858077455485}, {0.40396243929507614, 0.4993892372271171}, 
       {0.40595359862495406, 0.48837078649550675}, {0.4038284189555651, 
       0.49999997421052633}, {0.6734390505261534, 0.03475691051901186}, 
       {0.6508279046743664, 0.035789496759002774}, {0.6569736945290858, 
       0.03553764645656597}, {0.4855616802944972, 0.050340147982289335}, 
       {0.5001316057756233, 0.04823090169938106}, {0.6888513895699201, 
       0.052720133340317166}, {0.7079588608316335, 0.05125940158618368}, 
       {0.3594485408146317, 0.09381580644044321}, {0.5069474973278978, 
       0.08316253864736628}, {0.49572808033454707, 0.08736843869806095}, 
       {0.5001316057756233, 0.08565585664149067}, {0.5197368668698061, 
       0.07900700865715896}, {0.5138016804057468, 0.08092107095567869}, 
       {0.3414419509131874, 0.11315790966759004}, {0.3432895170221607, 
       0.11063940664322197}, {0.3296194423920371, 0.13894738063711912}, 
       {0.3258190084787605, 0.1647368516066482}, {0.32667099492279483, 
       0.19052632257617727}, {0.421174480040848, 0.19052632257617727}, 
       {0.32850898815037444, 0.21631579354570635}, {0.4214808122454446, 
       0.21631579354570635}, {0.42171056139889207, 0.2149558019125476}, 
       {0.32728365933198805, 0.24210526451523542}, {0.4190301546086717, 
       0.24210526451523542}, {0.3265561203460712, 0.2678947354847645}, 
       {0.41749849358568875, 0.2678947354847645}, {0.32621149661589993, 
       0.2936842064542936}, {0.4167326630741972, 0.2936842064542936}, 
       {0.3259721745810588, 0.3194736774238227}, {0.4162731647673023, 
       0.3194736774238227}, {0.3258190084787605, 0.3452631483933518}, 
       {0.4160817071394294, 0.3452631483933518}, {0.32563712373228126, 
       0.3710526193628809}, {0.41577537493483285, 0.3710526193628809}, 
       {0.3251776254253864, 0.39684209033241}, {0.4150478359489159, 
       0.39684209033241}, {0.3244117949138948, 0.42263156130193913}, 
       {0.41376506984216765, 0.42263156130193913}, {0.41152501559605487, 
       0.44842103227146823}, {0.4081553613454922, 0.47421050324099734}, 
       {0.6003788197298627, 0.06230933360559861}, {0.39657217485918295, 
       0.07265408477819048}, {0.44874437845454257, 0.11560085760122707}, 
       {0.43649109027067834, 0.059992310823179976}, {1.4803946604847646, 
       0.025891779873236237}}, {{{EdgeForm[], RGBColor[0, 1, 0], 
          Opacity[0.3], GraphicsGroup[{Polygon[{{167, 89, 38}, {164, 163, 
             33}, {165, 89, 35}, {141, 43, 16}, {39, 37, 14}, {207, 206, 41}, 
             {144, 36, 13}, {225, 224, 144}, {61, 40, 16}, {91, 56, 35}, {58, 
             38, 13}, {168, 61, 42}, {171, 107, 106}, {90, 59, 38}, {147, 37, 
             15}, {76, 39, 14}, {77, 57, 37}, {199, 161, 30}, {162, 161, 31}, 
             {179, 112, 111}, {51, 117, 25}, {138, 110, 18}, {45, 110, 19}, 
             {108, 109, 18}, {42, 106, 17}, {50, 116, 24}, {49, 115, 23}, 
             {48, 114, 22}, {47, 113, 21}, {47, 66, 20}, {48, 67, 21}, {174, 
             109, 108}, {212, 138, 18}, {46, 111, 20}, {216, 183, 68}, {111, 
             112, 20}, {140, 104, 3}, {110, 45, 18}, {111, 46, 19}, {35, 56, 
             1}, {78, 74, 55}, {231, 230, 196}, {37, 57, 12}, {101, 60, 1}, 
             {74, 54, 28}, {42, 61, 16}, {209, 169, 63}, {214, 178, 66}, {45, 
             64, 18}, {44, 63, 17}, {36, 58, 13}, {211, 173, 64}, {43, 62, 
             16}, {46, 65, 19}, {213, 176, 65}, {108, 44, 17}, {38, 59, 13}, 
             {227, 226, 147}, {200, 163, 32}, {142, 141, 40}, {60, 35, 1}, 
             {206, 37, 12}, {106, 42, 16}, {113, 47, 20}, {115, 49, 22}, 
             {121, 55, 28}, {120, 54, 27}, {63, 42, 17}, {118, 52, 25}, {172, 
             63, 44}, {116, 50, 23}, {119, 53, 26}, {114, 48, 21}, {117, 51, 
             24}, {194, 73, 54}, {81, 105, 3}, {137, 108, 17}, {131, 97, 8}, 
             {89, 91, 35}, {133, 98, 9}, {135, 99, 10}, {123, 93, 4}, {127, 
             95, 6}, {125, 94, 5}, {129, 96, 7}, {160, 100, 11}, {218, 187, 
             70}, {52, 71, 25}, {89, 90, 38}, {51, 70, 24}, {198, 78, 55}, 
             {151, 104, 80}, {219, 189, 71}, {217, 185, 69}, {92, 81, 3}, 
             {93, 82, 4}, {279, 517, 138}, {521, 522, 178}, {520, 519, 177}, 
             {514, 513, 175}, {515, 516, 176}, {548, 549, 189}, {388, 390, 
             110}, {293, 624, 57}, {91, 201, 56}, {94, 83, 5}, {96, 85, 7}, 
             {95, 84, 6}, {99, 88, 10}, {98, 87, 9}, {450, 401, 116}, {97, 
             86, 8}, {136, 106, 16}, {49, 68, 22}, {150, 102, 79}, {62, 136, 
             16}, {210, 137, 17}, {130, 131, 8}, {128, 129, 7}, {230, 121, 
             30}, {156, 130, 8}, {134, 135, 10}, {132, 133, 9}, {157, 132, 
             9}, {106, 107, 17}, {44, 108, 18}, {153, 124, 5}, {52, 118, 26}, 
             {54, 120, 28}, {158, 134, 10}, {53, 119, 27}, {50, 69, 23}, 
             {152, 122, 4}, {124, 125, 5}, {53, 72, 26}, {143, 76, 14}, {39, 
             77, 37}, {221, 193, 73}, {220, 191, 72}, {57, 75, 12}, {222, 
             195, 74}, {54, 73, 27}, {55, 74, 28}, {155, 128, 7}, {154, 126, 
             6}, {122, 123, 4}, {126, 127, 6}, {139, 102, 2}, {79, 101, 1}, 
             {80, 103, 2}, {509, 510, 173}, {73, 53, 27}, {180, 66, 47}, 
             {225, 145, 41}, {128, 155, 84}, {205, 142, 40}, {226, 141, 14}, 
             {141, 142, 14}, {148, 147, 15}, {124, 153, 82}, {122, 152, 81}, 
             {37, 147, 14}, {68, 183, 48}, {67, 181, 47}, {142, 143, 14}, 
             {102, 150, 2}, {227, 148, 43}, {104, 151, 3}, {149, 148, 15}, 
             {69, 185, 49}, {146, 145, 13}, {145, 144, 13}, {58, 166, 38}, 
             {33, 163, 34}, {132, 157, 86}, {100, 160, 88}, {134, 158, 87}, 
             {65, 176, 45}, {137, 174, 108}, {229, 164, 31}, {64, 173, 44}, 
             {126, 154, 83}, {130, 156, 85}, {202, 144, 12}, {66, 178, 46}, 
             {63, 169, 42}, {148, 170, 43}, {136, 171, 106}, {100, 159, 11}, 
             {182, 215, 67}, {184, 216, 68}, {72, 191, 52}, {70, 187, 50}, 
             {71, 189, 51}, {73, 193, 53}, {161, 196, 30}, {231, 197, 55}, 
             {197, 198, 55}, {161, 199, 32}, {37, 206, 15}, {163, 200, 34}, 
             {224, 225, 41}, {74, 195, 54}, {203, 202, 12}, {75, 203, 12}, 
             {202, 204, 36}, {144, 202, 36}, {180, 214, 66}, {197, 196, 29}, 
             {206, 207, 15}, {172, 209, 63}, {109, 212, 18}, {107, 210, 17}, 
             {175, 211, 64}, {177, 213, 65}, {186, 217, 69}, {190, 219, 71}, 
             {144, 224, 12}, {162, 223, 161}, {168, 208, 61}, {78, 222, 74}, 
             {224, 206, 12}, {192, 220, 72}, {196, 223, 29}, {188, 218, 70}, 
             {194, 221, 73}, {192, 72, 53}, {223, 196, 161}, {228, 161, 32}, 
             {488, 265, 36}, {278, 387, 109}, {624, 294, 57}, {276, 386, 
             107}, {593, 589, 207}, {365, 325, 83}, {361, 323, 82}, {280, 
             391, 112}, {357, 321, 81}, {226, 227, 43}, {161, 228, 31}, {40, 
             141, 16}, {164, 229, 163}, {228, 229, 31}, {369, 327, 84}, {163, 
             228, 32}, {141, 226, 43}, {103, 139, 2}, {69, 49, 23}, {64, 44, 
             18}, {175, 64, 45}, {177, 65, 46}, {67, 47, 21}, {66, 46, 20}, 
             {65, 45, 19}, {182, 67, 48}, {68, 48, 22}, {184, 68, 49}, {215, 
             181, 67}, {70, 50, 24}, {186, 69, 50}, {188, 70, 51}, {190, 71, 
             52}, {72, 52, 26}, {71, 51, 25}, {229, 228, 163}, {148, 227, 
             147}, {230, 231, 55}, {268, 353, 103}, {433, 434, 130}, {431, 
             432, 128}, {429, 430, 126}, {385, 335, 88}, {292, 585, 204}, 
             {303, 304, 75}, {625, 351, 100}, {147, 226, 14}, {223, 162, 29}, 
             {206, 224, 41}, {621, 295, 59}, {145, 225, 144}, {437, 438, 
             134}, {435, 436, 132}, {105, 140, 3}, {121, 230, 55}, {623, 299, 
             62}, {425, 426, 122}, {338, 316, 79}, {197, 231, 196}, {581, 
             283, 56}, {341, 318, 80}, {196, 230, 30}, {373, 329, 85}, {377, 
             331, 86}, {381, 333, 87}, {274, 504, 170}, {270, 355, 105}, 
             {622, 243, 39}, {427, 428, 124}, {446, 395, 114}, {448, 398, 
             115}, {495, 272, 40}, {444, 392, 113}, {508, 507, 172}, {452, 
             404, 117}, {350, 625, 100}, {419, 337, 1}, {553, 554, 191}, 
             {404, 406, 117}, {416, 418, 121}, {316, 420, 79}, {318, 422, 
             80}, {558, 559, 193}, {421, 340, 2}, {552, 551, 190}, {417, 619, 
             30}, {575, 579, 200}, {283, 302, 56}, {407, 409, 118}, {582, 
             583, 201}, {413, 415, 120}, {249, 421, 2}, {578, 580, 34}, {557, 
             556, 192}, {562, 561, 194}, {410, 412, 119}, {234, 621, 59}, 
             {619, 569, 30}, {616, 457, 27}, {618, 459, 28}, {606, 447, 22}, 
             {604, 445, 21}, {620, 576, 32}, {271, 622, 39}, {244, 623, 62}, 
             {610, 451, 24}, {250, 423, 3}, {563, 564, 195}, {296, 587, 60}, 
             {454, 407, 118}, {612, 453, 25}, {482, 567, 162}, {608, 449, 
             23}, {614, 455, 26}, {566, 245, 29}, {325, 363, 83}, {568, 572, 
             199}, {345, 258, 95}, {347, 260, 97}, {346, 259, 96}, {344, 257, 
             94}, {248, 419, 1}, {343, 256, 93}, {342, 255, 92}, {307, 592, 
             41}, {306, 305, 76}, {247, 254, 33}, {456, 410, 119}, {458, 413, 
             120}, {570, 568, 199}, {424, 342, 92}, {483, 482, 162}, {348, 
             261, 98}, {485, 484, 164}, {577, 575, 200}, {590, 313, 15}, 
             {309, 244, 62}, {354, 269, 104}, {235, 356, 4}, {236, 360, 5}, 
             {358, 235, 4}, {238, 368, 7}, {571, 620, 32}, {573, 246, 31}, 
             {484, 574, 164}, {323, 359, 82}, {489, 232, 58}, {252, 281, 29}, 
             {352, 267, 102}, {245, 252, 29}, {246, 253, 31}, {524, 523, 
             179}, {297, 296, 60}, {349, 262, 99}, {295, 312, 59}, {315, 314, 
             78}, {588, 298, 205}, {586, 481, 35}, {460, 416, 121}, {542, 
             541, 186}, {467, 466, 146}, {537, 536, 184}, {242, 384, 11}, 
             {240, 376, 9}, {398, 400, 115}, {239, 372, 8}, {374, 239, 8}, 
             {335, 383, 88}, {497, 307, 41}, {465, 498, 145}, {273, 495, 40}, 
             {331, 375, 86}, {594, 595, 208}, {382, 241, 10}, {502, 503, 
             169}, {241, 380, 10}, {327, 367, 84}, {392, 394, 113}, {411, 
             616, 27}, {405, 612, 25}, {402, 610, 24}, {532, 531, 182}, {533, 
             534, 183}, {470, 469, 149}, {399, 608, 23}, {408, 614, 26}, 
             {362, 236, 5}, {366, 237, 6}, {370, 238, 7}, {589, 591, 207}, 
             {329, 371, 85}, {538, 539, 185}, {494, 493, 167}, {501, 500, 
             168}, {395, 397, 114}, {237, 364, 6}, {547, 546, 188}, {599, 
             441, 19}, {543, 544, 187}, {601, 443, 20}, {527, 526, 180}, 
             {396, 606, 22}, {391, 602, 112}, {333, 379, 87}, {528, 529, 
             181}, {401, 403, 116}, {440, 279, 138}, {389, 599, 19}, {439, 
             277, 137}, {393, 604, 21}, {487, 486, 165}, {491, 492, 166}, 
             {264, 488, 36}, {378, 240, 9}, {414, 618, 28}}], 
            Polygon[{{397, 396, 22, 114}, {412, 411, 27, 119}, {464, 306, 76, 
             143}, {305, 271, 39, 76}, {517, 388, 110, 138}, {469, 468, 148, 
             149}, {506, 508, 172, 44}, {409, 408, 26, 118}, {512, 514, 175, 
             45}, {301, 440, 138, 212}, {587, 586, 35, 60}, {461, 352, 102, 
             139}, {403, 402, 24, 116}, {300, 439, 137, 210}, {602, 601, 20, 
             112}, {518, 520, 177, 46}, {462, 354, 104, 140}, {525, 527, 180, 
             47}, {287, 346, 96, 129}, {390, 389, 19, 110}, {285, 344, 94, 
             125}, {282, 315, 78, 198}, {523, 280, 112, 179}, {394, 393, 21, 
             113}, {466, 465, 145, 146}, {499, 501, 168, 42}, {530, 532, 182, 
             48}, {442, 524, 179, 111}, {400, 399, 23, 115}, {535, 537, 184, 
             49}, {540, 542, 186, 50}, {322, 427, 124, 82}, {406, 405, 25, 
             117}, {436, 289, 133, 132}, {457, 458, 120, 27}, {453, 454, 118, 
             25}, {455, 456, 119, 26}, {418, 417, 30, 121}, {434, 288, 131, 
             130}, {330, 435, 132, 86}, {376, 478, 157, 9}, {415, 414, 28, 
             120}, {380, 479, 158, 10}, {459, 460, 121, 28}, {441, 442, 111, 
             19}, {355, 462, 140, 105}, {451, 452, 117, 24}, {447, 448, 115, 
             22}, {443, 444, 113, 20}, {353, 461, 139, 103}, {449, 450, 116, 
             23}, {438, 290, 135, 134}, {445, 446, 114, 21}, {299, 275, 136, 
             62}, {423, 424, 92, 3}, {320, 425, 122, 81}, {426, 284, 123, 
             122}, {310, 293, 57, 77}, {312, 311, 13, 59}, {511, 278, 109, 
             174}, {251, 234, 59, 90}, {290, 349, 99, 135}, {289, 348, 98, 
             133}, {266, 297, 60, 101}, {288, 347, 97, 131}, {291, 584, 202, 
             203}, {384, 480, 160, 11}, {360, 474, 153, 5}, {368, 476, 155, 
             7}, {432, 287, 129, 128}, {328, 433, 130, 85}, {372, 477, 156, 
             8}, {326, 431, 128, 84}, {430, 286, 127, 126}, {324, 429, 126, 
             83}, {428, 285, 125, 124}, {364, 475, 154, 6}, {505, 276, 107, 
             171}, {298, 463, 142, 205}, {332, 437, 134, 87}, {336, 251, 90, 
             89}, {555, 557, 192, 53}, {265, 489, 58, 36}, {519, 598, 213, 
             177}, {387, 301, 212, 109}, {574, 573, 31, 164}, {253, 483, 162, 
             31}, {254, 485, 164, 33}, {567, 566, 29, 162}, {480, 385, 88, 
             160}, {549, 545, 51, 189}, {272, 588, 205, 40}, {492, 490, 38, 
             166}, {232, 491, 166, 58}, {479, 381, 87, 158}, {526, 600, 214, 
             180}, {513, 597, 211, 175}, {561, 615, 221, 194}, {541, 607, 
             217, 186}, {546, 609, 218, 188}, {314, 617, 222, 78}, {536, 605, 
             216, 184}, {595, 496, 61, 208}, {592, 593, 207, 41}, {386, 300, 
             210, 107}, {531, 603, 215, 182}, {507, 596, 209, 172}, {500, 
             594, 208, 168}, {591, 590, 15, 207}, {498, 497, 41, 145}, {463, 
             464, 143, 142}, {351, 263, 159, 100}, {544, 540, 50, 187}, {598, 
             515, 176, 213}, {609, 543, 187, 218}, {522, 518, 46, 178}, {600, 
             521, 178, 214}, {516, 512, 45, 176}, {607, 538, 185, 217}, {510, 
             506, 44, 173}, {539, 535, 49, 185}, {277, 511, 174, 137}, {504, 
             308, 43, 170}, {275, 505, 171, 136}, {529, 525, 47, 181}, {603, 
             528, 181, 215}, {534, 530, 48, 183}, {471, 249, 2, 150}, {476, 
             369, 84, 155}, {477, 373, 85, 156}, {472, 250, 3, 151}, {478, 
             377, 86, 157}, {551, 611, 219, 190}, {474, 361, 82, 153}, {475, 
             365, 83, 154}, {605, 533, 183, 216}, {473, 357, 81, 152}, {468, 
             274, 170, 148}, {503, 499, 42, 169}, {596, 502, 169, 209}, {556, 
             613, 220, 192}, {585, 264, 36, 204}, {615, 558, 193, 221}, {233, 
             339, 91, 89}, {481, 487, 165, 35}, {262, 334, 88, 99}, {496, 
             273, 40, 61}, {334, 350, 100, 88}, {545, 547, 188, 51}, {356, 
             473, 152, 4}, {337, 338, 79, 1}, {261, 332, 87, 98}, {319, 268, 
             103, 80}, {321, 270, 105, 81}, {317, 266, 101, 79}, {340, 341, 
             80, 2}, {260, 330, 86, 97}, {267, 317, 79, 102}, {256, 322, 82, 
             93}, {284, 343, 93, 123}, {255, 320, 81, 92}, {286, 345, 95, 
             127}, {281, 565, 197, 29}, {486, 336, 89, 165}, {258, 326, 84, 
             95}, {294, 303, 75, 57}, {490, 494, 167, 38}, {302, 248, 1, 56}, 
             {269, 319, 80, 104}, {257, 324, 83, 94}, {259, 328, 85, 96}, 
             {560, 562, 194, 54}, {313, 470, 149, 15}, {308, 309, 62, 43}, 
             {583, 581, 56, 201}, {339, 582, 201, 91}, {576, 577, 200, 32}, 
             {584, 292, 204, 202}, {565, 282, 198, 197}, {613, 553, 191, 
             220}, {554, 550, 52, 191}, {564, 560, 54, 195}, {304, 291, 203, 
             75}, {617, 563, 195, 222}, {611, 548, 189, 219}, {559, 555, 53, 
             193}, {579, 578, 34, 200}, {569, 570, 199, 30}, {572, 571, 32, 
             199}, {359, 358, 4, 82}, {493, 233, 89, 167}, {422, 472, 151, 
             80}, {243, 310, 77, 39}, {420, 471, 150, 79}, {311, 467, 146, 
             13}, {383, 382, 10, 88}, {375, 374, 8, 86}, {550, 552, 190, 52}, 
             {379, 378, 9, 87}, {367, 366, 6, 84}, {371, 370, 7, 85}, {363, 
             362, 5, 83}, {597, 509, 173, 211}}]}]}, {}, {}, {}, {}}, 
        {{RGBColor[0, 2/3, 0], Line[{242, 11, 159, 263, 351, 625, 350, 334, 
           262, 349, 290, 438, 437, 332, 261, 348, 289, 436, 435, 330, 260, 
           347, 288, 434, 433, 328, 259, 346, 287, 432, 431, 326, 258, 345, 
           286, 430, 429, 324, 257, 344, 285, 428, 427, 322, 256, 343, 284, 
           426, 425, 320, 255, 342, 424, 423, 250, 472, 422, 318, 341, 340, 
           421, 249, 471, 420, 316, 338, 337, 419, 248, 302, 283, 581, 583, 
           582, 339, 233, 493, 494, 490, 492, 491, 232, 489, 265, 488, 264, 
           585, 292, 584, 291, 304, 303, 294, 624, 293, 310, 243, 622, 271, 
           305, 306, 464, 463, 298, 588, 272, 495, 273, 496, 595, 594, 500, 
           501, 499, 503, 502, 596, 507, 508, 506, 510, 509, 597, 513, 514, 
           512, 516, 515, 598, 519, 520, 518, 522, 521, 600, 526, 527, 525, 
           529, 528, 603, 531, 532, 530, 534, 533, 605, 536, 537, 535, 539, 
           538, 607, 541, 542, 540, 544, 543, 609, 546, 547, 545, 549, 548, 
           611, 551, 552, 550, 554, 553, 613, 556, 557, 555, 559, 558, 615, 
           561, 562, 560, 564, 563, 617, 314, 315, 282, 565, 281, 252, 245, 
           566, 567, 482, 483, 253, 246, 573, 574, 484, 485, 254, 247, 33, 
           34, 580, 578, 579, 575, 577, 576, 620, 571, 572, 568, 570, 569, 
           619, 417, 418, 416, 460, 459, 618, 414, 415, 413, 458, 457, 616, 
           411, 412, 410, 456, 455, 614, 408, 409, 407, 454, 453, 612, 405, 
           406, 404, 452, 451, 610, 402, 403, 401, 450, 449, 608, 399, 400, 
           398, 448, 447, 606, 396, 397, 395, 446, 445, 604, 393, 394, 392, 
           444, 443, 601, 602, 391, 280, 523, 524, 442, 441, 599, 389, 390, 
           388, 517, 279, 440, 301, 387, 278, 511, 277, 439, 300, 386, 276, 
           505, 275, 299, 623, 244, 309, 308, 504, 274, 468, 469, 470, 313, 
           590, 591, 589, 593, 592, 307, 497, 498, 465, 466, 467, 311, 312, 
           295, 621, 234, 251, 336, 486, 487, 481, 586, 587, 296, 297, 266, 
           317, 267, 352, 461, 353, 268, 319, 269, 354, 462, 355, 270, 321, 
           357, 473, 356, 235, 358, 359, 323, 361, 474, 360, 236, 362, 363, 
           325, 365, 475, 364, 237, 366, 367, 327, 369, 476, 368, 238, 370, 
           371, 329, 373, 477, 372, 239, 374, 375, 331, 377, 478, 376, 240, 
           378, 379, 333, 381, 479, 380, 241, 382, 383, 335, 385, 480, 384, 
           242}]}}}], GraphicsComplex[{{0.010000078421052631, 
       0.2936842064542936}, {0.08842112279778394, 0.2936842064542936}, 
       {0.16684216717451525, 0.2936842064542936}, {0.24526321155124656, 
       0.2936842064542936}, {0.3236842559279779, 0.2936842064542936}, 
       {0.4021053003047092, 0.2936842064542936}, {0.4805263446814405, 
       0.2936842064542936}, {0.5589473890581718, 0.2936842064542936}, 
       {1.4999999215789475, 0.2936842064542936}, {0.010000078421052631, 
       0.3194736774238227}, {0.08842112279778394, 0.3194736774238227}, 
       {0.16684216717451525, 0.3194736774238227}, {0.24526321155124656, 
       0.3194736774238227}, {0.3236842559279779, 0.3194736774238227}, 
       {0.4021053003047092, 0.3194736774238227}, {0.4805263446814405, 
       0.3194736774238227}, {0.5589473890581718, 0.3194736774238227}, 
       {0.637368433434903, 0.3194736774238227}, {0.7157894778116343, 
       0.3194736774238227}, {0.7942105221883655, 0.3194736774238227}, 
       {0.8726315665650968, 0.3194736774238227}, {0.951052610941828, 
       0.3194736774238227}, {1.0294736553185593, 0.3194736774238227}, 
       {1.264736788448753, 0.3194736774238227}, {1.3431578328254843, 
       0.3194736774238227}, {1.4215788772022155, 0.3194736774238227}, 
       {1.4999999215789475, 0.3194736774238227}, {0.010000078421052631, 
       0.3452631483933518}, {0.08842112279778394, 0.3452631483933518}, 
       {0.16684216717451525, 0.3452631483933518}, {0.24526321155124656, 
       0.3452631483933518}, {0.3236842559279779, 0.3452631483933518}, 
       {0.4021053003047092, 0.3452631483933518}, {0.4805263446814405, 
       0.3452631483933518}, {0.5589473890581718, 0.3452631483933518}, 
       {0.637368433434903, 0.3452631483933518}, {0.7157894778116343, 
       0.3452631483933518}, {0.7942105221883655, 0.3452631483933518}, 
       {0.8726315665650968, 0.3452631483933518}, {0.951052610941828, 
       0.3452631483933518}, {1.0294736553185593, 0.3452631483933518}, 
       {1.1078946996952905, 0.3452631483933518}, {1.1863157440720218, 
       0.3452631483933518}, {1.264736788448753, 0.3452631483933518}, 
       {1.3431578328254843, 0.3452631483933518}, {1.4215788772022155, 
       0.3452631483933518}, {1.4999999215789475, 0.3452631483933518}, 
       {0.010000078421052631, 0.3710526193628809}, {0.08842112279778394, 
       0.3710526193628809}, {0.16684216717451525, 0.3710526193628809}, 
       {0.24526321155124656, 0.3710526193628809}, {0.3236842559279779, 
       0.3710526193628809}, {0.4021053003047092, 0.3710526193628809}, 
       {0.4805263446814405, 0.3710526193628809}, {0.5589473890581718, 
       0.3710526193628809}, {0.637368433434903, 0.3710526193628809}, 
       {0.7157894778116343, 0.3710526193628809}, {0.7942105221883655, 
       0.3710526193628809}, {0.8726315665650968, 0.3710526193628809}, 
       {0.951052610941828, 0.3710526193628809}, {1.0294736553185593, 
       0.3710526193628809}, {1.1078946996952905, 0.3710526193628809}, 
       {1.1863157440720218, 0.3710526193628809}, {1.264736788448753, 
       0.3710526193628809}, {1.3431578328254843, 0.3710526193628809}, 
       {1.4215788772022155, 0.3710526193628809}, {1.4999999215789475, 
       0.3710526193628809}, {0.010000078421052631, 0.39684209033241}, 
       {0.08842112279778394, 0.39684209033241}, {0.16684216717451525, 
       0.39684209033241}, {0.24526321155124656, 0.39684209033241}, 
       {0.3236842559279779, 0.39684209033241}, {0.4021053003047092, 
       0.39684209033241}, {0.4805263446814405, 0.39684209033241}, 
       {0.5589473890581718, 0.39684209033241}, {0.637368433434903, 
       0.39684209033241}, {0.7157894778116343, 0.39684209033241}, 
       {0.7942105221883655, 0.39684209033241}, {0.8726315665650968, 
       0.39684209033241}, {0.951052610941828, 0.39684209033241}, 
       {1.0294736553185593, 0.39684209033241}, {1.1078946996952905, 
       0.39684209033241}, {1.1863157440720218, 0.39684209033241}, 
       {1.264736788448753, 0.39684209033241}, {1.3431578328254843, 
       0.39684209033241}, {1.4215788772022155, 0.39684209033241}, 
       {1.4999999215789475, 0.39684209033241}, {0.010000078421052631, 
       0.42263156130193913}, {0.08842112279778394, 0.42263156130193913}, 
       {0.16684216717451525, 0.42263156130193913}, {0.24526321155124656, 
       0.42263156130193913}, {0.3236842559279779, 0.42263156130193913}, 
       {0.4021053003047092, 0.42263156130193913}, {0.4805263446814405, 
       0.42263156130193913}, {0.5589473890581718, 0.42263156130193913}, 
       {0.637368433434903, 0.42263156130193913}, {0.7157894778116343, 
       0.42263156130193913}, {0.7942105221883655, 0.42263156130193913}, 
       {0.8726315665650968, 0.42263156130193913}, {0.951052610941828, 
       0.42263156130193913}, {1.0294736553185593, 0.42263156130193913}, 
       {1.1078946996952905, 0.42263156130193913}, {1.1863157440720218, 
       0.42263156130193913}, {1.264736788448753, 0.42263156130193913}, 
       {1.3431578328254843, 0.42263156130193913}, {1.4215788772022155, 
       0.42263156130193913}, {1.4999999215789475, 0.42263156130193913}, 
       {0.010000078421052631, 0.44842103227146823}, {0.08842112279778394, 
       0.44842103227146823}, {0.16684216717451525, 0.44842103227146823}, 
       {0.24526321155124656, 0.44842103227146823}, {0.3236842559279779, 
       0.44842103227146823}, {0.4021053003047092, 0.44842103227146823}, 
       {0.4805263446814405, 0.44842103227146823}, {0.5589473890581718, 
       0.44842103227146823}, {0.637368433434903, 0.44842103227146823}, 
       {0.7157894778116343, 0.44842103227146823}, {0.7942105221883655, 
       0.44842103227146823}, {0.8726315665650968, 0.44842103227146823}, 
       {0.951052610941828, 0.44842103227146823}, {1.0294736553185593, 
       0.44842103227146823}, {1.1078946996952905, 0.44842103227146823}, 
       {1.1863157440720218, 0.44842103227146823}, {1.264736788448753, 
       0.44842103227146823}, {1.3431578328254843, 0.44842103227146823}, 
       {1.4215788772022155, 0.44842103227146823}, {1.4999999215789475, 
       0.44842103227146823}, {0.010000078421052631, 0.47421050324099734}, 
       {0.08842112279778394, 0.47421050324099734}, {0.16684216717451525, 
       0.47421050324099734}, {0.24526321155124656, 0.47421050324099734}, 
       {0.3236842559279779, 0.47421050324099734}, {0.4021053003047092, 
       0.47421050324099734}, {0.5589473890581718, 0.47421050324099734}, 
       {0.637368433434903, 0.47421050324099734}, {0.7157894778116343, 
       0.47421050324099734}, {0.7942105221883655, 0.47421050324099734}, 
       {0.8726315665650968, 0.47421050324099734}, {0.951052610941828, 
       0.47421050324099734}, {1.0294736553185593, 0.47421050324099734}, 
       {1.1078946996952905, 0.47421050324099734}, {1.1863157440720218, 
       0.47421050324099734}, {1.264736788448753, 0.47421050324099734}, 
       {1.3431578328254843, 0.47421050324099734}, {1.4215788772022155, 
       0.47421050324099734}, {0.010000078421052631, 0.49999997421052633}, 
       {0.08842112279778394, 0.49999997421052633}, {0.16684216717451525, 
       0.49999997421052633}, {0.24526321155124656, 0.49999997421052633}, 
       {0.3236842559279779, 0.49999997421052633}, {0.4021053003047092, 
       0.49999997421052633}, {0.5589473890581718, 0.49999997421052633}, 
       {0.637368433434903, 0.49999997421052633}, {0.7157894778116343, 
       0.49999997421052633}, {0.7942105221883655, 0.49999997421052633}, 
       {0.8726315665650968, 0.49999997421052633}, {0.951052610941828, 
       0.49999997421052633}, {1.0294736553185593, 0.49999997421052633}, 
       {1.1078946996952905, 0.49999997421052633}, {1.1863157440720218, 
       0.49999997421052633}, {1.264736788448753, 0.49999997421052633}, 
       {1.3431578328254843, 0.49999997421052633}, {0.04921060060941829, 
       0.28078947096952905}, {0.1276316449861496, 0.28078947096952905}, 
       {0.010000078421052631, 0.28078947096952905}, {0.2060526893628809, 
       0.28078947096952905}, {0.5981579112465374, 0.30657894193905816}, 
       {1.4607893993905816, 0.30657894193905816}, {0.6765789556232686, 
       0.30657894193905816}, {0.7549999999999999, 0.30657894193905816}, 
       {1.068684177506925, 0.33236841290858726}, {1.2255262662603874, 
       0.33236841290858726}, {1.38236835501385, 0.30657894193905816}, 
       {1.4215788772022155, 0.30657894193905816}, {1.1471052218836562, 
       0.33236841290858726}, {1.1863157440720218, 0.33236841290858726}, 
       {0.4413158224930749, 0.4613157677562328}, {0.4413158224930749, 
       0.48710523872576184}, {1.4607893993905816, 0.4613157677562328}, 
       {0.4413158224930749, 0.49999997421052633}, {1.38236835501385, 
       0.48710523872576184}, {1.4215788772022155, 0.48710523872576184}, 
       {1.38236835501385, 0.49999997421052633}, {0.08842112279778394, 
       0.28078947096952905}, {0.16684216717451525, 0.28078947096952905}, 
       {0.24526321155124656, 0.28078947096952905}, {1.4607893993905816, 
       0.2936842064542936}, {0.637368433434903, 0.30657894193905816}, 
       {0.7157894778116343, 0.30657894193905816}, {0.7942105221883655, 
       0.30657894193905816}, {1.2255262662603874, 0.3194736774238227}, 
       {1.1078946996952905, 0.33236841290858726}, {0.4805263446814405, 
       0.4613157677562328}, {0.4413158224930749, 0.47421050324099734}, 
       {1.4999999215789475, 0.4613157677562328}, {1.4607893993905816, 
       0.47421050324099734}, {1.4803946604847646, 0.2872368387119113}, 
       {0.4609210835872577, 0.46776313549861503}, {1.4803946604847646, 
       0.46776313549861503}, {1.4019736161080327, 0.4935526064681441}, 
       {0.6177631723407202, 0.3001315741966759}, {1.4411841382963986, 
       0.3001315741966759}, {1.0882894386011077, 0.325921045166205}, 
       {1.2059210051662046, 0.325921045166205}, {1.4411841382963986, 
       0.4806578709833796}, {1.4999999215789475, 0.2872368387119113}, 
       {1.4019736161080327, 0.49999997421052633}, {0.4609210835872577, 
       0.4935526064681441}, {0.4609210835872577, 0.4806578709833796}, 
       {0.4609210835872577, 0.47421050324099734}, {0.4609210835872577, 
       0.49999997421052633}, {0.2844737337396122, 0.30657894193905816}, 
       {0.2844737337396122, 0.2936842064542936}, {0.3628947781163435, 
       0.30657894193905816}, {0.3628947781163435, 0.2936842064542936}, 
       {0.4413158224930749, 0.30657894193905816}, {0.4413158224930749, 
       0.2936842064542936}, {0.5197368668698061, 0.30657894193905816}, 
       {0.5197368668698061, 0.2936842064542936}, {0.8334210443767311, 
       0.33236841290858726}, {0.8334210443767311, 0.3194736774238227}, 
       {0.9118420887534624, 0.33236841290858726}, {0.9118420887534624, 
       0.3194736774238227}, {0.9902631331301937, 0.33236841290858726}, 
       {0.9902631331301937, 0.3194736774238227}, {1.3039473106371187, 
       0.33236841290858726}, {1.3039473106371187, 0.3194736774238227}, 
       {0.5981579112465374, 0.4613157677562328}, {0.5589473890581718, 
       0.4613157677562328}, {0.5981579112465374, 0.48710523872576184}, 
       {0.5589473890581718, 0.48710523872576184}, {0.2648684726454294, 
       0.2872368387119113}, {0.3432895170221607, 0.2872368387119113}, 
       {0.42171056139889207, 0.2872368387119113}, {0.5001316057756233, 
       0.2872368387119113}, {0.6569736945290858, 0.3001315741966759}, 
       {0.8138157832825483, 0.3130263096814404}, {0.8922368276592796, 
       0.3130263096814404}, {1.4019736161080327, 0.3001315741966759}, 
       {1.1274999607894733, 0.325921045166205}, {1.166710482977839, 
       0.325921045166205}, {0.5197368668698061, 0.4355262967867037}, 
       {0.539342127963989, 0.45486840001385054}, {0.3040789948337951, 
       0.2872368387119113}, {0.3236842559279779, 0.2872368387119113}, 
       {0.38250003921052633, 0.2872368387119113}, {0.4021053003047092, 
       0.2872368387119113}, {0.4609210835872577, 0.2872368387119113}, 
       {0.4805263446814405, 0.2872368387119113}, {0.539342127963989, 
       0.2872368387119113}, {0.5589473890581718, 0.30657894193905816}, 
       {0.5785526501523546, 0.3001315741966759}, {0.5981579112465374, 
       0.3001315741966759}, {1.4411841382963986, 0.2936842064542936}, 
       {0.853026305470914, 0.3130263096814404}, {0.8726315665650968, 
       0.3130263096814404}, {1.0294736553185593, 0.33236841290858726}, 
       {1.049078916412742, 0.325921045166205}, {1.068684177506925, 
       0.325921045166205}, {1.2059210051662046, 0.3194736774238227}, 
       {1.3235525717313015, 0.3130263096814404}, {0.4805263446814405, 
       0.46776313549861503}, {0.539342127963989, 0.3001315741966759}, 
       {1.0098683942243765, 0.325921045166205}, {1.38236835501385, 
       0.33236841290858726}, {1.38236835501385, 0.3194736774238227}, 
       {0.3236842559279779, 0.30657894193905816}, {0.3040789948337951, 
       0.3001315741966759}, {0.4021053003047092, 0.30657894193905816}, 
       {0.38250003921052633, 0.3001315741966759}, {0.4805263446814405, 
       0.30657894193905816}, {0.4609210835872577, 0.3001315741966759}, 
       {0.8726315665650968, 0.33236841290858726}, {0.853026305470914, 
       0.325921045166205}, {0.951052610941828, 0.33236841290858726}, 
       {0.9314473498476452, 0.325921045166205}, {1.3431578328254843, 
       0.33236841290858726}, {1.3235525717313015, 0.325921045166205}, 
       {0.5981579112465374, 0.47421050324099734}, {0.5785526501523546, 
       0.4806578709833796}, {1.4019736161080327, 0.3130263096814404}, 
       {0.5981579112465374, 0.4355262967867037}, {0.5981579112465374, 
       0.44842103227146823}, {0.5785526501523546, 0.45486840001385054}, 
       {0.5981579112465374, 0.33236841290858726}, {0.5981579112465374, 
       0.3194736774238227}, {1.068684177506925, 0.35815788387811637}, 
       {1.068684177506925, 0.3452631483933518}, {1.4607893993905816, 
       0.33236841290858726}, {1.4215788772022155, 0.33236841290858726}, 
       {1.4019736161080327, 0.325921045166205}, {0.6177631723407202, 
       0.3130263096814404}, {1.0882894386011077, 0.3388157806509695}, 
       {1.4607893993905816, 0.3194736774238227}, {1.4411841382963986, 
       0.325921045166205}, {0.6765789556232686, 0.33236841290858726}, 
       {0.637368433434903, 0.33236841290858726}, {0.6177631723407202, 
       0.325921045166205}, {1.1471052218836562, 0.35815788387811637}, 
       {1.1078946996952905, 0.35815788387811637}, {1.0882894386011077, 
       0.3517105161357341}, {0.6765789556232686, 0.3194736774238227}, 
       {0.6569736945290858, 0.325921045166205}, {1.1471052218836562, 
       0.3452631483933518}, {1.1274999607894733, 0.3517105161357341}, 
       {0.08842112279778394, 0.27811985776369885}, {0.16684216717451525, 
       0.2790768889129588}, {0.24526321155124656, 0.2805376206670922}, 
       {0.637368433434903, 0.29761307117230784}, {0.7157894778116343, 
       0.30113267914886216}, {0.7942105221883655, 0.30592413115272243}, 
       {1.4215788772022155, 0.29585011905525016}, {1.1078946996952905, 
       0.32065737384527576}, {1.1863157440720218, 0.3196247876052848}, 
       {0.5291948736867265, 0.44842103227146823}, {0.4782671446725405, 
       0.47421050324099734}, {0.5434010296748939, 0.47421050324099734}, 
       {0.46875170056725846, 0.49999997421052633}, {0.5526292873383667, 
       0.49999997421052633}, {1.4097085042740969, 0.49999997421052633}, 
       {0.9367315803769367, 0.3147640767682544}, {1.0279228485327887, 
       0.3189636805613882}, {1.2542449104413191, 0.3160233282804384}, 
       {0.47855433111434986, 0.4735619887122226}, {0.5406440398335246, 
       0.4681912810127576}, {1.4821560706611954, 0.46834239119421966}, 
       {0.46988130057170846, 0.49649925500665476}, {0.5518921754710562, 
       0.49767980329932726}, {1.414112029715173, 0.4975444337617675}, 
       {0.0401546548110311, 0.27781134114321376}, {0.058017651491570725, 
       0.27789319249150574}, {0.12041369241534206, 0.2784157818690622}, 
       {0.1342943704361258, 0.2785983733383289}, {0.010000078421052631, 
       0.27774208231004366}, {0.20252029612862632, 0.2796278114495393}, 
       {0.2091925944599961, 0.27975688472953814}, {0.28255915746088345, 
       0.2814190967256211}, {0.35357079163893435, 0.2838557484016972}, 
       {0.42990494787185124, 0.2845420404758375}, {0.5144526363405146, 
       0.282527238056343}, {0.6959544675640039, 0.30020712928740695}, 
       {0.7433498033439352, 0.30274766921323826}, {0.762983783082299, 
       0.3039534025361544}, {0.8286824680868774, 0.3081372656853859}, 
       {0.8944577361426049, 0.3122959438043737}, {1.3720679346342888, 
       0.30319155537128306}, {0.5344216669276559, 0.456486538207007}, 
       {1.4456642467886238, 0.4821311952526349}, {1.4215788772022155, 
       0.4935651989832659}, {1.4346745789487203, 0.48710523872576184}, 
       {0.25728675058166334, 0.28078947096952905}, {0.3236842559279779, 
       0.28270353326804876}, {0.4021053003047092, 0.2852188881636364}, 
       {0.4805263446814405, 0.28235094284463724}, {0.5913420196942629, 
       0.2936842064542936}, {0.5981579112465374, 0.2945908675430662}, 
       {1.4999999215789475, 0.28320093761536147}, {1.4607893993905816, 
       0.2896042315548173}, {0.804491796805139, 0.30657894193905816}, 
       {0.8726315665650968, 0.31096113720145857}, {1.0437946858834506, 
       0.3194736774238227}, {1.068684177506925, 0.32017885827064574}, 
       {1.2255262662603874, 0.31785868735944667}, {1.3431578328254843, 
       0.3070826425439318}, {1.346795527755069, 0.30657894193905816}, 
       {0.48452780910398374, 0.4613157677562328}, {1.4999999215789475, 
       0.4628268695708536}, {1.4607893993905816, 0.47592308529756766}, 
       {1.4786715418339085, 0.2866701755314285}, {1.4855257249117577, 
       0.28554944168558466}, {1.2314231611988724, 0.3175344300950593}, 
       {0.5688266026564124, 0.2904353375528588}, {0.627125450343704, 
       0.29705270424938596}, {0.602523145162039, 0.29511975317818345}, 
       {1.4259824026432917, 0.29513234569330526}, {1.030718129899733, 
       0.3190644206823629}, {1.104410170868004, 0.3206195962999102}, 
       {1.070751919887952, 0.32015367324040206}, {1.1866986593277677, 
       0.3195996025750411}, {1.4839940638887748, 0.46776313549861503}, 
       {0.4730977887199728, 0.48710523872576184}, {0.47212135481782114, 
       0.48986929579500577}, {0.47784593789122015, 0.4750919792995261}, 
       {0.47386361923146436, 0.4849141410945616}, {0.48393429045757774, 
       0.4624365016020766}, {1.463278348552929, 0.47502901672391695}, 
       {1.46546096551068, 0.47421050324099734}, {1.4803946604847646, 
       0.46887127682933705}, {0.2844737337396122, 0.28149465181635214}, 
       {0.3628947781163435, 0.28418945005242596}, {0.4413158224930749, 
       0.28400685858315927}, {0.5197368668698061, 0.283156863812435}, 
       {0.8334210443767311, 0.30849300423757786}, {0.9118420887534624, 
       0.3133789001048519}, {0.9902631331301937, 0.31755961512530295}, 
       {1.3039473106371187, 0.31159076295755067}, {0.5371595110062382, 
       0.4613157677562328}, {0.540337707628928, 0.4674357301054472}, 
       {0.5483597822368016, 0.48710523872576184}, {0.549527673766826, 
       0.49020299744573453}, {0.04921060060941829, 0.27786800746126206}, 
       {0.01922833608452541, 0.27775467482516547}, {0.08007357022252641, 
       0.2780443026729678}, {0.1276316449861496, 0.27852281824759784}, 
       {0.09639533299868935, 0.2781670796954058}, {0.16125160444062714, 
       0.2789509637617404}, {0.2060526893628809, 0.27973169969929446}, 
       {0.17193494007593388, 0.2791146664583243}, {0.2444207979886059, 
       0.2805124356368485}, {0.33034698137795404, 0.28298056860072923}, 
       {0.4153924596790871, 0.2851590737168076}, {0.48480542266439935, 
       0.2821966845343947}, {0.6765789556232686, 0.2994263933498529}, 
       {0.6513831317951977, 0.2982930669888872}, {0.6611857623422892, 
       0.2987463975332734}, {0.6964714031592608, 0.3002260180600897}, 
       {0.7549999999999999, 0.3035063682493291}, {0.7298041761719289, 
       0.30197008140446463}, {0.7917407187888054, 0.3057667247136994}, 
       {0.8889820479854404, 0.311955945896084}, {0.9613913228469635, 
       0.31607369834092575}, {0.9831792008988971, 0.3171440621262822}, 
       {1.2823604630944516, 0.31367797233899564}, {1.285490795310173, 
       0.3134040851350956}, {1.38236835501385, 0.30173082361714965}, 
       {1.4093351618997447, 0.2977106631645021}, {1.3992932093178125, 
       0.299250098138147}, {1.1471052218836562, 0.3205818187545447}, 
       {1.1114941030993006, 0.32065737384527576}, {1.143812150684243, 
       0.32055663372430104}, {1.1858658186465203, 0.31962163947650435}, 
       {1.1501302524040475, 0.32046848611844814}, {0.492396717609559, 
       0.44842103227146823}, {0.5197368668698061, 0.43736480399449235}, 
       {0.49025239217738276, 0.4516195311124157}, {0.48535107690383705, 
       0.4597291108508809}, {0.5319135720025212, 0.4524254520802135}, 
       {0.5452390229024737, 0.4787186236546162}, {0.5469238500277551, 
       0.48315118897750403}, {1.42931376536828, 0.4896489267803736}, 
       {1.4411841382963986, 0.48410822012676386}, {0.28669464222293756, 
       0.2815198368465958}, {0.3184957542126229, 0.2824957567685384}, 
       {0.37434394426314177, 0.2845546329909593}, {0.38943080533952446, 
       0.28495759347485816}, {0.4498548326962053, 0.28359760184169946}, 
       {0.4753378429660855, 0.2824957567685384}, {0.5319805821722767, 
       0.2848159276797375}, {0.542137409330933, 0.28631758510801697}, 
       {0.5589473890581718, 0.2889494207684816}, {0.5481491788461414, 
       0.2872368387119113}, {0.5962050434422341, 0.2943264247255074}, 
       {1.452441846815324, 0.2909390381577324}, {1.4351340772556154, 
       0.2936842064542936}, {1.4411841382963986, 0.29277754536552103}, 
       {1.475110429955473, 0.2872368387119113}, {0.8404571122010596, 
       0.3088928165926963}, {0.8614887326228953, 0.3102433638395137}, 
       {0.9276947803413367, 0.3142603761633808}, {0.951052610941828, 
       0.3155448127058085}, {0.9956430924734216, 0.3177044290492041}, 
       {1.0294736553185593, 0.3190203468794365}, {1.0668653300421322, 
       0.3200718218921101}, {1.264736788448753, 0.31519222228239696}, 
       {1.2213524899727586, 0.31810109327554204}, {1.1902214796806283, 
       0.3194736774238227}, {1.2059210051662046, 0.31885664418285253}, 
       {1.3153964767839172, 0.3103441039604884}, {1.340879487053797, 
       0.30732819658880767}, {0.4805263446814405, 0.4692742373132359}, 
       {0.4812155921417829, 0.46776313549861503}, {1.4491679213786974, 
       0.4806578709833796}, {0.24604818782552534, 0.28053132440953127}, 
       {0.7958187662624976, 0.30605005630394083}}, 
       {{{EdgeForm[], RGBColor[1, 0, 0], Opacity[0.3], GraphicsGroup[
           {Polygon[{{11, 1, 2}, {268, 267, 212}, {12, 2, 3}, {239, 174, 
             173}, {13, 3, 4}, {201, 188, 167}, {272, 271, 216}, {270, 269, 
             214}, {263, 251, 218}, {168, 9, 27}, {298, 297, 285}, {30, 11, 
             12}, {58, 37, 38}, {29, 10, 11}, {32, 13, 14}, {34, 15, 16}, 
             {35, 16, 17}, {33, 14, 15}, {31, 12, 13}, {296, 19, 37}, {274, 
             273, 220}, {241, 176, 175}, {264, 257, 224}, {276, 275, 222}, 
             {203, 192, 171}, {289, 27, 47}, {278, 277, 226}, {172, 24, 44}, 
             {38, 19, 20}, {49, 28, 29}, {57, 36, 37}, {54, 33, 34}, {52, 31, 
             32}, {51, 30, 31}, {53, 32, 33}, {50, 29, 30}, {56, 35, 36}, 
             {55, 34, 35}, {102, 81, 82}, {59, 38, 39}, {61, 40, 41}, {64, 
             43, 44}, {301, 300, 287}, {70, 49, 50}, {299, 43, 63}, {69, 48, 
             49}, {66, 45, 46}, {65, 44, 45}, {67, 46, 47}, {71, 50, 51}, 
             {79, 58, 59}, {73, 52, 53}, {60, 39, 40}, {72, 51, 52}, {75, 54, 
             55}, {77, 56, 57}, {78, 57, 58}, {76, 55, 56}, {80, 59, 60}, 
             {81, 60, 61}, {82, 61, 62}, {84, 63, 64}, {85, 64, 65}, {86, 65, 
             66}, {87, 66, 67}, {89, 68, 69}, {90, 69, 70}, {91, 70, 71}, 
             {83, 62, 63}, {92, 71, 72}, {94, 73, 74}, {97, 76, 77}, {95, 74, 
             75}, {96, 75, 76}, {98, 77, 78}, {93, 72, 73}, {291, 290, 265}, 
             {100, 79, 80}, {99, 78, 79}, {101, 80, 81}, {103, 82, 83}, {297, 
             296, 36}, {113, 92, 93}, {107, 86, 87}, {114, 93, 94}, {105, 84, 
             85}, {109, 88, 89}, {112, 91, 92}, {106, 85, 86}, {110, 89, 90}, 
             {242, 95, 115}, {121, 100, 101}, {117, 96, 97}, {282, 96, 116}, 
             {122, 101, 102}, {144, 124, 125}, {119, 98, 99}, {120, 99, 100}, 
             {118, 97, 98}, {111, 90, 91}, {123, 102, 103}, {124, 103, 104}, 
             {130, 109, 110}, {127, 106, 107}, {126, 105, 106}, {129, 108, 
             109}, {193, 177, 114}, {132, 111, 112}, {131, 110, 111}, {228, 
             116, 135}, {137, 117, 118}, {143, 123, 124}, {125, 104, 105}, 
             {140, 120, 121}, {138, 118, 119}, {139, 119, 120}, {141, 121, 
             122}, {104, 83, 84}, {142, 122, 123}, {136, 116, 117}, {74, 53, 
             54}, {145, 125, 126}, {188, 169, 18}, {156, 137, 138}, {150, 
             131, 132}, {157, 138, 139}, {148, 129, 130}, {151, 132, 133}, 
             {155, 136, 137}, {149, 130, 131}, {230, 135, 153}, {158, 139, 
             140}, {165, 163, 1}, {160, 141, 142}, {159, 140, 141}, {184, 
             164, 2}, {195, 179, 127}, {162, 143, 144}, {182, 181, 145}, 
             {161, 142, 143}, {154, 135, 136}, {185, 166, 3}, {1, 11, 10}, 
             {269, 216, 15}, {212, 13, 4}, {3, 13, 12}, {267, 214, 14}, {189, 
             170, 19}, {251, 167, 17}, {271, 218, 16}, {174, 168, 26}, {11, 
             30, 29}, {285, 35, 17}, {2, 12, 11}, {14, 33, 32}, {12, 31, 30}, 
             {13, 32, 31}, {15, 34, 33}, {147, 128, 129}, {16, 35, 34}, {10, 
             29, 28}, {308, 473, 186}, {19, 38, 37}, {273, 222, 39}, {192, 
             175, 42}, {275, 224, 40}, {28, 49, 48}, {257, 171, 41}, {290, 
             289, 46}, {226, 44, 24}, {176, 172, 43}, {277, 265, 45}, {29, 
             50, 49}, {37, 58, 57}, {31, 52, 51}, {59, 80, 79}, {30, 51, 50}, 
             {33, 54, 53}, {35, 56, 55}, {36, 57, 56}, {34, 55, 54}, {38, 59, 
             58}, {39, 60, 59}, {40, 61, 60}, {300, 299, 62}, {43, 64, 63}, 
             {44, 65, 64}, {45, 66, 65}, {46, 67, 66}, {48, 69, 68}, {49, 70, 
             69}, {287, 61, 41}, {50, 71, 70}, {52, 73, 72}, {55, 76, 75}, 
             {53, 74, 73}, {54, 75, 74}, {56, 77, 76}, {51, 72, 71}, {32, 53, 
             52}, {58, 79, 78}, {57, 78, 77}, {102, 123, 122}, {103, 124, 
             123}, {62, 83, 82}, {65, 86, 85}, {63, 84, 83}, {71, 92, 91}, 
             {64, 85, 84}, {70, 91, 90}, {68, 89, 88}, {66, 87, 86}, {69, 90, 
             89}, {72, 93, 92}, {80, 101, 100}, {74, 95, 94}, {61, 82, 81}, 
             {73, 94, 93}, {76, 97, 96}, {78, 99, 98}, {79, 100, 99}, {77, 
             98, 97}, {81, 102, 101}, {82, 103, 102}, {83, 104, 103}, {85, 
             106, 105}, {86, 107, 106}, {88, 109, 108}, {89, 110, 109}, {90, 
             111, 110}, {91, 112, 111}, {92, 113, 112}, {84, 105, 104}, {93, 
             114, 113}, {282, 115, 95}, {98, 119, 118}, {96, 117, 116}, {97, 
             118, 117}, {99, 120, 119}, {242, 114, 94}, {60, 81, 80}, {101, 
             122, 121}, {100, 121, 120}, {133, 112, 113}, {104, 125, 124}, 
             {198, 194, 177}, {109, 130, 129}, {106, 127, 126}, {229, 228, 
             134}, {108, 129, 128}, {177, 133, 113}, {111, 132, 131}, {110, 
             131, 130}, {112, 133, 132}, {116, 136, 135}, {124, 144, 143}, 
             {118, 138, 137}, {2, 164, 3}, {117, 137, 136}, {120, 140, 139}, 
             {122, 142, 141}, {123, 143, 142}, {121, 141, 140}, {125, 145, 
             144}, {179, 145, 126}, {128, 147, 146}, {130, 149, 148}, {131, 
             150, 149}, {132, 151, 150}, {178, 151, 133}, {231, 230, 152}, 
             {135, 154, 153}, {136, 155, 154}, {129, 148, 147}, {137, 156, 
             155}, {139, 158, 157}, {142, 161, 160}, {140, 159, 158}, {141, 
             160, 159}, {143, 162, 161}, {138, 157, 156}, {119, 139, 138}, 
             {1, 163, 2}, {181, 162, 144}, {220, 38, 20}, {105, 126, 125}, 
             {202, 187, 168}, {19, 170, 20}, {294, 168, 27}, {281, 174, 26}, 
             {302, 169, 19}, {281, 266, 173}, {204, 191, 172}, {293, 288, 
             171}, {43, 172, 44}, {304, 175, 43}, {178, 180, 151}, {114, 177, 
             113}, {292, 286, 167}, {175, 176, 43}, {194, 178, 133}, {127, 
             179, 126}, {199, 196, 179}, {208, 180, 178}, {145, 181, 144}, 
             {200, 183, 181}, {205, 182, 145}, {163, 184, 2}, {164, 185, 3}, 
             {166, 186, 4}, {168, 187, 9}, {292, 188, 18}, {169, 189, 19}, 
             {170, 190, 20}, {181, 183, 162}, {172, 191, 24}, {262, 198, 
             193}, {179, 196, 145}, {177, 194, 133}, {210, 209, 194}, {187, 
             197, 9}, {293, 192, 42}, {3, 166, 4}, {195, 199, 179}, {193, 
             198, 177}, {182, 200, 181}, {253, 201, 167}, {174, 202, 168}, 
             {176, 204, 172}, {196, 205, 145}, {197, 206, 9}, {200, 207, 
             183}, {194, 209, 178}, {198, 210, 194}, {208, 211, 180}, {234, 
             217, 6}, {213, 212, 4}, {232, 213, 4}, {284, 283, 228}, {14, 
             214, 15}, {13, 212, 14}, {233, 215, 5}, {217, 216, 6}, {15, 216, 
             16}, {270, 215, 6}, {268, 213, 5}, {272, 217, 7}, {264, 225, 
             23}, {235, 219, 7}, {263, 219, 8}, {221, 220, 20}, {38, 220, 
             39}, {237, 221, 20}, {274, 221, 21}, {223, 222, 21}, {219, 218, 
             7}, {16, 218, 17}, {276, 223, 22}, {225, 224, 22}, {40, 224, 
             41}, {39, 222, 40}, {227, 226, 24}, {44, 226, 45}, {278, 227, 
             25}, {238, 223, 21}, {215, 214, 5}, {279, 228, 135}, {280, 279, 
             230}, {186, 232, 4}, {152, 230, 153}, {190, 237, 20}, {280, 231, 
             134}, {188, 236, 169}, {247, 234, 6}, {245, 233, 5}, {249, 235, 
             7}, {256, 238, 21}, {217, 248, 7}, {95, 242, 94}, {284, 229, 
             115}, {192, 240, 175}, {213, 244, 5}, {215, 246, 6}, {246, 247, 
             6}, {244, 245, 5}, {248, 249, 7}, {219, 250, 8}, {218, 251, 17}, 
             {251, 252, 167}, {252, 253, 167}, {202, 254, 187}, {221, 255, 
             21}, {255, 256, 21}, {224, 257, 41}, {258, 257, 23}, {252, 251, 
             8}, {257, 258, 171}, {204, 260, 191}, {219, 263, 218}, {227, 
             261, 25}, {251, 263, 8}, {257, 264, 23}, {258, 259, 171}, {45, 
             265, 46}, {266, 265, 25}, {225, 264, 224}, {229, 243, 115}, 
             {173, 266, 25}, {192, 293, 171}, {214, 267, 5}, {267, 268, 5}, 
             {213, 268, 212}, {214, 269, 15}, {216, 269, 6}, {269, 270, 6}, 
             {215, 270, 214}, {224, 275, 22}, {275, 276, 22}, {271, 272, 7}, 
             {217, 272, 216}, {220, 273, 39}, {216, 271, 16}, {273, 274, 21}, 
             {221, 274, 220}, {222, 275, 40}, {218, 271, 7}, {222, 273, 21}, 
             {223, 276, 222}, {228, 283, 116}, {265, 277, 25}, {277, 278, 
             25}, {227, 278, 226}, {228, 279, 134}, {230, 279, 135}, {279, 
             280, 134}, {231, 280, 230}, {35, 285, 36}, {226, 277, 45}, {96, 
             282, 95}, {283, 282, 116}, {282, 283, 115}, {174, 281, 173}, 
             {283, 284, 115}, {229, 284, 228}, {286, 285, 17}, {266, 281, 
             26}, {167, 286, 17}, {298, 286, 18}, {288, 287, 41}, {301, 288, 
             42}, {61, 287, 62}, {290, 291, 26}, {171, 288, 41}, {295, 290, 
             26}, {46, 289, 47}, {295, 294, 289}, {265, 290, 46}, {266, 291, 
             265}, {290, 295, 289}, {286, 292, 18}, {212, 267, 14}, {188, 
             292, 167}, {288, 293, 42}, {289, 294, 27}, {294, 295, 26}, {168, 
             294, 26}, {303, 302, 296}, {36, 296, 37}, {285, 297, 36}, {297, 
             298, 18}, {286, 298, 285}, {305, 304, 299}, {62, 299, 63}, {287, 
             300, 62}, {305, 300, 42}, {300, 301, 42}, {303, 297, 18}, {288, 
             301, 287}, {296, 302, 19}, {175, 304, 42}, {302, 303, 18}, {297, 
             303, 296}, {299, 304, 43}, {169, 302, 18}, {291, 266, 26}, {300, 
             305, 299}, {304, 305, 42}, {75, 96, 95}, {311, 474, 190}, {387, 
             386, 196}, {376, 361, 23}, {348, 441, 205}, {438, 317, 134}, 
             {350, 440, 182}, {440, 349, 182}, {413, 341, 169}, {326, 388, 
             199}, {450, 372, 8}, {454, 455, 254}, {400, 399, 231}, {378, 
             377, 203}, {380, 326, 199}, {472, 348, 205}, {466, 467, 260}, 
             {321, 460, 22}, {374, 373, 201}, {453, 358, 187}, {471, 470, 
             262}, {366, 385, 193}, {372, 355, 8}, {363, 371, 191}, {322, 
             462, 23}, {417, 343, 170}, {259, 203, 171}, {365, 346, 173}, 
             {407, 336, 166}, {398, 397, 229}, {474, 359, 190}, {404, 333, 
             164}, {386, 368, 196}, {401, 331, 163}, {465, 363, 191}, {424, 
             396, 227}, {449, 451, 250}, {436, 366, 193}, {468, 469, 261}, 
             {448, 449, 250}, {369, 370, 197}, {420, 345, 238}, {347, 437, 
             243}, {446, 447, 248}, {442, 443, 244}, {473, 351, 186}, {457, 
             458, 255}, {444, 445, 246}, {394, 459, 223}, {422, 395, 225}, 
             {395, 461, 225}, {317, 325, 134}, {433, 435, 114}, {332, 404, 
             164}, {427, 426, 239}, {306, 405, 184}, {346, 425, 173}, {460, 
             421, 22}, {406, 307, 185}, {403, 306, 184}, {419, 311, 190}, 
             {432, 431, 241}, {411, 339, 234}, {414, 415, 236}, {330, 401, 
             163}, {409, 308, 186}, {412, 340, 235}, {416, 310, 189}, {410, 
             338, 233}, {429, 430, 240}, {310, 418, 189}, {383, 384, 209}, 
             {319, 328, 152}, {335, 407, 166}, {382, 327, 208}, {342, 417, 
             170}, {464, 423, 24}, {456, 369, 197}, {307, 408, 185}, {399, 
             439, 231}, {462, 376, 23}, {323, 464, 24}, {334, 402, 165}}], 
            Polygon[{{428, 432, 241, 175}, {345, 394, 223, 238}, {360, 420, 
             238, 256}, {385, 471, 262, 193}, {364, 365, 173, 25}, {371, 323, 
             24, 191}, {361, 463, 258, 23}, {377, 313, 192, 203}, {352, 410, 
             233, 245}, {373, 309, 188, 201}, {314, 379, 204, 176}, {370, 
             357, 206, 197}, {316, 383, 209, 210}, {367, 380, 199, 195}, 
             {329, 320, 207, 200}, {470, 324, 198, 262}, {349, 329, 200, 
             182}, {312, 375, 202, 174}, {388, 387, 196, 199}, {425, 427, 
             239, 173}, {356, 374, 201, 253}, {362, 378, 203, 259}, {355, 
             452, 252, 8}, {441, 350, 182, 205}, {354, 412, 235, 249}, {353, 
             411, 234, 247}, {384, 381, 178, 209}, {340, 392, 219, 235}, 
             {434, 433, 114, 242}, {325, 398, 229, 134}, {459, 321, 22, 223}, 
             {461, 322, 23, 225}, {333, 406, 185, 164}, {439, 438, 134, 231}, 
             {351, 337, 232, 186}, {435, 436, 193, 114}, {463, 362, 259, 
             258}, {397, 347, 243, 229}, {327, 318, 211, 208}, {336, 409, 
             186, 166}, {337, 389, 213, 232}, {331, 403, 184, 163}, {415, 
             413, 169, 236}, {421, 422, 225, 22}, {338, 390, 215, 233}, {359, 
             344, 237, 190}, {343, 419, 190, 170}, {328, 400, 231, 152}, 
             {341, 416, 189, 169}, {423, 424, 227, 24}, {313, 429, 240, 192}, 
             {430, 428, 175, 240}, {315, 434, 242, 115}, {309, 414, 236, 
             188}, {379, 466, 260, 204}, {368, 472, 205, 196}, {467, 465, 
             191, 260}, {324, 316, 210, 198}, {392, 448, 250, 219}, {437, 
             315, 115, 243}, {418, 342, 170, 189}, {452, 356, 253, 252}, 
             {408, 335, 166, 185}, {426, 312, 174, 239}, {402, 330, 163, 
             165}, {405, 332, 164, 184}, {431, 314, 176, 241}, {381, 382, 
             208, 178}, {455, 453, 187, 254}, {375, 454, 254, 202}, {451, 
             450, 8, 250}, {458, 360, 256, 255}, {396, 468, 261, 227}, {469, 
             364, 25, 261}, {393, 457, 255, 221}, {358, 456, 197, 187}, {390, 
             444, 246, 215}, {443, 352, 245, 244}, {447, 354, 249, 248}, 
             {344, 393, 221, 237}, {391, 446, 248, 217}, {445, 353, 247, 
             246}, {389, 442, 244, 213}, {339, 391, 217, 234}}]}]}, {}, {}, 
         {}, {}}, {{RGBColor[2/3, 0, 0], Line[{165, 1, 10, 28, 48, 68, 88, 
           108, 128, 146, 147, 148, 149, 150, 151, 180, 211, 318, 327, 382, 
           381, 384, 383, 316, 324, 470, 471, 385, 366, 436, 435, 433, 434, 
           315, 437, 347, 397, 398, 325, 317, 438, 439, 399, 400, 328, 319, 
           152, 153, 154, 155, 156, 157, 158, 159, 160, 161, 162, 183, 207, 
           320, 329, 349, 440, 350, 441, 348, 472, 368, 386, 387, 388, 326, 
           380, 367, 195, 127, 107, 87, 67, 47, 27, 9, 206, 357, 370, 369, 
           456, 358, 453, 455, 454, 375, 312, 426, 427, 425, 346, 365, 364, 
           469, 468, 396, 424, 423, 464, 323, 371, 363, 465, 467, 466, 379, 
           314, 431, 432, 428, 430, 429, 313, 377, 378, 362, 463, 361, 376, 
           462, 322, 461, 395, 422, 421, 460, 321, 459, 394, 345, 420, 360, 
           458, 457, 393, 344, 359, 474, 311, 419, 343, 417, 342, 418, 310, 
           416, 341, 413, 415, 414, 309, 373, 374, 356, 452, 355, 372, 450, 
           451, 449, 448, 392, 340, 412, 354, 447, 446, 391, 339, 411, 353, 
           445, 444, 390, 338, 410, 352, 443, 442, 389, 337, 351, 473, 308, 
           409, 336, 407, 335, 408, 307, 406, 333, 404, 332, 405, 306, 403, 
           331, 401, 330, 402, 334, 165}]}}}], GraphicsComplex[
       {{0.4805263446814405, 0.010000025789473685}, {0.5589473890581718, 
       0.010000025789473685}, {0.637368433434903, 0.010000025789473685}, 
       {0.7157894778116343, 0.010000025789473685}, {0.7942105221883655, 
       0.010000025789473685}, {0.8726315665650968, 0.010000025789473685}, 
       {0.951052610941828, 0.010000025789473685}, {1.0294736553185593, 
       0.010000025789473685}, {1.1078946996952905, 0.010000025789473685}, 
       {1.1863157440720218, 0.010000025789473685}, {1.264736788448753, 
       0.010000025789473685}, {1.3431578328254843, 0.010000025789473685}, 
       {1.4215788772022155, 0.010000025789473685}, {1.4999999215789475, 
       0.010000025789473685}, {0.4805263446814405, 0.035789496759002774}, 
       {0.5589473890581718, 0.035789496759002774}, {0.637368433434903, 
       0.035789496759002774}, {0.7157894778116343, 0.035789496759002774}, 
       {0.7942105221883655, 0.035789496759002774}, {0.8726315665650968, 
       0.035789496759002774}, {0.951052610941828, 0.035789496759002774}, 
       {1.0294736553185593, 0.035789496759002774}, {1.1078946996952905, 
       0.035789496759002774}, {1.1863157440720218, 0.035789496759002774}, 
       {1.264736788448753, 0.035789496759002774}, {1.3431578328254843, 
       0.035789496759002774}, {1.4215788772022155, 0.035789496759002774}, 
       {1.4999999215789475, 0.035789496759002774}, {0.4805263446814405, 
       0.06157896772853186}, {0.5589473890581718, 0.06157896772853186}, 
       {0.637368433434903, 0.06157896772853186}, {0.7157894778116343, 
       0.06157896772853186}, {0.7942105221883655, 0.06157896772853186}, 
       {0.8726315665650968, 0.06157896772853186}, {0.951052610941828, 
       0.06157896772853186}, {1.0294736553185593, 0.06157896772853186}, 
       {1.1078946996952905, 0.06157896772853186}, {1.1863157440720218, 
       0.06157896772853186}, {1.264736788448753, 0.06157896772853186}, 
       {1.3431578328254843, 0.06157896772853186}, {1.4215788772022155, 
       0.06157896772853186}, {1.4999999215789475, 0.06157896772853186}, 
       {0.4805263446814405, 0.08736843869806095}, {0.5589473890581718, 
       0.08736843869806095}, {0.637368433434903, 0.08736843869806095}, 
       {0.7157894778116343, 0.08736843869806095}, {0.7942105221883655, 
       0.08736843869806095}, {0.8726315665650968, 0.08736843869806095}, 
       {0.951052610941828, 0.08736843869806095}, {1.0294736553185593, 
       0.08736843869806095}, {1.1078946996952905, 0.08736843869806095}, 
       {1.1863157440720218, 0.08736843869806095}, {1.264736788448753, 
       0.08736843869806095}, {1.3431578328254843, 0.08736843869806095}, 
       {1.4215788772022155, 0.08736843869806095}, {1.4999999215789475, 
       0.08736843869806095}, {0.4805263446814405, 0.11315790966759004}, 
       {0.5589473890581718, 0.11315790966759004}, {0.637368433434903, 
       0.11315790966759004}, {0.7157894778116343, 0.11315790966759004}, 
       {0.7942105221883655, 0.11315790966759004}, {0.8726315665650968, 
       0.11315790966759004}, {0.951052610941828, 0.11315790966759004}, 
       {1.0294736553185593, 0.11315790966759004}, {1.1078946996952905, 
       0.11315790966759004}, {1.1863157440720218, 0.11315790966759004}, 
       {1.264736788448753, 0.11315790966759004}, {1.3431578328254843, 
       0.11315790966759004}, {1.4215788772022155, 0.11315790966759004}, 
       {1.4999999215789475, 0.11315790966759004}, {0.4805263446814405, 
       0.13894738063711912}, {0.5589473890581718, 0.13894738063711912}, 
       {0.637368433434903, 0.13894738063711912}, {0.7157894778116343, 
       0.13894738063711912}, {0.7942105221883655, 0.13894738063711912}, 
       {0.8726315665650968, 0.13894738063711912}, {0.951052610941828, 
       0.13894738063711912}, {1.0294736553185593, 0.13894738063711912}, 
       {1.1078946996952905, 0.13894738063711912}, {1.1863157440720218, 
       0.13894738063711912}, {1.264736788448753, 0.13894738063711912}, 
       {1.3431578328254843, 0.13894738063711912}, {1.4215788772022155, 
       0.13894738063711912}, {1.4999999215789475, 0.13894738063711912}, 
       {0.4805263446814405, 0.1647368516066482}, {0.5589473890581718, 
       0.1647368516066482}, {0.637368433434903, 0.1647368516066482}, 
       {0.7157894778116343, 0.1647368516066482}, {0.7942105221883655, 
       0.1647368516066482}, {0.8726315665650968, 0.1647368516066482}, 
       {0.951052610941828, 0.1647368516066482}, {1.0294736553185593, 
       0.1647368516066482}, {1.1078946996952905, 0.1647368516066482}, 
       {1.1863157440720218, 0.1647368516066482}, {1.264736788448753, 
       0.1647368516066482}, {1.3431578328254843, 0.1647368516066482}, 
       {1.4215788772022155, 0.1647368516066482}, {1.4999999215789475, 
       0.1647368516066482}, {0.4805263446814405, 0.19052632257617727}, 
       {0.5589473890581718, 0.19052632257617727}, {0.637368433434903, 
       0.19052632257617727}, {0.7157894778116343, 0.19052632257617727}, 
       {0.7942105221883655, 0.19052632257617727}, {0.8726315665650968, 
       0.19052632257617727}, {0.951052610941828, 0.19052632257617727}, 
       {1.0294736553185593, 0.19052632257617727}, {1.1078946996952905, 
       0.19052632257617727}, {1.1863157440720218, 0.19052632257617727}, 
       {1.264736788448753, 0.19052632257617727}, {1.3431578328254843, 
       0.19052632257617727}, {1.4215788772022155, 0.19052632257617727}, 
       {1.4999999215789475, 0.19052632257617727}, {0.4805263446814405, 
       0.21631579354570635}, {0.5589473890581718, 0.21631579354570635}, 
       {0.637368433434903, 0.21631579354570635}, {0.7157894778116343, 
       0.21631579354570635}, {0.7942105221883655, 0.21631579354570635}, 
       {0.8726315665650968, 0.21631579354570635}, {0.951052610941828, 
       0.21631579354570635}, {1.0294736553185593, 0.21631579354570635}, 
       {1.1078946996952905, 0.21631579354570635}, {1.1863157440720218, 
       0.21631579354570635}, {1.264736788448753, 0.21631579354570635}, 
       {1.3431578328254843, 0.21631579354570635}, {1.4215788772022155, 
       0.21631579354570635}, {1.4999999215789475, 0.21631579354570635}, 
       {0.4805263446814405, 0.24210526451523542}, {0.5589473890581718, 
       0.24210526451523542}, {0.637368433434903, 0.24210526451523542}, 
       {0.7157894778116343, 0.24210526451523542}, {0.7942105221883655, 
       0.24210526451523542}, {0.8726315665650968, 0.24210526451523542}, 
       {0.951052610941828, 0.24210526451523542}, {1.0294736553185593, 
       0.24210526451523542}, {1.1078946996952905, 0.24210526451523542}, 
       {1.1863157440720218, 0.24210526451523542}, {1.264736788448753, 
       0.24210526451523542}, {1.3431578328254843, 0.24210526451523542}, 
       {1.4215788772022155, 0.24210526451523542}, {1.4999999215789475, 
       0.24210526451523542}, {0.4805263446814405, 0.2678947354847645}, 
       {0.5589473890581718, 0.2678947354847645}, {0.637368433434903, 
       0.2678947354847645}, {0.7157894778116343, 0.2678947354847645}, 
       {0.7942105221883655, 0.2678947354847645}, {0.8726315665650968, 
       0.2678947354847645}, {0.951052610941828, 0.2678947354847645}, 
       {1.0294736553185593, 0.2678947354847645}, {1.1078946996952905, 
       0.2678947354847645}, {1.1863157440720218, 0.2678947354847645}, 
       {1.264736788448753, 0.2678947354847645}, {1.3431578328254843, 
       0.2678947354847645}, {1.4215788772022155, 0.2678947354847645}, 
       {1.4999999215789475, 0.2678947354847645}, {0.4805263446814405, 
       0.2936842064542936}, {0.5589473890581718, 0.2936842064542936}, 
       {0.637368433434903, 0.2936842064542936}, {0.7157894778116343, 
       0.2936842064542936}, {0.7942105221883655, 0.2936842064542936}, 
       {0.8726315665650968, 0.2936842064542936}, {0.951052610941828, 
       0.2936842064542936}, {1.0294736553185593, 0.2936842064542936}, 
       {1.1078946996952905, 0.2936842064542936}, {1.1863157440720218, 
       0.2936842064542936}, {1.264736788448753, 0.2936842064542936}, 
       {1.3431578328254843, 0.2936842064542936}, {1.4215788772022155, 
       0.2936842064542936}, {1.4999999215789475, 0.2936842064542936}, 
       {0.4805263446814405, 0.3194736774238227}, {0.5589473890581718, 
       0.3194736774238227}, {0.637368433434903, 0.3194736774238227}, 
       {0.7157894778116343, 0.3194736774238227}, {0.7942105221883655, 
       0.3194736774238227}, {0.8726315665650968, 0.3194736774238227}, 
       {0.951052610941828, 0.3194736774238227}, {1.0294736553185593, 
       0.3194736774238227}, {1.1078946996952905, 0.3194736774238227}, 
       {1.1863157440720218, 0.3194736774238227}, {1.264736788448753, 
       0.3194736774238227}, {1.3431578328254843, 0.3194736774238227}, 
       {1.4215788772022155, 0.3194736774238227}, {1.4999999215789475, 
       0.3194736774238227}, {0.4805263446814405, 0.3452631483933518}, 
       {0.5589473890581718, 0.3452631483933518}, {0.637368433434903, 
       0.3452631483933518}, {0.7157894778116343, 0.3452631483933518}, 
       {0.7942105221883655, 0.3452631483933518}, {0.8726315665650968, 
       0.3452631483933518}, {0.951052610941828, 0.3452631483933518}, 
       {1.0294736553185593, 0.3452631483933518}, {1.1078946996952905, 
       0.3452631483933518}, {1.1863157440720218, 0.3452631483933518}, 
       {1.264736788448753, 0.3452631483933518}, {1.3431578328254843, 
       0.3452631483933518}, {1.4215788772022155, 0.3452631483933518}, 
       {1.4999999215789475, 0.3452631483933518}, {0.4805263446814405, 
       0.3710526193628809}, {0.5589473890581718, 0.3710526193628809}, 
       {0.637368433434903, 0.3710526193628809}, {0.7157894778116343, 
       0.3710526193628809}, {0.7942105221883655, 0.3710526193628809}, 
       {0.8726315665650968, 0.3710526193628809}, {0.951052610941828, 
       0.3710526193628809}, {1.0294736553185593, 0.3710526193628809}, 
       {1.1078946996952905, 0.3710526193628809}, {1.1863157440720218, 
       0.3710526193628809}, {1.264736788448753, 0.3710526193628809}, 
       {1.3431578328254843, 0.3710526193628809}, {1.4215788772022155, 
       0.3710526193628809}, {1.4999999215789475, 0.3710526193628809}, 
       {0.4805263446814405, 0.39684209033241}, {0.5589473890581718, 
       0.39684209033241}, {0.637368433434903, 0.39684209033241}, 
       {0.7157894778116343, 0.39684209033241}, {0.7942105221883655, 
       0.39684209033241}, {0.8726315665650968, 0.39684209033241}, 
       {0.951052610941828, 0.39684209033241}, {1.0294736553185593, 
       0.39684209033241}, {1.1078946996952905, 0.39684209033241}, 
       {1.1863157440720218, 0.39684209033241}, {1.264736788448753, 
       0.39684209033241}, {1.3431578328254843, 0.39684209033241}, 
       {1.4215788772022155, 0.39684209033241}, {1.4999999215789475, 
       0.39684209033241}, {0.4805263446814405, 0.42263156130193913}, 
       {0.5589473890581718, 0.42263156130193913}, {0.637368433434903, 
       0.42263156130193913}, {0.7157894778116343, 0.42263156130193913}, 
       {0.7942105221883655, 0.42263156130193913}, {0.8726315665650968, 
       0.42263156130193913}, {0.951052610941828, 0.42263156130193913}, 
       {1.0294736553185593, 0.42263156130193913}, {1.1078946996952905, 
       0.42263156130193913}, {1.1863157440720218, 0.42263156130193913}, 
       {1.264736788448753, 0.42263156130193913}, {1.3431578328254843, 
       0.42263156130193913}, {1.4215788772022155, 0.42263156130193913}, 
       {1.4999999215789475, 0.42263156130193913}, {0.4805263446814405, 
       0.44842103227146823}, {0.5589473890581718, 0.44842103227146823}, 
       {0.637368433434903, 0.44842103227146823}, {0.7157894778116343, 
       0.44842103227146823}, {0.7942105221883655, 0.44842103227146823}, 
       {0.8726315665650968, 0.44842103227146823}, {0.951052610941828, 
       0.44842103227146823}, {1.0294736553185593, 0.44842103227146823}, 
       {1.1078946996952905, 0.44842103227146823}, {1.1863157440720218, 
       0.44842103227146823}, {1.264736788448753, 0.44842103227146823}, 
       {1.3431578328254843, 0.44842103227146823}, {1.4215788772022155, 
       0.44842103227146823}, {1.4999999215789475, 0.44842103227146823}, 
       {0.4805263446814405, 0.47421050324099734}, {0.5589473890581718, 
       0.47421050324099734}, {0.637368433434903, 0.47421050324099734}, 
       {0.7157894778116343, 0.47421050324099734}, {0.7942105221883655, 
       0.47421050324099734}, {0.8726315665650968, 0.47421050324099734}, 
       {0.951052610941828, 0.47421050324099734}, {1.0294736553185593, 
       0.47421050324099734}, {1.1078946996952905, 0.47421050324099734}, 
       {1.1863157440720218, 0.47421050324099734}, {1.264736788448753, 
       0.47421050324099734}, {1.3431578328254843, 0.47421050324099734}, 
       {1.4215788772022155, 0.47421050324099734}, {1.4999999215789475, 
       0.47421050324099734}, {0.4805263446814405, 0.49999997421052633}, 
       {0.5589473890581718, 0.49999997421052633}, {0.637368433434903, 
       0.49999997421052633}, {0.7157894778116343, 0.49999997421052633}, 
       {0.7942105221883655, 0.49999997421052633}, {0.8726315665650968, 
       0.49999997421052633}, {0.951052610941828, 0.49999997421052633}, 
       {1.0294736553185593, 0.49999997421052633}, {1.1078946996952905, 
       0.49999997421052633}, {1.1863157440720218, 0.49999997421052633}, 
       {1.264736788448753, 0.49999997421052633}, {1.3431578328254843, 
       0.49999997421052633}, {1.4215788772022155, 0.49999997421052633}, 
       {1.4999999215789475, 0.49999997421052633}, {0.4413158224930749, 
       0.02289476127423823}, {0.4413158224930749, 0.04868423224376732}, 
       {0.4413158224930749, 0.07447370321329641}, {0.4413158224930749, 
       0.10026317418282549}, {0.4413158224930749, 0.1260526451523546}, 
       {0.4413158224930749, 0.15184211612188364}, {0.4413158224930749, 
       0.17763158709141275}, {0.4413158224930749, 0.2034210580609418}, 
       {0.4413158224930749, 0.2292105290304709}, {0.4413158224930749, 
       0.25499999999999995}, {0.4413158224930749, 0.28078947096952905}, 
       {0.4413158224930749, 0.30657894193905816}, {0.4413158224930749, 
       0.33236841290858726}, {0.4413158224930749, 0.35815788387811637}, 
       {0.4413158224930749, 0.3839473548476455}, {0.4413158224930749, 
       0.4097368258171746}, {0.4413158224930749, 0.4355262967867037}, 
       {0.4413158224930749, 0.4613157677562328}, {0.4413158224930749, 
       0.48710523872576184}, {0.4413158224930749, 0.49999997421052633}, 
       {0.4413158224930749, 0.010000025789473685}, {0.4413158224930749, 
       0.035789496759002774}, {0.4413158224930749, 0.06157896772853186}, 
       {0.4413158224930749, 0.08736843869806095}, {0.4413158224930749, 
       0.11315790966759004}, {0.4413158224930749, 0.13894738063711912}, 
       {0.4413158224930749, 0.1647368516066482}, {0.4413158224930749, 
       0.19052632257617727}, {0.4413158224930749, 0.21631579354570635}, 
       {0.4413158224930749, 0.24210526451523542}, {0.4413158224930749, 
       0.2678947354847645}, {0.4413158224930749, 0.2936842064542936}, 
       {0.4413158224930749, 0.3194736774238227}, {0.4413158224930749, 
       0.3452631483933518}, {0.4413158224930749, 0.3710526193628809}, 
       {0.4413158224930749, 0.39684209033241}, {0.4413158224930749, 
       0.42263156130193913}, {0.4413158224930749, 0.44842103227146823}, 
       {0.4413158224930749, 0.47421050324099734}, {0.42171056139889207, 
       0.016447393531855956}, {0.42171056139889207, 0.0293421290166205}, 
       {0.42171056139889207, 0.042236864501385044}, {0.42171056139889207, 
       0.05513159998614959}, {0.42171056139889207, 0.06802633547091413}, 
       {0.42171056139889207, 0.08092107095567869}, {0.42171056139889207, 
       0.09381580644044321}, {0.42171056139889207, 0.10671054192520776}, 
       {0.42171056139889207, 0.11960527740997232}, {0.42171056139889207, 
       0.13250001289473684}, {0.42171056139889207, 0.1453947483795014}, 
       {0.42171056139889207, 0.15828948386426592}, {0.42171056139889207, 
       0.17118421934903047}, {0.42171056139889207, 0.184078954833795}, 
       {0.42171056139889207, 0.19697369031855955}, {0.42171056139889207, 
       0.20986842580332407}, {0.42171056139889207, 0.22276316128808862}, 
       {0.42171056139889207, 0.23565789677285315}, {0.42171056139889207, 
       0.2485526322576177}, {0.42171056139889207, 0.2614473677423822}, 
       {0.42171056139889207, 0.2743421032271468}, {0.42171056139889207, 
       0.2872368387119113}, {0.42171056139889207, 0.3001315741966759}, 
       {0.42171056139889207, 0.3130263096814404}, {0.42171056139889207, 
       0.325921045166205}, {0.42171056139889207, 0.3388157806509695}, 
       {0.42171056139889207, 0.3517105161357341}, {0.42171056139889207, 
       0.3646052516204986}, {0.42171056139889207, 0.3774999871052632}, 
       {0.42171056139889207, 0.3903947225900277}, {0.42171056139889207, 
       0.40328945807479233}, {0.42171056139889207, 0.4161841935595568}, 
       {0.42171056139889207, 0.42907892904432143}, {0.42171056139889207, 
       0.44197366452908593}, {0.42171056139889207, 0.45486840001385054}, 
       {0.42171056139889207, 0.46776313549861503}, {0.42171056139889207, 
       0.4806578709833796}, {0.42171056139889207, 0.4935526064681441}, 
       {0.42171056139889207, 0.49999997421052633}, {0.42171056139889207, 
       0.035789496759002774}, {0.42171056139889207, 0.06157896772853186}, 
       {0.42171056139889207, 0.08736843869806095}, {0.42171056139889207, 
       0.11315790966759004}, {0.42171056139889207, 0.13894738063711912}, 
       {0.42171056139889207, 0.1647368516066482}, {0.42171056139889207, 
       0.19052632257617727}, {0.42171056139889207, 0.21631579354570635}, 
       {0.42171056139889207, 0.24210526451523542}, {0.42171056139889207, 
       0.2678947354847645}, {0.42171056139889207, 0.2936842064542936}, 
       {0.42171056139889207, 0.3194736774238227}, {0.42171056139889207, 
       0.3452631483933518}, {0.42171056139889207, 0.3710526193628809}, 
       {0.42171056139889207, 0.39684209033241}, {0.42171056139889207, 
       0.42263156130193913}, {0.42171056139889207, 0.44842103227146823}, 
       {0.42171056139889207, 0.47421050324099734}, {0.4159668325627057, 
       0.010000025789473685}, {0.4159668325627057, 0.02289476127423823}, 
       {0.4159668325627057, 0.014558516263579901}, {0.4159668325627057, 
       0.01833627080013201}, {0.4159668325627057, 0.031231006284896556}, 
       {0.4159668325627057, 0.027453251748344447}, {0.4159668325627057, 
       0.04868423224376732}, {0.4159668325627057, 0.04034798723310899}, 
       {0.4159668325627057, 0.044125741769661095}, {0.4159668325627057, 
       0.05702047725442565}, {0.4159668325627057, 0.05324272271787353}, 
       {0.4159668325627057, 0.07447370321329641}, {0.4159668325627057, 
       0.06613745820263808}, {0.4159668325627057, 0.06991521273919019}, 
       {0.4159668325627057, 0.08280994822395474}, {0.4159668325627057, 
       0.07903219368740264}, {0.4159668325627057, 0.10026317418282549}, 
       {0.4159668325627057, 0.09192692917216716}, {0.4159668325627057, 
       0.09570468370871926}, {0.4159668325627057, 0.10859941919348381}, 
       {0.4159668325627057, 0.10482166465693171}, {0.4159668325627057, 
       0.1260526451523546}, {0.4159668325627057, 0.11771640014169626}, 
       {0.4159668325627057, 0.12149415467824837}, {0.4159668325627057, 
       0.13438889016301292}, {0.4159668325627057, 0.13061113562646082}, 
       {0.4159668325627057, 0.15184211612188364}, {0.4159668325627057, 
       0.1435058711112253}, {0.4159668325627057, 0.14728362564777742}, 
       {0.4159668325627057, 0.16017836113254197}, {0.4159668325627057, 
       0.15640060659598987}, {0.4159668325627057, 0.17763158709141275}, 
       {0.4159668325627057, 0.16929534208075442}, {0.4159668325627057, 
       0.17307309661730652}, {0.4159668325627057, 0.18596783210207107}, 
       {0.4159668325627057, 0.18219007756551897}, {0.4159668325627057, 
       0.2034210580609418}, {0.4159668325627057, 0.19508481305028347}, 
       {0.4159668325627057, 0.19886256758683557}, {0.4159668325627057, 
       0.21175730307160012}, {0.4159668325627057, 0.20797954853504802}, 
       {0.4159668325627057, 0.2292105290304709}, {0.4159668325627057, 
       0.22087428401981257}, {0.4159668325627057, 0.22465203855636467}, 
       {0.4159668325627057, 0.23754677404112923}, {0.4159668325627057, 
       0.23376901950457712}, {0.4159668325627057, 0.25499999999999995}, 
       {0.4159668325627057, 0.24666375498934162}, {0.4159668325627057, 
       0.2504415095258938}, {0.4159668325627057, 0.2633362450106583}, 
       {0.4159668325627057, 0.2595584904741061}, {0.4159668325627057, 
       0.28078947096952905}, {0.4159668325627057, 0.2724532259588707}, 
       {0.4159668325627057, 0.2762309804954229}, {0.4159668325627057, 
       0.2891257159801874}, {0.4159668325627057, 0.2853479614436352}, 
       {0.4159668325627057, 0.30657894193905816}, {0.4159668325627057, 
       0.29824269692839983}, {0.4159668325627057, 0.302020451464952}, 
       {0.4159668325627057, 0.3149151869497165}, {0.4159668325627057, 
       0.3111374324131643}, {0.4159668325627057, 0.33236841290858726}, 
       {0.4159668325627057, 0.32403216789792894}, {0.4159668325627057, 
       0.3278099224344811}, {0.4159668325627057, 0.3407046579192456}, 
       {0.4159668325627057, 0.33692690338269343}, {0.4159668325627057, 
       0.35815788387811637}, {0.4159668325627057, 0.34982163886745804}, 
       {0.4159668325627057, 0.3535993934040102}, {0.4159668325627057, 
       0.3664941288887747}, {0.4159668325627057, 0.36271637435222254}, 
       {0.4159668325627057, 0.3839473548476455}, {0.4159668325627057, 
       0.37561110983698714}, {0.4159668325627057, 0.3793888643735393}, 
       {0.4159668325627057, 0.3922835998583038}, {0.4159668325627057, 
       0.38850584532175164}, {0.4159668325627057, 0.4097368258171746}, 
       {0.4159668325627057, 0.40140058080651625}, {0.4159668325627057, 
       0.4051783353430684}, {0.4159668325627057, 0.4180730708278329}, 
       {0.4159668325627057, 0.41429531629128075}, {0.4159668325627057, 
       0.4355262967867037}, {0.4159668325627057, 0.42719005177604535}, 
       {0.4159668325627057, 0.4309678063125975}, {0.4159668325627057, 
       0.443862541797362}, {0.4159668325627057, 0.44008478726080985}, 
       {0.4159668325627057, 0.4613157677562328}, {0.4159668325627057, 
       0.45297952274557446}, {0.4159668325627057, 0.4567572772821266}, 
       {0.4159668325627057, 0.4696520127668911}, {0.4159668325627057, 
       0.46587425823033896}, {0.4159668325627057, 0.48710523872576184}, 
       {0.4159668325627057, 0.47876899371510356}, {0.4159668325627057, 
       0.4825467482516556}, {0.4159668325627057, 0.4954414837364201}, 
       {0.4159668325627057, 0.49166372919986806}, {0.4159668325627057, 
       0.49999997421052633}, {0.4159668325627057, 0.035789496759002774}, 
       {0.4159668325627057, 0.06157896772853186}, {0.4159668325627057, 
       0.08736843869806095}, {0.4159668325627057, 0.11315790966759004}, 
       {0.4159668325627057, 0.13894738063711912}, {0.4159668325627057, 
       0.1647368516066482}, {0.4159668325627057, 0.19052632257617727}, 
       {0.4159668325627057, 0.21631579354570635}, {0.4159668325627057, 
       0.24210526451523542}, {0.4159668325627057, 0.2678947354847645}, 
       {0.4159668325627057, 0.2936842064542936}, {0.4159668325627057, 
       0.3194736774238227}, {0.4159668325627057, 0.3452631483933518}, 
       {0.4159668325627057, 0.3710526193628809}, {0.4159668325627057, 
       0.39684209033241}, {0.4159668325627057, 0.42263156130193913}, 
       {0.4159668325627057, 0.44842103227146823}, {0.4159668325627057, 
       0.47421050324099734}}, {{{EdgeForm[], RGBColor[1, 1, 0], Opacity[0.2], 
          GraphicsGroup[{Polygon[{{281, 1, 15}, {17, 2, 3}, {16, 1, 2}, {23, 
             8, 9}, {18, 3, 4}, {19, 4, 5}, {24, 9, 10}, {21, 6, 7}, {20, 5, 
             6}, {25, 10, 11}, {26, 11, 12}, {32, 17, 18}, {30, 15, 16}, {27, 
             12, 13}, {28, 13, 14}, {22, 7, 8}, {282, 15, 29}, {36, 21, 22}, 
             {31, 16, 17}, {33, 18, 19}, {34, 19, 20}, {59, 44, 45}, {35, 20, 
             21}, {58, 43, 44}, {40, 25, 26}, {39, 24, 25}, {46, 31, 32}, 
             {41, 26, 27}, {42, 27, 28}, {47, 32, 33}, {44, 29, 30}, {283, 
             29, 43}, {48, 33, 34}, {49, 34, 35}, {55, 40, 41}, {53, 38, 39}, 
             {50, 35, 36}, {51, 36, 37}, {37, 22, 23}, {52, 37, 38}, {38, 23, 
             24}, {54, 39, 40}, {56, 41, 42}, {284, 43, 57}, {45, 30, 31}, 
             {60, 45, 46}, {92, 77, 78}, {62, 47, 48}, {65, 50, 51}, {64, 49, 
             50}, {66, 51, 52}, {70, 55, 56}, {63, 48, 49}, {68, 53, 54}, 
             {69, 54, 55}, {294, 183, 197}, {285, 57, 71}, {73, 58, 59}, {76, 
             61, 62}, {77, 62, 63}, {74, 59, 60}, {67, 52, 53}, {78, 63, 64}, 
             {81, 66, 67}, {72, 57, 58}, {79, 64, 65}, {80, 65, 66}, {61, 46, 
             47}, {82, 67, 68}, {84, 69, 70}, {87, 72, 73}, {86, 71, 72}, 
             {93, 78, 79}, {88, 73, 74}, {89, 74, 75}, {94, 79, 80}, {91, 76, 
             77}, {90, 75, 76}, {95, 80, 81}, {96, 81, 82}, {102, 87, 88}, 
             {100, 85, 86}, {97, 82, 83}, {98, 83, 84}, {83, 68, 69}, {287, 
             85, 99}, {286, 71, 85}, {101, 86, 87}, {103, 88, 89}, {104, 89, 
             90}, {105, 90, 91}, {106, 91, 92}, {107, 92, 93}, {109, 94, 95}, 
             {116, 101, 102}, {111, 96, 97}, {112, 97, 98}, {288, 99, 113}, 
             {110, 95, 96}, {115, 100, 101}, {114, 99, 100}, {117, 102, 103}, 
             {118, 103, 104}, {119, 104, 105}, {122, 107, 108}, {123, 108, 
             109}, {120, 105, 106}, {128, 113, 114}, {124, 109, 110}, {289, 
             113, 127}, {129, 114, 115}, {125, 110, 111}, {126, 111, 112}, 
             {121, 106, 107}, {130, 115, 116}, {144, 129, 130}, {132, 117, 
             118}, {139, 124, 125}, {134, 119, 120}, {135, 120, 121}, {136, 
             121, 122}, {133, 118, 119}, {138, 123, 124}, {137, 122, 123}, 
             {140, 125, 126}, {290, 127, 141}, {142, 127, 128}, {145, 130, 
             131}, {146, 131, 132}, {143, 128, 129}, {151, 136, 137}, {147, 
             132, 133}, {150, 135, 136}, {131, 116, 117}, {148, 133, 134}, 
             {149, 134, 135}, {108, 93, 94}, {152, 137, 138}, {154, 139, 
             140}, {156, 141, 142}, {291, 141, 155}, {162, 147, 148}, {157, 
             142, 143}, {158, 143, 144}, {163, 148, 149}, {160, 145, 146}, 
             {159, 144, 145}, {164, 149, 150}, {165, 150, 151}, {171, 156, 
             157}, {292, 155, 169}, {166, 151, 152}, {167, 152, 153}, {161, 
             146, 147}, {168, 153, 154}, {175, 160, 161}, {170, 155, 156}, 
             {172, 157, 158}, {173, 158, 159}, {174, 159, 160}, {176, 161, 
             162}, {153, 138, 139}, {185, 170, 171}, {178, 163, 164}, {179, 
             164, 165}, {186, 171, 172}, {180, 165, 166}, {182, 167, 168}, 
             {181, 166, 167}, {184, 169, 170}, {293, 169, 183}, {75, 60, 61}, 
             {187, 172, 173}, {194, 179, 180}, {192, 177, 178}, {189, 174, 
             175}, {190, 175, 176}, {188, 173, 174}, {191, 176, 177}, {177, 
             162, 163}, {193, 178, 179}, {195, 180, 181}, {196, 181, 182}, 
             {110, 125, 124}, {198, 183, 184}, {200, 185, 186}, {202, 187, 
             188}, {201, 186, 187}, {208, 193, 194}, {203, 188, 189}, {204, 
             189, 190}, {209, 194, 195}, {206, 191, 192}, {205, 190, 191}, 
             {210, 195, 196}, {295, 197, 211}, {217, 202, 203}, {215, 200, 
             201}, {212, 197, 198}, {213, 198, 199}, {207, 192, 193}, {214, 
             199, 200}, {221, 206, 207}, {216, 201, 202}, {218, 203, 204}, 
             {219, 204, 205}, {244, 229, 230}, {220, 205, 206}, {243, 228, 
             229}, {296, 211, 225}, {224, 209, 210}, {231, 216, 217}, {226, 
             211, 212}, {227, 212, 213}, {232, 217, 218}, {229, 214, 215}, 
             {228, 213, 214}, {233, 218, 219}, {234, 219, 220}, {240, 225, 
             226}, {238, 223, 224}, {235, 220, 221}, {236, 221, 222}, {222, 
             207, 208}, {237, 222, 223}, {223, 208, 209}, {297, 225, 239}, 
             {241, 226, 227}, {242, 227, 228}, {230, 215, 216}, {245, 230, 
             231}, {277, 262, 263}, {247, 232, 233}, {250, 235, 236}, {249, 
             234, 235}, {251, 236, 237}, {255, 240, 241}, {248, 233, 234}, 
             {298, 239, 253}, {254, 239, 240}, {11, 26, 25}, {256, 241, 242}, 
             {258, 243, 244}, {261, 246, 247}, {262, 247, 248}, {259, 244, 
             245}, {252, 237, 238}, {263, 248, 249}, {266, 251, 252}, {257, 
             242, 243}, {264, 249, 250}, {265, 250, 251}, {246, 231, 232}, 
             {299, 253, 267}, {269, 254, 255}, {272, 257, 258}, {271, 256, 
             257}, {278, 263, 264}, {273, 258, 259}, {274, 259, 260}, {279, 
             264, 265}, {276, 261, 262}, {275, 260, 261}, {280, 265, 266}, 
             {1, 16, 15}, {7, 22, 21}, {5, 20, 19}, {2, 17, 16}, {3, 18, 17}, 
             {268, 253, 254}, {4, 19, 18}, {270, 255, 256}, {6, 21, 20}, {8, 
             23, 22}, {9, 24, 23}, {10, 25, 24}, {12, 27, 26}, {78, 93, 92}, 
             {15, 30, 29}, {22, 37, 36}, {17, 32, 31}, {18, 33, 32}, {19, 34, 
             33}, {16, 31, 30}, {21, 36, 35}, {20, 35, 34}, {23, 38, 37}, 
             {24, 39, 38}, {25, 40, 39}, {29, 44, 43}, {30, 45, 44}, {26, 41, 
             40}, {35, 50, 49}, {31, 46, 45}, {34, 49, 48}, {36, 51, 50}, 
             {32, 47, 46}, {33, 48, 47}, {27, 42, 41}, {37, 52, 51}, {52, 67, 
             66}, {39, 54, 53}, {47, 62, 61}, {41, 56, 55}, {43, 58, 57}, 
             {44, 59, 58}, {40, 55, 54}, {46, 61, 60}, {45, 60, 59}, {48, 63, 
             62}, {49, 64, 63}, {50, 65, 64}, {53, 68, 67}, {54, 69, 68}, 
             {51, 66, 65}, {60, 75, 74}, {55, 70, 69}, {59, 74, 73}, {38, 53, 
             52}, {57, 72, 71}, {58, 73, 72}, {61, 76, 75}, {62, 77, 76}, 
             {63, 78, 77}, {64, 79, 78}, {67, 82, 81}, {66, 81, 80}, {68, 83, 
             82}, {73, 88, 87}, {65, 80, 79}, {71, 86, 85}, {72, 87, 86}, 
             {13, 28, 27}, {74, 89, 88}, {76, 91, 90}, {79, 94, 93}, {80, 95, 
             94}, {77, 92, 91}, {69, 84, 83}, {81, 96, 95}, {85, 100, 99}, 
             {75, 90, 89}, {82, 97, 96}, {83, 98, 97}, {86, 101, 100}, {87, 
             102, 101}, {88, 103, 102}, {97, 112, 111}, {90, 105, 104}, {91, 
             106, 105}, {99, 114, 113}, {92, 107, 106}, {94, 109, 108}, {93, 
             108, 107}, {96, 111, 110}, {95, 110, 109}, {199, 184, 185}, 
             {100, 115, 114}, {107, 122, 121}, {105, 120, 119}, {102, 117, 
             116}, {103, 118, 117}, {101, 116, 115}, {104, 119, 118}, {89, 
             104, 103}, {106, 121, 120}, {108, 123, 122}, {109, 124, 123}, 
             {260, 245, 246}, {111, 126, 125}, {338, 367, 310}, {116, 131, 
             130}, {115, 130, 129}, {122, 137, 136}, {117, 132, 131}, {118, 
             133, 132}, {123, 138, 137}, {120, 135, 134}, {119, 134, 133}, 
             {124, 139, 138}, {125, 140, 139}, {132, 147, 146}, {130, 145, 
             144}, {127, 142, 141}, {128, 143, 142}, {121, 136, 135}, {129, 
             144, 143}, {136, 151, 150}, {131, 146, 145}, {133, 148, 147}, 
             {134, 149, 148}, {161, 176, 175}, {135, 150, 149}, {160, 175, 
             174}, {141, 156, 155}, {139, 154, 153}, {147, 162, 161}, {142, 
             157, 156}, {143, 158, 157}, {148, 163, 162}, {145, 160, 159}, 
             {144, 159, 158}, {149, 164, 163}, {150, 165, 164}, {157, 172, 
             171}, {155, 170, 169}, {151, 166, 165}, {152, 167, 166}, {137, 
             152, 151}, {153, 168, 167}, {138, 153, 152}, {156, 171, 170}, 
             {158, 173, 172}, {159, 174, 173}, {146, 161, 160}, {162, 177, 
             176}, {197, 212, 211}, {164, 179, 178}, {167, 182, 181}, {166, 
             181, 180}, {169, 184, 183}, {173, 188, 187}, {165, 180, 179}, 
             {171, 186, 185}, {172, 187, 186}, {359, 321, 302}, {174, 189, 
             188}, {176, 191, 190}, {179, 194, 193}, {180, 195, 194}, {177, 
             192, 191}, {170, 185, 184}, {181, 196, 195}, {185, 200, 199}, 
             {175, 190, 189}, {183, 198, 197}, {184, 199, 198}, {163, 178, 
             177}, {186, 201, 200}, {188, 203, 202}, {191, 206, 205}, {190, 
             205, 204}, {198, 213, 212}, {192, 207, 206}, {193, 208, 207}, 
             {199, 214, 213}, {195, 210, 209}, {194, 209, 208}, {200, 215, 
             214}, {201, 216, 215}, {207, 222, 221}, {205, 220, 219}, {202, 
             217, 216}, {203, 218, 217}, {187, 202, 201}, {204, 219, 218}, 
             {189, 204, 203}, {206, 221, 220}, {208, 223, 222}, {209, 224, 
             223}, {211, 226, 225}, {212, 227, 226}, {213, 228, 227}, {215, 
             230, 229}, {222, 237, 236}, {217, 232, 231}, {218, 233, 232}, 
             {219, 234, 233}, {216, 231, 230}, {221, 236, 235}, {220, 235, 
             234}, {223, 238, 237}, {225, 240, 239}, {226, 241, 240}, {229, 
             244, 243}, {230, 245, 244}, {227, 242, 241}, {235, 250, 249}, 
             {231, 246, 245}, {234, 249, 248}, {236, 251, 250}, {232, 247, 
             246}, {233, 248, 247}, {228, 243, 242}, {237, 252, 251}, {253, 
             268, 267}, {240, 255, 254}, {247, 262, 261}, {242, 257, 256}, 
             {243, 258, 257}, {244, 259, 258}, {241, 256, 255}, {246, 261, 
             260}, {245, 260, 259}, {248, 263, 262}, {249, 264, 263}, {250, 
             265, 264}, {254, 269, 268}, {255, 270, 269}, {251, 266, 265}, 
             {260, 275, 274}, {256, 271, 270}, {259, 274, 273}, {239, 254, 
             253}, {257, 272, 271}, {258, 273, 272}, {214, 229, 228}, {261, 
             276, 275}, {263, 278, 277}, {265, 280, 279}, {264, 279, 278}, 
             {304, 283, 43}, {320, 301, 281}, {302, 281, 15}, {326, 304, 
             284}, {303, 282, 29}, {322, 302, 282}, {305, 284, 57}, {328, 
             305, 285}, {334, 308, 288}, {332, 307, 287}, {306, 285, 71}, 
             {330, 306, 286}, {324, 303, 283}, {307, 286, 85}, {338, 310, 
             290}, {308, 287, 99}, {309, 288, 113}, {336, 309, 289}, {310, 
             289, 127}, {311, 290, 141}, {262, 277, 276}, {348, 315, 295}, 
             {312, 291, 155}, {342, 312, 292}, {316, 295, 211}, {313, 292, 
             169}, {314, 293, 183}, {344, 313, 293}, {315, 294, 197}, {346, 
             314, 294}, {178, 193, 192}, {350, 316, 296}, {300, 299, 267}, 
             {319, 298, 253}, {352, 317, 297}, {318, 297, 239}, {317, 296, 
             225}, {354, 318, 298}, {340, 311, 291}, {356, 319, 299}, {358, 
             357, 300}, {281, 301, 1}, {113, 128, 127}, {114, 129, 128}, 
             {283, 303, 29}, {305, 327, 284}, {304, 325, 283}, {307, 331, 
             286}, {306, 329, 285}, {308, 333, 287}, {312, 341, 291}, {294, 
             314, 183}, {293, 313, 169}, {364, 331, 307}, {361, 325, 304}, 
             {287, 307, 85}, {372, 347, 315}, {362, 327, 305}, {363, 329, 
             306}, {286, 306, 71}, {285, 305, 57}, {311, 339, 290}, {310, 
             337, 289}, {309, 335, 288}, {298, 318, 239}, {381, 382, 321}, 
             {375, 353, 318}, {282, 302, 15}, {461, 462, 353}, {460, 459, 
             352}, {455, 454, 350}, {284, 304, 43}, {297, 317, 225}, {296, 
             316, 211}, {303, 323, 282}, {302, 321, 281}, {374, 351, 317}, 
             {299, 319, 253}, {295, 315, 197}, {376, 355, 319}, {373, 349, 
             316}, {466, 467, 355}, {365, 333, 308}, {366, 335, 309}, {360, 
             323, 303}, {317, 351, 296}, {316, 349, 295}, {319, 355, 298}, 
             {318, 353, 297}, {330, 363, 306}, {334, 365, 308}, {346, 371, 
             314}, {348, 372, 315}, {336, 366, 309}, {342, 369, 312}, {300, 
             357, 299}, {340, 368, 311}, {332, 364, 307}, {350, 373, 316}, 
             {344, 370, 313}, {328, 362, 305}, {326, 361, 304}, {324, 360, 
             303}, {290, 310, 127}, {291, 311, 141}, {368, 339, 311}, {371, 
             345, 314}, {292, 312, 155}, {369, 341, 312}, {370, 343, 313}, 
             {288, 308, 99}, {289, 309, 113}, {313, 343, 292}, {322, 359, 
             302}, {352, 374, 317}, {367, 337, 310}, {354, 375, 318}, {315, 
             347, 294}, {314, 345, 293}, {356, 376, 319}, {456, 457, 351}, 
             {380, 379, 320}, {396, 397, 327}, {471, 472, 357}, {431, 432, 
             341}, {395, 394, 326}, {440, 439, 344}, {436, 437, 343}, {430, 
             429, 340}, {441, 442, 345}, {406, 407, 331}, {410, 409, 332}, 
             {401, 402, 329}, {400, 399, 328}, {411, 412, 333}, {470, 469, 
             356}, {390, 389, 324}, {405, 404, 330}, {385, 384, 322}, {435, 
             434, 342}, {451, 452, 349}, {450, 449, 348}, {465, 464, 354}, 
             {391, 392, 325}, {420, 419, 336}, {421, 422, 337}, {446, 447, 
             347}, {415, 414, 334}, {416, 417, 335}, {386, 387, 323}, {426, 
             427, 339}, {445, 444, 346}, {425, 424, 338}}], 
            Polygon[{{428, 430, 340, 291}, {433, 435, 342, 292}, {383, 385, 
             322, 282}, {418, 420, 336, 289}, {403, 405, 330, 286}, {398, 
             400, 328, 285}, {393, 395, 326, 284}, {388, 390, 324, 283}, 
             {423, 425, 338, 290}, {463, 465, 354, 298}, {479, 406, 331, 
             364}, {379, 377, 301, 320}, {484, 431, 341, 369}, {482, 421, 
             337, 367}, {412, 408, 287, 333}, {480, 411, 333, 365}, {417, 
             413, 288, 335}, {481, 416, 335, 366}, {422, 418, 289, 337}, 
             {432, 428, 291, 341}, {427, 423, 290, 339}, {483, 426, 339, 
             368}, {378, 380, 320, 281}, {458, 460, 352, 297}, {448, 450, 
             348, 295}, {453, 455, 350, 296}, {438, 440, 344, 293}, {468, 
             470, 356, 299}, {437, 433, 292, 343}, {443, 445, 346, 294}, 
             {408, 410, 332, 287}, {452, 448, 295, 349}, {392, 388, 283, 
             325}, {491, 466, 355, 376}, {429, 483, 368, 340}, {424, 482, 
             367, 338}, {439, 485, 370, 344}, {434, 484, 369, 342}, {487, 
             446, 347, 372}, {459, 489, 374, 352}, {444, 486, 371, 346}, 
             {454, 488, 373, 350}, {464, 490, 375, 354}, {457, 453, 296, 
             351}, {488, 451, 349, 373}, {442, 438, 293, 345}, {462, 458, 
             297, 353}, {490, 461, 353, 375}, {467, 463, 298, 355}, {382, 
             378, 281, 321}, {447, 443, 294, 347}, {489, 456, 351, 374}, 
             {449, 487, 372, 348}, {419, 481, 366, 336}, {414, 480, 365, 
             334}, {478, 401, 329, 363}, {407, 403, 286, 331}, {397, 393, 
             284, 327}, {486, 441, 345, 371}, {476, 391, 325, 361}, {402, 
             398, 285, 329}, {475, 386, 323, 360}, {387, 383, 282, 323}, 
             {477, 396, 327, 362}, {474, 381, 321, 359}, {485, 436, 343, 
             370}, {404, 478, 363, 330}, {472, 468, 299, 357}, {409, 479, 
             364, 332}, {413, 415, 334, 288}, {473, 471, 357, 358}, {389, 
             475, 360, 324}, {384, 474, 359, 322}, {399, 477, 362, 328}, 
             {394, 476, 361, 326}, {469, 491, 376, 356}}]}]}, {}, {}, {}, 
         {}}, {{RGBColor[2/3, 2/3, 0], Line[{2, 1, 301, 377, 379, 380, 378, 
           382, 381, 474, 384, 385, 383, 387, 386, 475, 389, 390, 388, 392, 
           391, 476, 394, 395, 393, 397, 396, 477, 399, 400, 398, 402, 401, 
           478, 404, 405, 403, 407, 406, 479, 409, 410, 408, 412, 411, 480, 
           414, 415, 413, 417, 416, 481, 419, 420, 418, 422, 421, 482, 424, 
           425, 423, 427, 426, 483, 429, 430, 428, 432, 431, 484, 434, 435, 
           433, 437, 436, 485, 439, 440, 438, 442, 441, 486, 444, 445, 443, 
           447, 446, 487, 449, 450, 448, 452, 451, 488, 454, 455, 453, 457, 
           456, 489, 459, 460, 458, 462, 461, 490, 464, 465, 463, 467, 466, 
           491, 469, 470, 468, 472, 471, 473, 358, 300, 267, 268, 269, 270, 
           271, 272, 273, 274, 275, 276, 277, 278, 279, 280, 266, 252, 238, 
           224, 210, 196, 182, 168, 154, 140, 126, 112, 98, 84, 70, 56, 42, 
           28, 14, 13, 12, 11, 10, 9, 8, 7, 6, 5, 4, 3, 2}]}}}], {}}, 
     {PlotLabel -> "\!\(\*SubscriptBox[\(M\), \(jj\)]\)=150 GeV, \
\!\(\*SubscriptBox[\(M\), \(Wjj\)]\)=260 GeV", PlotRange -> 
       {{0.05, 1}, {0.02, 0.45}}, AspectRatio -> 0.7, ImageSize -> 250, 
      AspectRatio -> 1, Frame -> True, FrameLabel -> 
       {"\[Lambda]", "\!\(\*SubscriptBox[\(g\), \(Q\)]\)"}, 
      Method -> {"TransparentPolygonMesh" -> True, "AxesInFront" -> True}, 
      PlotRange -> {{0.01, 1.5}, {0.01, 0.5}}, PlotRangeClipping -> True, 
      PlotRangePadding -> {Scaled[0.02], Scaled[0.02]}}]

